One-Wayness in Quantum Cryptography

The existence of one-way functions is one of the most fundamental assumptions in classical cryptography. In the quantum world, on the other hand, there are evidences that some cryptographic primitives can exist even if one-way functions do not exist. We therefore have the following important open problem in quantum cryptography: What is the most fundamental element in quantum cryptography? In this direction, Brakerski, Canetti, and Qian recently defined a notion called EFI pairs, which are pairs of efficiently generatable states that are statistically distinguishable but computationally indistinguishable, and showed its equivalence with some cryptographic primitives including commitments, oblivious transfer, and general multi-party computations. However, their work focuses on decision-type primitives and does not cover search-type primitives like quantum money and digital signatures. In this paper, we study properties of one-way state generators (OWSGs), which are a quantum analogue of one-way functions. We first revisit the definition of OWSGs and generalize it by allowing mixed output states. Then we show the following results. (1) We define a weaker version of OWSGs, weak OWSGs, and show that they are equivalent to OWSGs. (2) Quantum digital signatures are equivalent to OWSGs. (3) Private-key quantum money schemes (with pure money states) imply OWSGs. (4) Quantum pseudo one-time pad schemes imply both OWSGs and EFI pairs. (5) We introduce an incomparable variant of OWSGs, which we call secretly-verifiable and statistically-invertible OWSGs, and show that they are equivalent to EFI pairs.

==> 1-OWSGfromEFI.tex <==
\section{Single-copy OWSGs from EFI pairs}
\label{sec:1-OWSG}

\begin{theorem}
If EFI pairs exist then single-copy OWSGs exist.
\end{theorem}

\begin{proof}
Let $\mathsf{EFI}.\Gen(b,1^\secp)\to\rho_b$ be an EFI pair.
Without loss of generality, we can assume that the algorithm $\mathsf{EFI}.\Gen$ runs as follows. It applies a QPT unitary $U_b$ on $|0...0\rangle_{AB}$ to
generate $|\psi_b\rangle_{AB}\coloneqq U_b|0...0\rangle_{AB}$, and trace out the register $A$.
It outputs the state $\rho_b$ of the register $B$.
Let $m$ be the number of qubits in the register $A$.

From the EFI pair, we construct a single-copy OWSG as follows.
\begin{itemize}
    \item 
    $\Gen_1(1^\secp)\to (k,x,z):$
    Choose $k\gets\bit^\secp$. Define 
    $x\coloneqq \{x_{i,j}\}_{i=1,j=1}^{\secp,m}$
    $z\coloneqq \{z_{i,j}\}_{i=1,j=1}^{\secp,m}$.
    Choose $x_{i,j},z_{i,j}\gets\bit$ for each $i\in[\secp]$ and each $j\in [m]$.
    Output $(k,x,z)$.
    \item
    $\Gen_2(k,x,z)\to |\phi_{k,x,z}\rangle:$
    Generate $|\psi_{k_i}\rangle_{A_iB_i}\coloneqq U_{k_i}|0...0\rangle_{A_iB_i}$ for each $i\in[\secp]$.
    Define 
    \begin{eqnarray*}
    |\Psi_{k_i,x_i,z_i}\rangle_{A_iB_i}\coloneqq ((X^{x_i}Z^{z_i})_{A_i}\otimes I_{B_i})|\psi_{k_i}\rangle_{A_iB_i}
    \end{eqnarray*}
    for each $i\in[\secp]$,
    where $x_i\coloneqq(x_{i,1},x_{i,2},...,x_{i,m})$
    and $z_i\coloneqq(z_{i,1},z_{i,2},...,z_{i,m})$.
   Output $|\phi_{k,x,z}\rangle\coloneqq \bigotimes_{i=1}^\secp|\Psi_{k_i,x_i,z_i}\rangle$. 
   \item
   $\Ver((k',x',z'),|\phi_{k,x,z}\rangle)\to\top/\bot:$
   Parse $|\phi_{k,x,z}\rangle=\bigotimes_{i=1}^\secp|\Psi_{k_i,x_i,z_i}\rangle$. 
   For each $i\in[\secp]$, do the following operation.
   First, apply $X^{x_i'}Z^{z_i'}$ on the $A_i$ register of $|\Psi_{k_i,x_i,z_i}\rangle_{A_iB_i}$,
   which maps $|\Psi_{k_i,x_i,z_i}\rangle$ to $|\Psi_{k_i,x_i\oplus x_i',z_i\oplus z_i'}\rangle$.
   Next, ppply $U_{k_i'}^\dagger$, which maps
   $|\Psi_{k_i,x_i\oplus x_i',z_i\oplus z_i'}\rangle$ to
   $U_{k_i'}^\dagger|\Psi_{k_i,x_i\oplus x_i',z_i\oplus z_i'}\rangle$.
   Finally, measure all qubits in the computational basis.
   If the result is all 0, set $v_i=1$. Otherwise, set $v_i=0$.
   If $\sum_{i=1}^\secp v_i=\secp$, 
   output $\top$. Otherwise, output $\bot$.
\end{itemize}
The correctness is clear. Let us show the security.
Assume that there exists a QPT adversary $\cA$ and a polynomial $p$ such that
\begin{eqnarray}
\frac{1}{2^{\secp+2\secp m}}\sum_{k,x,z}\sum_{k',x',z'}
\Pr[(k',x',z')\gets\cA(|\phi_{k,x,z}\rangle)]
\prod_{i=1}^\secp|\langle\Psi_{k_i,x_i,z_i}|\Psi_{k_i',x_i',z_i'}\rangle|^2
\ge\frac{1}{p}.
\label{1OWSG_A}
\end{eqnarray}
Note that
$|\langle\Psi_{k_i,x_i,z_i}|\Psi_{k_i',x_i',z_i'}\rangle|^2\le\negl(\secp)$
for any $x_i,z_i,x_i',z_i'$ and any $k_i,k_i'$ such that $k_i\neq k_i'$.
In fact,
\begin{eqnarray*}
|\langle\Psi_{k_i,x_i,z_i}|\Psi_{k_i',x_i',z_i'}\rangle|^2
&=&
|\langle\psi_{k_i}|(X^{x_i}Z^{z_i}\otimes I)(X^{x_i'}Z^{z_i'}\otimes I)|\psi_{k_i'}\rangle|^2\\
&=&
F((X^{x_i}Z^{z_i}\otimes I)|\psi_{k_i}\rangle,
(X^{x_i'}Z^{z_i'}\otimes I)|\psi_{k_i'}\rangle)\\
&\le&
F(\rho_{k_i},
\rho_{k_i'})\\
&\le&
\negl(\secp).
\end{eqnarray*}
Therefore, Eq.~(\ref{1OWSG_A}) becomes
\begin{eqnarray*}
\frac{1}{p}&\le&\frac{1}{2^{\secp+2\secp m}}\sum_{k,x,z,k',x',z'}
\Pr[(k',x',z')\gets\cA(|\phi_{k,x,z}\rangle)]
\prod_{i=1}^\secp|\langle\Psi_{k_i,x_i,z_i}|\Psi_{k_i',x_i',z_i'}\rangle|^2\\
&=&
\frac{1}{2^{\secp+2\secp m}}\sum_{k,x,z,x',z'}
\Pr[(k,x',z')\gets\cA(|\phi_{k,x,z}\rangle)]
\prod_{i=1}^\secp|\langle\Psi_{k_i,x_i,z_i}|\Psi_{k_i,x_i',z_i'}\rangle|^2\\
&&+
\frac{1}{2^{\secp+2\secp m}}\sum_{k,x,z,k',x',z':k\neq k'}
\Pr[(k',x',z')\gets\cA(|\phi_{k,x,z}\rangle)]
\prod_{i=1}^\secp|\langle\Psi_{k_i,x_i,z_i}|\Psi_{k_i',x_i',z_i'}\rangle|^2\\
&\le&
\frac{1}{2^{\secp+2\secp m}}\sum_{k,x,z,x',z'}
\Pr[(k,x',z')\gets\cA(|\phi_{k,x,z}\rangle)]\\
&&+\negl(\secp)
\frac{1}{2^{\secp+2\secp m}}\sum_{k,x,z,k',x',z':k\neq k'}
\Pr[(k',x',z')\gets\cA(|\phi_{k,x,z}\rangle)]\\
&\le&
\frac{1}{2^{\secp+2\secp m}}\sum_{k,x,z,x',z'}
\Pr[(k,x',z')\gets\cA(|\phi_{k,x,z}\rangle)]
+\negl(\secp),
\end{eqnarray*}
which means
\begin{eqnarray*}
\frac{1}{2^{\secp+2\secp m}}\sum_{k,x,z,x',z'}
\Pr[(k,x',z')\gets\cA(|\phi_{k,x,z}\rangle)]
\ge\frac{1}{p}-\negl(\secp).
\end{eqnarray*}
It is equivalent to
\begin{eqnarray*}
\frac{1}{2^{\secp}}
\sum_{k}
\Pr\Big[k\gets\cA\Big(\bigotimes_{i=1}^\secp\Big(\frac{I^{\otimes m}}{2^m}\otimes\rho_{k_i}\Big)\Big)\Big]
\ge\frac{1}{p}-\negl(\secp).
\end{eqnarray*}
From this $\cA$, let us construct a QPT adversary $\cB$ that breaks the security of the EFI pair as follows.
On input $\rho_b$ with a uniformly random $b\gets\bit$, choose $k_2,...,k_\secp\gets\bit$ and runs
\begin{eqnarray*}
(k',x',z')\gets\cA\Big(\Big(\frac{I^{\otimes m}}{2^m}\otimes\rho_b\Big)\otimes\bigotimes_{j=2}^\secp \Big(\frac{I^{\otimes m}}{2^m}\otimes\rho_{k_i}\Big)\Big).
\end{eqnarray*}
Output $k'_1$.
Then, the probability that $\cB$ wins is at least
\begin{eqnarray*}
\frac{1}{2^\secp}\sum_{b,k_2,...,k_\secp}\Pr[k\gets\cA(\rho_b\otimes\rho_2\otimes...\otimes\rho_\secp)]
\ge\frac{1}{p}-\negl(\secp),
\end{eqnarray*}
which is non-negligible, and therefore $\cB$ breaks the security of the EFI pair.
\mor{it must be larger than 1/2!}
\mor{weak nara ikeru.}


\end{proof}

==> DSfromEFI.tex <==
\section{OWSG from EFI}
\mor{mikansei}

Let $\mathsf{EFI}.\StateGen(1^\secp,b)\to\rho_b$ be an EFI pair.
Without loss of generality, we can assume that it first applies a QPT unitary $U_{1^\secp,b}$ on $|0...0\rangle_{AB}$
to generate $|\psi_b\rangle\coloneqq U_{1^\secp,b}|0...0\rangle$,
and then traces out the register $A$ to get the state $\rho_b$ of the register $B$.

From it, we construct OWSG as follows.
We define
\begin{eqnarray*}
\phi_{k,\sk}\coloneqq \bigotimes_{i=1}^n [(\Enc_{\sk})_{A_i}|\psi_{k_i}\rangle\langle\psi_{k_i}|_{A_i,B_i}].
\end{eqnarray*}
Then, a QPT algorithm $\mathsf{OWSG}.\StateGen(1^\secp,(x,z,k))\to|\phi_{x,z,k}\rangle$ is a OWSG.
In fact,
for any QPT adversary $\cA$,
\begin{eqnarray*}
&&\frac{1}{2^{2n|A|+n}}\sum_{x,z,k}\sum_{x',z',k'}
\Pr[(x',z',k')\gets\cA(|\phi_{x,z,k}\rangle)]
|\langle\phi_{x,z,k}|\phi_{x',z',k'}\rangle|^2\\
&=&\frac{1}{2^{2n|A|+n}}\sum_{x,z,k}\sum_{x',z',k'}
\mbox{Tr}[\Pi_{x',z',k'}|\phi_{x,z,k}\rangle\langle\phi_{x,z,k}|]
\mbox{Tr}[|\phi_{x',z',k'}\rangle\langle\phi_{x',z',k'}|\times|\phi_{x,z,k}\rangle\langle\phi_{x,z,k}|]\\
&=&\frac{1}{2^{2n|A|+n}}\sum_{x,z,k}\sum_{x',z',k'}
\mbox{Tr}[\Pi_{x',z',k'}\otimes |\phi_{x',z',k'}\rangle\langle\phi_{x',z',k'}|\times
|\phi_{x,z,k}\rangle\langle\phi_{x,z,k}|^{\otimes 2}]\\
\end{eqnarray*}

Let $x\coloneqq(x_1,...,x_n)$, $z\coloneqq(z_1,...,z_n)$, and $k\coloneqq(k_1,...,k_n)$,
where $x_i,z_i\in\bit^{|A|}$ and $k_i\in\bit$.
Then, for each $x,z,k$,
we define
\begin{eqnarray*}
|\phi_{x,z,k}\rangle\coloneqq \bigotimes_{i=1}^n [(X^{x_i}Z^{z_i})_{A_i}|\psi_{k_i}\rangle_{A_i,B_i}].
\end{eqnarray*}
Then, a QPT algorithm $\mathsf{OWSG}.\StateGen(1^\secp,(x,z,k))\to|\phi_{x,z,k}\rangle$ is a OWSG.
In fact,
for any QPT adversary $\cA$,
\begin{eqnarray*}
&&\frac{1}{2^{2n|A|+n}}\sum_{x,z,k}\sum_{x',z',k'}
\Pr[(x',z',k')\gets\cA(|\phi_{x,z,k}\rangle)]
|\langle\phi_{x,z,k}|\phi_{x',z',k'}\rangle|^2\\
&=&\frac{1}{2^{2n|A|+n}}\sum_{x,z,k}\sum_{x',z',k'}
\mbox{Tr}[\Pi_{x',z',k'}|\phi_{x,z,k}\rangle\langle\phi_{x,z,k}|]
\mbox{Tr}[|\phi_{x',z',k'}\rangle\langle\phi_{x',z',k'}|\times|\phi_{x,z,k}\rangle\langle\phi_{x,z,k}|]\\
&=&\frac{1}{2^{2n|A|+n}}\sum_{x,z,k}\sum_{x',z',k'}
\mbox{Tr}[\Pi_{x',z',k'}\otimes |\phi_{x',z',k'}\rangle\langle\phi_{x',z',k'}|\times
|\phi_{x,z,k}\rangle\langle\phi_{x,z,k}|^{\otimes 2}]\\
\end{eqnarray*}

==> EFIfromDS.tex <==
\section{EFI from DS}
\begin{definition}[Quantum digital signatures with quantum public keys]
A quantum digital signature scheme with quantum public keys is a tuple of algorithms $(\Gen,\Sign,\Ver)$ such that
\begin{itemize}
\item
$\Gen_1(1^\secp)\to \sk:$
It is a QPT algorithm that, on input the security parameter $\secp$, outputs a classical secret key $\sk$.
\item
$\Gen_2(\sk)\to \rho_{\sk}:$
It is a QPT algorithm that, on input $\sk$, outputs a quantum public key $\rho_{\sk}$.
More precisely, it first runs a classical polynomial-time deterministic algorithm that, on input $\sk$, outputs
a classical description of a quantum circuit that implements a unitary $U_{\sk}$. It then
applies $U_{\sk}$ on $|0...0\rangle$ to generate a state $|\psi_{\sk}\rangle_{\regA\regB}$ on the registers $\regA$ and $\regB$. 
It outputs the state $\rho_{\sk}$ of the register $\regA$.
\item
$\Sign(\sk,m)\to\sigma:$
It is a QPT algorithm that, on input $\sk$ and a message $m$, outputs a classical signature $\sigma$.
\item
$\Ver(m,\sigma,\rho_{\sk})\to\top/\bot:$
It is a QPT algorithm that, on input $m$, $\sigma$ and $\rho_{\sk}$, outputs $\top$ or $\bot$.
\end{itemize}
We require the following correctness and security.
\paragraph{\bf Correctness:}
For any message $m$,
\begin{eqnarray*}
\Pr[\top\gets\Ver(m,\sigma,\rho_{\sk}):\sk\gets\Gen_1(1^\secp),\rho_{\sk}\gets\Gen_2(\sk),\sigma\gets\Sign(\sk,m)]\ge1-\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For any QPT adversary $\cA$ and any message $m$,
\begin{eqnarray*}
\Pr[\top\gets\Ver(m,\sigma,\rho_{\sk}):\sk\gets\Gen_1(1^\secp),\rho_{\sk}\gets\Gen_2(\sk),(m,\sigma)\gets\cA(\rho_{\sk})]\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{definition}[Statistically distinguishable but computationally indistinguishable states generators]
\end{definition}


\begin{theorem}
If quantum digital signatures with quantum public keys exist then
SDCISG exist.
\end{theorem}

\begin{proof}
Let us consider the following security game of SDCISG with the parameter $b\in\bit$ between a challenger $\cC$ and a QPT adversary $\cA$.
\begin{enumerate}
    \item 
    $\cC$ runs $\sk\leftarrow \Gen_1(1^\secp)$.
    $\cC$ generates $|\psi_{\sk}^b\rangle\coloneqq|0\rangle|\sk\rangle+(-1)^b|1\rangle|\phi_{\sk}\rangle$,
    and sends it to $\cA$.
    (The number of qubits of $|\sk\rangle$ and $|\psi_{\sk}\rangle$ could be different with each other.
    In that case, we implicitly assume that $|0\rangle$ states are appropriately padded.)
    Note that this state can be generated in QPT as follows.
    \begin{enumerate}
        \item 
        Prepare $|0\rangle|\sk\rangle|0...0\rangle+(-1)^b|1\rangle|\sk\rangle|0...0\rangle$.
        \item
        Copy the content of the second register to the third register if the first qubit is 0:
        $|0\rangle|\sk\rangle|\sk\rangle+(-1)^b|1\rangle|\sk\rangle|0...0\rangle$.
        \item
        Run $\Gen_2$ on the second and third registers if the first qubit is 1:
        $|0\rangle|\sk\rangle|\sk\rangle+(-1)^b|1\rangle|\sk\rangle|\phi_{\sk}\rangle$.
        \item
        Swap the second and the third registers if the first qubit is 1:
        $|0\rangle|\sk\rangle|\sk\rangle+(-1)^b|1\rangle|\phi_{\sk}\rangle|\sk\rangle$.
        \item
        Discard the third register:
        $|0\rangle|\sk\rangle+(-1)^b|1\rangle|\phi_{\sk}\rangle$.
    \end{enumerate}
    \item
    $\cA$ sends $b'\in\{0,1\}$ to $C$.
\end{enumerate}
Assume that $|\Pr[b'=1|b=0]-\Pr[b'=1|b=1]|\ge\frac{1}{p}$
with a certain polynomial $p$.
Then, due to the average argument, for $1/2p$ fraction of $\sk$,
\begin{eqnarray*}
|\Pr[1\leftarrow A(|\psi_{\sk}^{b=0}\rangle)|b=0]
-\Pr[1\leftarrow A(|\psi_{\sk}^{b=1}\rangle)|b=0]|\ge \frac{1}{2p}.
\end{eqnarray*}
Let us fix such $\sk$. From [AAS], there exists a QPT unitary $U$ such that
$|\langle0|\langle\sk|U|1\rangle|\phi_{\sk}\rangle|\ge\frac{1}{p}$. 
It is clear that by using $U$, we can break the security of the quantum digital signatures.
\end{proof}

==> EFIfromOTP.tex <==
\section{EFI from quantum pseudo OTPs}

\begin{definition}[Quantum pseudo one-time pads]
A quantum pseudo one-time pad scheme is a tuple of algorithms $(\Enc,\Dec)$ such that
\begin{itemize}
    \item 
    $\Enc(k,x)\to\ct:$ It is a QPT algorithm that, on input a classical secret key $k\in\bit^\secp$ and 
    a classical message $x\in\bit^l$ with
    $l>\secp$, outputs an $ln$-qubit quantum ciphertext $\ct$.
    \item
    $\Dec(\ct,k)\to x':$ It is a QPT algorithm that, on input $\ct$ and $k$, outputs $x'\in\bit^l$.
\end{itemize}
\paragraph{\bf Correctness:}
For any $x\in\bit^l$,
\begin{eqnarray*}
\Pr[x\gets\Dec(k,\ct):k\gets\bit^\secp,\ct\gets\Enc(k,x)]\ge1-\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For any $x\in\bit^l$, any QPT adversary $\cA$, and any polynomial $t$,
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\ct^{\otimes t}):k\gets\bit^\secp,\ct\gets\Enc(k,x)]\\
&&-\Pr[1\gets\cA((|\psi_1\rangle\otimes...\otimes |\psi_l\rangle)^{\otimes t}):|\psi_1\rangle,...,|\psi_l\rangle\gets \mu_n]|
\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{theorem}
If quantum pseudo one-time pads exist then EFI exists.
\end{theorem}

\begin{proof}
Let $\ct_{k,x}$ be the output of $\Enc(k,x)$.
Define an algorithm $\StateGen(1^\secp,b)$ that outputs
\begin{eqnarray*}
\rho_0&\coloneqq&\frac{1}{2^{\secp+l}}\sum_{k\in\bit^\secp,x\in\bit^l}\ct_{k,x}^{\otimes T+1},\\
\rho_1&\coloneqq&\int_{|\psi_1\rangle,...,|\psi_l\rangle\gets\mu_n}(|\psi_1\rangle\langle\psi_1|\otimes...\otimes|\psi_l\rangle\langle\psi_l|)^{\otimes T+1},
\end{eqnarray*}
as follows.
(Here, $T$ is a certain polynomial specified later.)
\begin{enumerate}
    \item 
    \item
\end{enumerate}
It is clear that thus defined $\StateGen$ is QPT.


\begin{eqnarray*}
\rho_0&\coloneqq&\frac{1}{2^{\secp+l}}\sum_{k\in\bit^\secp,x\in\bit^l}\ct_{k,x}\\
&=&\sum_{i=1}^\xi\lambda_i|\phi_i\rangle\langle\phi_i|,\\
\rho_1&\coloneqq&\int_{|\psi_1\rangle,...,|\psi_l\rangle\gets\mu_n}
(|\psi_1\rangle\langle\psi_1|\otimes...\otimes|\psi_l\rangle\langle\psi_l|)\\
&=&\Big(\frac{I^{\otimes n}}{2^n}\Big)^{\otimes l}.
\end{eqnarray*}
\begin{eqnarray*}
F(\rho_0,\rho_1)&=&\mbox{Tr}\sqrt{\sqrt{I^{\otimes nl}/2^{nl}}\sigma\sqrt{I^{\otimes nl}/2^{nl}}}
\end{eqnarray*}
$\xi\le 2^{\secp+l+nl}$
$\frac{2^{\secp+l+nl}}{2^{nl}}$


Due to the security, $\rho_0$ and $\rho_1$ are computationally indistinguishable.

Finally, let us show that $\rho_0$ and $\rho_1$ are statistically distinguishable.
To show it, we use the following two lemmas.

\begin{lemma}
For each $x\in\bit^l$, let us define
\begin{eqnarray*}
S_x\coloneqq\Big\{k\in\bit^\secp~\Big|~\Pr[x\gets\Dec(k,\ct_{k,x})]\ge\frac{1}{2}\Big\}.
\end{eqnarray*}
Then, $\frac{|S_x|}{2^\secp}\ge\frac{1}{4}$ for any $x\in\bit^l$.
\end{lemma}

\begin{proof}
Assume that $\frac{|S_{x^*}|}{2^\secp}<\frac{1}{4}$ for a certain $x^*\in\bit^l$. Then,
\begin{eqnarray*}
\frac{1}{2^\secp}\sum_k\Pr[x^*\gets\Dec(k,\ct_{k,x^*})]
&=&
\frac{1}{2^\secp}\sum_{k\in S_{x^*}}\Pr[x^*\gets\Dec(k,\ct_{k,x^*})]\\
&&+\frac{1}{2^\secp}\sum_{k\notin S_{x^*}}\Pr[x^*\gets\Dec(k,\ct_{k,x^*})]\\
&\le&\frac{|S_{x^*}|}{2^\secp}+\frac{1}{2}\\
&\le&\frac{3}{4},
\end{eqnarray*}
which contradicts the correctness.
\end{proof}

\begin{lemma}
For each $x\in\bit^l$, define 
\begin{eqnarray*}
R_x\coloneqq\Big\{k\in\bit^\secp~\Big|~\Pr[x\gets\Dec(k,|\psi_1\rangle\otimes...\otimes|\psi_l\rangle):
|\psi_1\rangle,...,|\psi_l\rangle\gets\mu_n]\ge\frac{1}{2}\Big\}.
\end{eqnarray*}
Then, $|R_x|=0$ for at least one $x\in\bit^l$.
\end{lemma}

\begin{proof}
Assume that $|R_x|>0$ for all $x\in\bit^l$.
Then, the following protocol allows Alice to send her $l$-bit string to Bob
with probability at least $1/2$
by sending only $\secp$ bits ($\secp<l$), which is imformation theoretically impossible.
\begin{enumerate}
    \item 
    Alice gets an input $x\in\bit^l$.
    \item
    Because $|R_x|>0$, Alice can always choose $k\in R_x$. Alice sends it to Bob.
    \item
    Bob generates $|\psi_1\rangle,...,|\psi_l\rangle\gets\mu_n$ and runs
$\Dec(k,|\psi_1\rangle\otimes...\otimes|\psi_l\rangle)$. Let $x'$ be the output.
\item
Bob outputs $x'$.
\end{enumerate}
Then, for any $x\in\bit^l$,
the probability that Bob outputs $x$ is
at least $1/2$.
\end{proof}

\if0
\begin{lemma}\label{lemma:unbounded_algorithm2}
There is a (not necessarily polynomial-time) quantum algorithm $\cQ$ that, on input $T$ copies $\ct_{k,x}^{\otimes T}$ of $\ct_{k,x}$
with $T=\poly(\secp)$,
outputs $x^*(k,x)\in\bit^l$ and $k^*(k,x)\in\bit^\secp$ such that 
\begin{eqnarray*}
\Pr[x^*(k,x)\gets \Dec(k^*(k,x),\ct_{k,x})]\ge 
\Pr[x\gets \Dec(k,\ct_{k,x})]-\frac{1}{\poly(\secp)}
\end{eqnarray*}
with probability at least $1-2^{-\poly(\secp)}$.
\end{lemma}
\fi

Let $\Pi_{k,x}$ be a POVM element that corresponds to the accepting event in the following operation:
On input an $nl$-qubit state $\sigma$, run $x'\gets\Dec(k,\sigma)$. If $x'=x$, accept. Otherwise, reject.
In other words,
\begin{eqnarray*}
\mbox{Tr}(\Pi_{k,x}\sigma)=\Pr[x\gets\Dec(k,\sigma)].
\end{eqnarray*}
The following unbounded adversary $\cA$ can distinguish $\rho_0$ and $\rho_1$.
\begin{enumerate}
\item 
For $\{\Pi_{k',x'}\}_{k'\in\bit^\secp,x'\in\bit^l}$,
run the shadow tomography algorithm on input $\ct_{k,x}^{\otimes T}$.
The shadow tomography algorithm outputs $\{\eta_{k',x'}\}_{k'\in\bit^\secp,x'\in\bit^l}$ such that
$|\eta_{k',x'}-\mbox{Tr}(\Pi_{k',x'}\ct_{k,x})|\le\epsilon$ for each $k'\in\bit^\secp$
and each $x'\in\bit^l$
with probability at least $1-\delta$. 
\item
If there exists $k',x'$ such that
$\eta_{k',x'}\ge\frac{1}{2}$,
output 1. Otherwise, output 0.
\end{enumerate}

Then, 
\begin{eqnarray*}
\Pr[1\gets\cA(\rho_0)]
&\ge& (1-2^{-\poly(\secp)})\frac{1}{4}.
\end{eqnarray*}
On the other hand,
\begin{eqnarray*}
\Pr[1\gets\cA(\rho_1)]
&\le& \frac{1}{2}\frac{1}{2}-\frac{1}{\poly(\secp)}.
\end{eqnarray*}
\end{proof}


==> EFIfromOTP_IND.tex <==
\section{EFI pairs from quantum pseudo one-time pad}
\mor{This is correct. But a single-copy version was already shown by KaiMin et al.}
In this paper, we construct EFI pairs from quantum pseudo one-time pad.

Quantum pseudo one-time pad is defined as follows.
\begin{definition}[(IND-based) quantum pseudo one-time pad]
\label{def:OTP}
An (IND-based) quantum pseudo one-time pad scheme with the key length $\secp$ and
the plaintext length $l$ ($l>k$) is a tuple of algorithms $(\Enc,\Dec)$ such that
\begin{itemize}
    \item 
    $\Enc(k,x)\to\ct:$ It is a QPT algorithm that, on input a classical secret key $k\in\bit^\secp$ and 
    a classical plaintext message $x\in\bit^l$,
    outputs an $ln$-qubit quantum ciphertext $\ct$.
    \item
    $\Dec(\ct,k)\to x':$ It is a QPT algorithm that, on input $\ct$ and $k$, outputs $x'\in\bit^l$.
\end{itemize}
\paragraph{\bf Correctness:}
For any $x\in\bit^l$,
\begin{eqnarray*}
\Pr[x\gets\Dec(k,\ct):k\gets\bit^\secp,\ct\gets\Enc(k,x)]\ge1-\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For any $x_0,x_1\in\bit^l$, any (non-uniform) QPT adversary $\cA$, and any polynomial $t$,
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\ct_0^{\otimes t}):k\gets\bit^\secp,\ct_0\gets\Enc(k,x_0)]\\
&&-\Pr[1\gets\cA(\ct_1^{\otimes t}):k\gets\bit^\secp,\ct_1\gets\Enc(k,x_1)]|
\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{remark}
Note that the definition of security given in \cite{cryptoeprint:2021/1663} is different from the above one.
We consider the IND-based version of quantum pseudo one-time pad.
The security definition of \cite{cryptoeprint:2021/1663} is as follows:
For any $x\in\bit^l$, any (non-uniform) QPT adversary $\cA$, and any polynomial $t$,
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\ct^{\otimes t}):k\gets\bit^\secp,\ct\gets\Enc(k,x)]\\
&&-\Pr[1\gets\cA((|\psi_1\rangle\otimes...\otimes|\psi_l\rangle)^{\otimes t})
:|\psi_1\rangle,...,|\psi_l\rangle\gets\mu_n]|
\le\negl(\secp),
\end{eqnarray*}
where $|\psi\rangle\gets\mu_n$ means the Haar random sampling of $n$-qubit states.
However, it is clear that the secuity definition of \cite{cryptoeprint:2021/1663} implies
that of \cref{def:OTP}, and therefore if quantum pseudo one-time pad of \cite{cryptoeprint:2021/1663} exists,
that of \cref{def:OTP} exists.
\end{remark}


\mor{kokomade check ok}
\begin{theorem}
\label{theorem:OTP}
(IND-based) quantum pseudo one-time pad with $l-\secp\ge\log\poly(\secp)$ implies EFI pairs.
\end{theorem}

\begin{proof}
Let $\ct_{k,x}$ be the output of $\Enc(k,x)$.
We define an algorithm $\StateGen(1^\secp,b)$ that outputs
\begin{eqnarray*}
\rho_0\coloneqq\frac{1}{2^{\secp+l}}\sum_{k\in\bit^\secp,x\in\bit^l}|x\rangle\langle x|\otimes\ct_{k,x}^{\otimes T}
\end{eqnarray*}
if $b=0$, and
\begin{eqnarray*}
\rho_1\coloneqq\frac{1}{2^{\secp+2l}}\sum_{k\in\bit^\secp,x,x'\in\bit^l}|x\rangle\langle x|\otimes\ct_{k,x'}^{\otimes T}
\end{eqnarray*}
if $b=1$
as follows.
(Here, $T$ is a certain polynomial of $\secp$ specified later.)
When $b=0$, $\StateGen$ runs as follows.
\begin{enumerate}
    \item Generate $\frac{1}{2^{\secp+l}}\sum_{k,x}|k\rangle\langle k|\otimes |x\rangle\langle x|$.
    \item 
    Run $\Enc$ $T$ times:
    $\frac{1}{2^{\secp+l}}\sum_{k,x}|k\rangle\langle k|\otimes |x\rangle\langle x|\otimes \ct_{k,x}^{\otimes T}$.
    \item
    Trace out the $|k\rangle$ register:
    $\frac{1}{2^{\secp+l}}\sum_{k,x}|x\rangle\langle x|\otimes \ct_{k,x}^{\otimes T}$.
\end{enumerate}
When $b=1$, $\StateGen$ runs as follows.
\begin{enumerate}
    \item Generate $\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}|k\rangle\langle k|\otimes |x\rangle\langle x|\otimes|x'\rangle\langle x'|$.
    \item 
    Run $\Enc$ $T$ times:
    $\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}|k\rangle\langle k|\otimes |x\rangle\langle x|\otimes|x'\rangle\langle x'|\otimes
    \ct_{k,x'}^{\otimes T}$.
    \item
    Trace out the $|k\rangle$ register and the $|x'\rangle$ register:
    $\frac{1}{2^{\secp+2l}}\sum_{k,x,x'} |x\rangle\langle x|\otimes
    \ct_{k,x'}^{\otimes T}$.
\end{enumerate}
It is clear that thus defined $\StateGen$ is QPT.

Due to the security, $\rho_0$ and $\rho_1$ are computationally indistinguishable.

Finally, let us show that $\rho_0$ and $\rho_1$ are statistically distinguishable.
Let $\Pi_k$ be a POVM element that corresponds to the accepting event in the following operation:
On input a state $|x\rangle\langle x|\otimes\sigma$, run 
$x'\gets\Dec(k,\sigma)$. If $x'=x$, accept. Otherwise, reject.
In other words,
\begin{eqnarray*}
\mbox{Tr}[\Pi_k(|x\rangle\langle x|\otimes \sigma)]=\Pr[x\gets\Dec(k,\sigma)].
\end{eqnarray*}
The following unbounded adversary $\cA$ can distinguish $\rho_0$ and $\rho_1$.
\begin{enumerate}
\item 
For $\{\Pi_{k'}\}_{k'\in\bit^\secp}$,
run the shadow tomography algorithm on input 
$|x\rangle\langle x|\otimes \sigma$, where
$\sigma=\ct_{k,x}^{\otimes T}$ (when $b=0$)
and $\sigma=\ct_{k,x'}^{\otimes T}$ (when $b=1$).
The shadow tomography algorithm outputs 
$\{\eta_{k'}\}_{k'\in\bit^\secp}$ such that
\begin{eqnarray*}
|\eta_{k'}-\mbox{Tr}[\Pi_{k'}(|x\rangle\langle x|\otimes\sigma)]|\le\epsilon
\end{eqnarray*}
for each $k'\in\bit^\secp$
with probability at least $1-\delta$. 
In other words,
the shadow tomography algorithm outputs 
$\{\eta_{k'}\}_{k'\in\bit^\secp}$ such that
\begin{eqnarray*}
|\eta_{k'}-\Pr[x\gets\Dec(k',\sigma)]|\le\epsilon
\end{eqnarray*}
for each $k'\in\bit^\secp$
with probability at least $1-\delta$. 
\item
Find
$k^*\coloneqq\arg\max_{k'}\{\eta_{k'}\}_{k'\in\bit^\secp}$.
(Note that $k^*$ depends on $k,x,x'$.)
Output 1 with probability $\min(\eta_{k^*},1)$.
\end{enumerate}
Then
\begin{eqnarray*}
\Pr[1\gets \cA(\rho_0)]&=&
\frac{1}{2^{\secp+l}}\sum_{k,x}\Pr[1\gets\cA(|x\rangle\langle x|\otimes\ct_{k,x}^{\otimes T})]\\
&\ge&(1-\delta)\frac{1}{2^{\secp+l}}\sum_{k,x}\eta_{k^*}\\
&\ge&(1-\delta)\frac{1}{2^{\secp+l}}\sum_{k,x}\eta_k\\
&\ge&(1-\delta)\frac{1}{2^{\secp+l}}\sum_{k,x}\Big(\Pr[x\gets\Dec(k,\ct_{k,x})]-\epsilon\Big)\\
&\ge&(1-\delta)(1-\negl(\secp)-\epsilon)\\
&\ge&1-\frac{1}{\poly(\secp)}.
\end{eqnarray*}
On the other hand, let $p_{st}$ be the success probability of the shadow tomography algorithm.
Then,
\begin{eqnarray*}
\Pr[1\gets\cA(\rho_1)]&=&
\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}\Pr[1\gets\cA(|x\rangle\langle x|\otimes\ct_{k,x'}^{\otimes T})]\\
&\le&\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}(p_{st}\eta_{k^*}+(1-p_{st}))\\
&\le&\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}\eta_{k^*}+\delta\\
&\le&\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}\Big(\Pr[x\gets\Dec(k^*,\ct_{k,x'})]+\epsilon\Big)+\delta\\
&=&\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}\Pr[x\gets\Dec(k^*,\ct_{k,x'})]+\epsilon+\delta\\
&\le&\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}\sum_{k'}\Pr[x\gets\Dec(k',\ct_{k,x'})]+\epsilon+\delta\\
&=&\frac{2^\secp}{2^l}\sum_x\Big(
\frac{1}{2^{2\secp+l}}\sum_{k,k',x'}\Pr[x\gets\Dec(k',\ct_{k,x'})]\Big)+\epsilon+\delta\\
&\le&\frac{2^\secp}{2^l}\sum_x\frac{1}{2^{l}}+\epsilon+\delta\\
&=&\frac{2^\secp}{2^l}+\epsilon+\delta\\
&\le&\frac{1}{\poly(\secp)}.
\end{eqnarray*}
\end{proof}


==> EFIfromOTP_IND_singlecopy.tex <==
\section{EFI pairs from single-copy-secure quantum pseudo one-time pad}
\mor{mikansei. Anyway it was shown by KaiMin}
In this paper, we construct EFI pairs from single-copy-secure quantum pseudo one-time pad.

Single-copy-secure quantum pseudo one-time pad is defined as follows.
\begin{definition}[(IND-based) single-copy-secure quantum pseudo one-time pad]
\label{def:OTP}
An (IND-based) quantum pseudo one-time pad scheme with the key length $\secp$ and
the plaintext length $l$ ($l>k$) is a tuple of algorithms $(\Enc,\Dec)$ such that
\begin{itemize}
    \item 
    $\Enc(k,x)\to\ct:$ It is a QPT algorithm that, on input a classical secret key $k\in\bit^\secp$ and 
    a classical plaintext message $x\in\bit^l$,
    outputs an $ln$-qubit quantum ciphertext $\ct$.
    \item
    $\Dec(\ct,k)\to x':$ It is a QPT algorithm that, on input $\ct$ and $k$, outputs $x'\in\bit^l$.
\end{itemize}
\paragraph{\bf Correctness:}
For any $x\in\bit^l$,
\begin{eqnarray*}
\Pr[x\gets\Dec(k,\ct):k\gets\bit^\secp,\ct\gets\Enc(k,x)]\ge1-\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For any $x_0,x_1\in\bit^l$, any (non-uniform) QPT adversary $\cA$, and any polynomial $t$,
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\ct_0):k\gets\bit^\secp,\ct_0\gets\Enc(k,x_0)]\\
&&-\Pr[1\gets\cA(\ct_1):k\gets\bit^\secp,\ct_1\gets\Enc(k,x_1)]|
\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{remark}
Note that the definition of security given in \cite{cryptoeprint:2021/1663} is different from the above one
in the following two points.
First, we consider the security against adversaries who can have only a single copy of $\ct$, while
they consider the security against adversaries who can have polynomially many copies of $\ct$.
Second,
we consider the IND-based version of quantum pseudo one-time pad.
The security definition of \cite{cryptoeprint:2021/1663} is as follows:
For any $x\in\bit^l$, any (non-uniform) QPT adversary $\cA$, and any polynomial $t$,
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\ct^{\otimes t}):k\gets\bit^\secp,\ct\gets\Enc(k,x)]\\
&&-\Pr[1\gets\cA((|\psi_1\rangle\otimes...\otimes|\psi_l\rangle)^{\otimes t})
:|\psi_1\rangle,...,|\psi_l\rangle\gets\mu_n]|
\le\negl(\secp),
\end{eqnarray*}
where $|\psi\rangle\gets\mu_n$ means the Haar random sampling of $n$-qubit states.
However, it is clear that the security definition of \cite{cryptoeprint:2021/1663} implies
that of \cref{def:OTP}, and therefore if quantum pseudo one-time pad of \cite{cryptoeprint:2021/1663} exists,
that of \cref{def:OTP} exists.
\end{remark}


\begin{theorem}
\label{theorem:OTP}
(IND-based) single-copy-secure quantum pseudo one-time pad with implies EFI pairs.
\end{theorem}

\begin{proof}
Let $\ct_{k,x}$ be the output of $\Enc(k,x)$.
We define an algorithm $\StateGen(1^\secp,b)$ that outputs
\begin{eqnarray*}
\rho_0\coloneqq\frac{1}{2^{\secp+l}}\sum_{k\in\bit^\secp,x\in\bit^l}|x\rangle\langle x|\otimes\ct_{k,x}
\end{eqnarray*}
if $b=0$, and
\begin{eqnarray*}
\rho_1\coloneqq\frac{1}{2^{\secp+2l}}\sum_{k\in\bit^\secp,x,x'\in\bit^l}|x\rangle\langle x|\otimes\ct_{k,x'}
\end{eqnarray*}
if $b=1$
as follows.
When $b=0$, $\StateGen$ runs as follows.
\begin{enumerate}
    \item Generate $\frac{1}{2^{\secp+l}}\sum_{k,x}|k\rangle\langle k|\otimes |x\rangle\langle x|$.
    \item 
    Run $\Enc$:
    $\frac{1}{2^{\secp+l}}\sum_{k,x}|k\rangle\langle k|\otimes |x\rangle\langle x|\otimes \ct_{k,x}$.
    \item
    Trace out the $|k\rangle$ register:
    $\frac{1}{2^{\secp+l}}\sum_{k,x}|x\rangle\langle x|\otimes \ct_{k,x}$.
\end{enumerate}
When $b=1$, $\StateGen$ runs as follows.
\begin{enumerate}
    \item Generate $\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}|k\rangle\langle k|\otimes |x\rangle\langle x|\otimes|x'\rangle\langle x'|$.
    \item 
    Run $\Enc$:
    $\frac{1}{2^{\secp+2l}}\sum_{k,x,x'}|k\rangle\langle k|\otimes |x\rangle\langle x|\otimes|x'\rangle\langle x'|\otimes
    \ct_{k,x'}$.
    \item
    Trace out the $|k\rangle$ register and the $|x'\rangle$ register:
    $\frac{1}{2^{\secp+2l}}\sum_{k,x,x'} |x\rangle\langle x|\otimes
    \ct_{k,x'}$.
\end{enumerate}
It is clear that thus defined $\StateGen$ is QPT.

Due to the security, $\rho_0$ and $\rho_1$ are computationally indistinguishable.

Finally, let us show that $\rho_0$ and $\rho_1$ are statistically distinguishable.
Let $\Pi_k$ be a POVM element that corresponds to the accepting event in the following operation:
On input a state $|x\rangle\langle x|\otimes\sigma$, run 
$x'\gets\Dec(k,\sigma)$. If $x'=x$, accept. Otherwise, reject.
In other words,
\begin{eqnarray*}
\mbox{Tr}[\Pi_k(|x\rangle\langle x|\otimes \sigma)]=\Pr[x\gets\Dec(k,\sigma)].
\end{eqnarray*}
The unbounded adversary $\cA$ who runs the algorithm of \cref{theorem:HLM17} can distinguish $\rho_0$ and $\rho_1$.
Let us first show a lowerbound of $\Pr[1\gets\cA(\rho_0)]$.
Fix a parameter $\epsilon<\frac{1}{2}$.
For each $x\in\bit^l$,
define the set
\begin{eqnarray*}
S_x\coloneqq\{k\in\bit^\secp~|~\mbox{Tr}(\Pi_k|x\rangle\langle x|\otimes\ct_{k,x})\ge \epsilon\}.
\end{eqnarray*}
Then, for any $x\in\bit^l$, $\frac{|S_x|}{2^\secp}\ge1-\epsilon-\negl(\secp)$.
In fact, assume that $\frac{|S_x|}{2^\secp}<1-\epsilon-\frac{1}{p}$ for an $x\in\bit^\secp$ and a polynomial $p$. Then,
for that $x$,
\begin{eqnarray*}
\frac{1}{2^\secp}\sum_{k\in\bit^\secp}\Pr[x\gets\Dec(k,\ct_{k,x})]&=&
\frac{1}{2^\secp}\sum_{k\in\bit^\secp}\mbox{Tr}[\Pi_k|x\rangle\langle x|\otimes \ct_{k,x}]\\
&=&
\frac{1}{2^\secp}\sum_{k\in S_x}\mbox{Tr}[\Pi_k|x\rangle\langle x|\otimes \ct_{k,x}]\\
&&+\frac{1}{2^\secp}\sum_{k\notin S_x}\mbox{Tr}[\Pi_k|x\rangle\langle x|\otimes \ct_{k,x}]\\
&<&
\frac{|S_x|}{2^\secp}
+
\epsilon\\
&<&1-\frac{1}{p},
\end{eqnarray*}
which contradicts the correctness.
Therefore,
\begin{eqnarray*}
\Pr[1\gets\cA(\rho_0)]&=&\frac{1}{2^l}\sum_{x\in\bit^l}\frac{1}{2^\secp}\sum_{k\in\bit^\secp}\Pr[1\gets \cA(|x\rangle\langle x|\otimes \ct_{k,x})]\\
&\ge&\frac{1}{2^l}\sum_{x\in\bit^l}\frac{1}{2^\secp}\sum_{k\in S_x}\Pr[1\gets \cA(|x\rangle\langle x|\otimes \ct_{k,x})]\\
&\ge&\frac{1}{2^l}\sum_{x\in\bit^l}\frac{1}{2^\secp}\sum_{k\in S_x}\frac{(1-\epsilon)^2}{7}\\
&\ge&\frac{(1-\epsilon)^3}{7}-\negl(\secp).
\end{eqnarray*}

Next let us show an upperbound of $\Pr[1\gets\cA(\rho_1)]$.
Note that
\begin{eqnarray*}
\frac{1}{2^\secp}\sum_{k'}\mbox{Tr}(\Pi_{k'}\rho_1)&=&
\frac{1}{2^{2\secp+2l}}\sum_{x,x',k,k'}\mbox{Tr}(\Pi_{k'}|x\rangle\langle x|\otimes \ct_{k,x'})\\
&=&
\frac{1}{2^l}\sum_{x}\Big[\frac{1}{2^{2\secp+l}}\sum_{x',k,k'}\Pr[x\gets \Dec(k',\ct_{k,x'})]\Big]\\
&\le&
\frac{1}{2^l}\sum_{x}\frac{1}{2^l}\\
&=&
\frac{1}{2^l}.
\end{eqnarray*}
Therefore,
\begin{eqnarray*}
\Pr[1\gets\cA(\rho_1)]&\le&4\times2^{-l}2^\secp.
\end{eqnarray*}

If
\begin{eqnarray*}
\secp\le l+\log\Big(\frac{1}{56}-\frac{1}{\poly(\secp)}\Big)-2,
\end{eqnarray*}
the statistical distinguishability of $\rho_0$ and $\rho_1$ is obtained.
\end{proof}


==> EFIfromOWSG.tex <==
\section{EFI pairs from one-way states generators}
\mor{Exponential security is required}


\begin{definition}[One-way states generators (OWSGs)\cite{cryptoeprint:2021/1691}]
\label{def:OWSG}
Let $\StateGen$ be a QPT algorithm that, on input $k\in\bit^\secp$, outputs an $m$-qubit quantum state $|\phi_k\rangle$.
Let us consider the following security game, $\mathsf{Exp}$, between a challenger $\cC$
and a QPT adversary $\cA$:
\begin{enumerate}
\item
$\cC$ chooses $k\leftarrow\bit^\secp$.
\item
$\cC$ runs $|\phi_k\rangle\leftarrow G(k)$ $t+1$ times.
\item
$\cC$ sends $|\phi_k\rangle^{\otimes t}$ to $\cA$.
\item
$\cA$ sends $k'\in\bit^\secp$ to $\cC$. 
\item
$\cC$ measures $|\phi_k\rangle$ with $\{|\phi_{k'}\rangle\langle\phi_{k'}|,I-|\phi_{k'}\rangle\langle\phi_{k'}|\}$.
If the result is $|\phi_{k'}\rangle\langle\phi_{k'}|$, the output of the experiment is 1.
Otherwise, the output of the experiment is 0.
\end{enumerate}
We say that $\StateGen$ is a one-way states generator (OWSG) if
for any $t=\poly(\secp)$ and any QPT adversary $\cA$ there exists a negligible function $\negl$ such that
\begin{eqnarray*}
\Pr[\mathsf{Exp}=1]\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\if0
In this paper, we consider a weaker version of it.
\begin{definition}[Simpler OWSGs (SOWSGs)]
\label{def:SOWSG}
Let $\StateGen$ be a QPT algorithm that, on input $k\in\bit^\secp$, outputs an $m$-qubit quantum state $|\phi_k\rangle$.
We say that $\StateGen$ is a simpler one-way state generator if
for any $t=\poly(\secp)$ and any QPT adversary $\cA$ there exists a negligible function $\negl$ such that
\begin{eqnarray*}
\Pr[k\gets\cA(|\phi_k\rangle^{\otimes t}):k\gets\bit^\secp,|\phi_k\rangle\gets G(k)]\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{remark}
It is clear that OWSGs imply SOWSGs, but the inverse would not hold.
Moreover, OWSGs imply one-time quantum digital signatures~\cite{cryptoeprint:2021/1691}, but SOWSGs will not.
\end{remark}
\fi

We use the following result by Harrow, Lin, and Montanaro.
\begin{theorem}[\cite{HLM17}]
\label{theorem:HLM17}
Let $\Lambda_1,...,\Lambda_n$ be projectors.
Fix parameters $\epsilon<\frac{1}{2}$ and $\delta$.
Let $\rho$ be a state such that either there exists $i$ such that
$\mbox{Tr}(\Lambda_i\rho)\ge1-\epsilon$,
or
$\frac{1}{n}\sum_{j=1}^n\mbox{Tr}(\Lambda_j \rho)\le\delta$.
Then there is an algorithm that uses a single copy of $\rho$ and in the former case
accepts with probability at least $(1-\epsilon)^2/7$
and in the latter case accepts with probability at most $4\delta n$.
\end{theorem}

\begin{theorem}
If OWSGs exist, then EFI pairs exist.
\end{theorem}

\begin{proof}
Let $\mathsf{OWSG}.\StateGen(k)\to|\phi_k\rangle$ be a OWSG,
where $k\in\bit^\secp$ and $|\phi_k\rangle$ is an $m$-qubit state.
For each $b\in\bit$ and $k\in\bit^\secp$, define
\begin{eqnarray*}
|\Psi_k^b\rangle\coloneqq\frac{1}{\sqrt{2}}(|0\rangle|k0^{tm-\secp}\rangle+(-1)^b|1\rangle|\phi_k^{\otimes t}\rangle).
\end{eqnarray*}

We construct an EFI pair $\mathsf{EFI}.\StateGen(b,1^\secp)\to\rho_b$ with
\begin{eqnarray*}
\rho_b&\coloneqq&\frac{1}{2^\secp}\sum_{k\in\bit^\secp}|\Psi_k^b\rangle\langle\Psi_k^b|,
\end{eqnarray*}
as follows.
\mor{For simplicity, we assume that $\mathsf{SOWSG}$ runs as $U_k|0...0\rangle=|\phi_k\rangle$, i.e., no ancilla outputs exist. A generalization to $U_k|0...0\rangle=|\phi_k\rangle|junk_k\rangle$ is easy.}
\begin{enumerate}
    \item Prepare 
   \begin{eqnarray*} 
    \frac{1}{\sqrt{2^\secp}}\sum_{k\in\bit^\secp}|k\rangle\otimes\frac{1}{\sqrt{2}}(|0\rangle|0^{tm}\rangle+(-1)^b|1\rangle|0^{tm}\rangle).
   \end{eqnarray*} 
    \item Copy the content of the first register to the third register if the second register is 0:
    \begin{eqnarray*}
    \frac{1}{\sqrt{2^\secp}}\sum_{k\in\bit^\secp}|k\rangle\otimes\frac{1}{\sqrt{2}}(|0\rangle|k0^{tm-\secp}\rangle+(-1)^b|1\rangle|0^{tm}\rangle).
    \end{eqnarray*}
    \item Run $\mathsf{OWSG}.\StateGen$ $t$ times on the first and third registers if the second register is 1:
    \begin{eqnarray*}
&&    \frac{1}{\sqrt{2^\secp}}\sum_{k\in\bit^\secp}|k\rangle\otimes\frac{1}{\sqrt{2}}(|0\rangle|k0^{tm-\secp}\rangle+(-1)^b|1\rangle|\phi_k\rangle^{\otimes t})\\
    &=&\frac{1}{\sqrt{2^\secp}}\sum_{k\in\bit^\secp}|k\rangle\otimes|\Psi_k^b\rangle.
    \end{eqnarray*}
    \item
    Trace out the first register:
    \begin{eqnarray*}
    \frac{1}{2^\secp}\sum_{k\in\bit^\secp}|\Psi_k^b\rangle\langle\Psi_k^b|=\rho_b.
    \end{eqnarray*}
    Output this state.
\end{enumerate}
It is clear that this algorithm is QPT.

\paragraph{\bf Computational indistinguishability.}
We next show that $\rho_0$ and $\rho_1$ are computationally indistinguishable.
To show it, we use the following lemma, whose proof is given later.
\begin{lemma}
\label{lem:OWSG}
If there exists a (non-uniform) QPT adversary $\cA$ such that
\begin{eqnarray*}
|\Pr[1\gets\cA(|\Psi_k^0\rangle)]-\Pr[1\gets\cA(|\Psi_k^1\rangle)]|\ge\Delta
\end{eqnarray*}
with a non-negligible $\Delta$ for all $k\in S$ in a set $S\subseteq\bit^\secp$,
then there exists a (non-uniform) QPT adversary $\cB$ such that
\begin{eqnarray*}
\Pr[k\gets\cB(|\phi_k\rangle^{\otimes t})]\ge\Delta^2
\end{eqnarray*}
for all $k\in S$.
\end{lemma}

Assume that there exists a QPT adversary $\cA$ and a polynomial $p$ such that
\begin{eqnarray*}
|\Pr[1\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\ge\frac{1}{p}.
\end{eqnarray*}
Define
\begin{eqnarray*}
S\coloneqq\Big\{k\in\bit^\secp~\Big|~|\Pr[1\gets\cA(|\Psi_k^0\rangle)]-\Pr[1\gets\cA(|\Psi_k^1\rangle)]|\ge\frac{1}{2p}\Big\}.
\end{eqnarray*}
Then, $\frac{|S|}{2^\secp}\ge\frac{1}{2p}$,
because otherwise,
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\\
&\le&
\frac{1}{2^\secp}\sum_{k\in\bit^\secp}|\Pr[1\gets\cA(|\Psi_k^0\rangle)]-\Pr[1\gets\cA(|\Psi_k^1\rangle)]|\\
&=&
\frac{1}{2^\secp}\sum_{k\in S}|\Pr[1\gets\cA(|\Psi_k^0\rangle)]-\Pr[1\gets\cA(|\Psi_k^1\rangle)]|\\
&&+\frac{1}{2^\secp}\sum_{k\notin S}|\Pr[1\gets\cA(|\Psi_k^0\rangle)]-\Pr[1\gets\cA(|\Psi_k^1\rangle)]|\\
&<&
\frac{|S|}{2^\secp}+\frac{1}{2p}\\
&<&\frac{1}{p},
\end{eqnarray*}
which is the contradiction.

Then, by using \cref{lem:OWSG},
\begin{eqnarray*}
&&\Pr[k\gets\cB(|\phi_k\rangle^{\otimes t};|\tau\rangle):k\gets\bit^\secp]\\
&=&
\frac{1}{2^\secp}\sum_{k\in\bit^\secp}\Pr[k\gets\cB(|\phi_k\rangle^{\otimes t};|\tau\rangle)]\\
&\ge&\frac{1}{2^\secp}\sum_{k\in S}\Pr[k\gets\cB(|\phi_k\rangle^{\otimes t};|\tau\rangle)]\\
&\ge&\frac{1}{2p}\frac{1}{4p^2},
\end{eqnarray*}
which breaks the security of the OWSG.
Hence the computational indistinguishability of $\rho_0$ and $\rho_1$ is shown.

\begin{proof}[Proof of \cref{lem:OWSG}]
Assume that 
there exists a (non-uniform) QPT adversary $\cA$ such that
\begin{eqnarray*}
|\Pr[1\gets\cA(|\Psi_k^0\rangle)]
-\Pr[1\gets\cA(|\Psi_k^1\rangle)]|\ge\Delta
\end{eqnarray*}
with a non-negligible $\Delta$ for all $k\in S$ in a set $S\subseteq\bit^\secp$.
Note that $\langle\Psi_k^0|\Psi_k^1\rangle=0$ for all $k\in\bit^\secp$.
Therefore, due to \cite{HMY22}, there exists a QPT unitary $U$ and a $\poly(\secp)$-qubit state $|\tau\rangle$ (quantum advice) such that
    \begin{align*}
        \frac{|\bra{y}\bra{\tau}U\ket{x}\ket{\tau}+\bra{x}\bra{\tau}U\ket{y}\ket{\tau}|}{2}\ge\Delta,
    \end{align*}
    where 
    \begin{eqnarray*}
    |x\rangle&\coloneqq&\frac{|\Psi_k^0\rangle+|\Psi_k^1\rangle}{\sqrt{2}}=|0\rangle|k0^{tm-\secp}\rangle,\\
    |y\rangle&\coloneqq&\frac{|\Psi_k^0\rangle-|\Psi_k^1\rangle}{\sqrt{2}}=|1\rangle|\phi_k\rangle^{\otimes t}.
    \end{eqnarray*}
    It means that
        $|\bra{y}\bra{\tau}U\ket{x}\ket{\tau}|\ge\Delta$ or
        $|\bra{x}\bra{\tau}U\ket{y}\ket{\tau}|\ge\Delta$.
        Without loss of generality, we can assume the latter case, i.e., 
        \begin{eqnarray*}
        |\bra{0}\bra{k0^{tm-\secp}}\bra{\tau}U\ket{1}\ket{\phi_k}^{\otimes t}\ket{\tau}|\ge\Delta.
        \end{eqnarray*}
        (In the former case, we have
        $|\bra{0}\bra{k0^{tm-\secp}}\bra{\tau}U^\dagger\ket{1}\ket{\phi_k}^{\otimes t}\ket{\tau}|\ge\Delta$, and therefore
        we can use $U^\dagger$ instead of $U$ in the following argument.)
       With $U$ (or $U^\dagger$), we can construct the following QPT adversary $\cB$.
       \begin{enumerate}
           \item 
           On input $|\phi_k\rangle^{\otimes t}$, add $\ket{1}$ and $\ket{\tau}$: $|1\rangle|\phi_k\rangle^{\otimes t}\ket{\tau}$.
           \item
           Apply $U$ (or $U^\dagger$):
           $U(|1\rangle|\phi_k\rangle^{\otimes t}\ket{\tau})$.
           \item
           Measure the first $\secp$ qubits of the second register in the computational basis, and output the measurement result.
       \end{enumerate}
       Then, for all $k\in S$,
       \begin{eqnarray*}
       \Pr[k\gets\cB(|\phi_k\rangle^{\otimes t};|\tau\rangle)]
       &=& \|(I\otimes |k\rangle\langle k|\otimes I)U(|1\rangle|\phi_k\rangle^{\otimes t}\ket{\tau})\|^2\\
       &\ge& |(\bra{0}\bra{k0^{tm-\secp}}\bra{\tau})U(|1\rangle|\phi_k\rangle^{\otimes t}\ket{\tau})|^2\\
       &\ge& \Delta^2.
       \end{eqnarray*}
\end{proof}       
       
       \paragraph{\bf Statistical distinguishability.}
      Finally, we show the statistical distinguishability of $\rho_0$ and $\rho_1$. 
      For each $k\in\bit^\secp$, define the projection operator $\Pi_k\coloneqq|\Psi_k^0\rangle\langle\Psi_k^0|$.
      We show that an unbounded adversary $\cA$ who, on input $|\Psi_k^b\rangle$, runs the algorithm of \cref{theorem:HLM17} 
      with $\{\Pi_k\}_{k\in\bit^\secp}$ can distinguish $\rho_0$ and $\rho_1$.
      
      First we show a lowerbound of $\Pr[1\gets\cA(\rho_0)]$. Note that, for any $k\in\bit^\secp$, there exists
      $k'$ such that $\mbox{Tr}(\Pi_{k'}|\Psi_k^0\rangle\langle\Psi_k^0|)=1$. (In fact, we have only to take $k'=k$.)
      Therefore, from \cref{theorem:HLM17},
      \begin{eqnarray*}
      \Pr[1\gets\cA(\rho_0)]&=&\frac{1}{2^\secp}\sum_{k\in\bit^\secp}\Pr[1\gets\cA(|\Psi_k^0\rangle)]\\
      &\ge&\frac{1}{7}.
      \end{eqnarray*}
      
Next we show an upperbound of $\Pr[1\gets\cA(\rho_1)]$.
     For that goal, consider a QPT adversary of OWSGs that uniformly randomly returns $k'\in\bit^\secp$. Its success probability is
     \begin{eqnarray*} 
     \frac{1}{2^\secp}\sum_k\frac{1}{2^\secp}\sum_{k'}|\langle\phi_{k'}|\phi_k\rangle|^2
&\ge&     \frac{1}{2^\secp}\sum_k\frac{1}{2^\secp}\sum_{k'\neq k}|\langle\phi_{k'}|\phi_k\rangle|^2\\
&=&     \frac{1}{2^\secp}\sum_k\Big[\frac{4}{2^\secp}\sum_{k'\in\bit^\secp}\mbox{Tr}(\Pi_{k'}|\Psi_k^1\rangle\langle\Psi_k^1|)\Big]\\
&=&4 \times    \frac{1}{2^\secp}\sum_{k'\in\bit^\secp}\mbox{Tr}(\Pi_{k'}\frac{1}{2^\secp}\sum_k|\Psi_k^1\rangle\langle\Psi_k^1|)\\
&=&4 \times    \frac{1}{2^\secp}\sum_{k'\in\bit^\secp}\mbox{Tr}(\Pi_{k'}\rho_1)\coloneqq4\delta.
     \end{eqnarray*} 
     Then due to the (exponential) security of OWSG, the left-hand-side has to be smaller than $\frac{1}{7}2^{-\secp}$.
     Therefore, $4\delta<\frac{1}{7}2^{-\secp}$ must be satisfied.
     Then, from \cref{theorem:HLM17},
           \begin{eqnarray*}
      \Pr[1\gets\cA(\rho_1)] &\le&4\delta 2^{\secp}<\frac{1}{7}.
      \end{eqnarray*}
      \end{proof}
      
     
      



==> EFIfromPKE.tex <==
\section{EFI pairs from quantum PKE}
\mor{This is correct, but single-copy QPOTP version was already shown
by KaiMin et al.}
In this appendix, we construct EFI from quantum PKE.

Quantum PKE is defined as follows.
\begin{definition}[Quantum PKE]
A quantum PKE scheme is a tuple of algorithms $(\Gen_1,\Gen_2,\Enc,\Dec)$ such that
\begin{itemize}
    \item 
    $\Gen_1(1^\secp)\to\sk:$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs
    a classical secret key $\sk$.
    \item
    $\Gen_2(\sk)\to\pk:$
    It is a QPT algorithm that, on input $\sk$, outputs
    a quantum public key $\pk$.
    \item
    $\Enc(x,\pk)\to\ct:$
    It is a QPT algorithm that, on input a message $x\in\bit^l$ and $\pk$, outputs
    a quantum ciphertext $\ct$.
    \item
    $\Dec(\sk,\ct)\to x':$
    It is a QPT algorithm that, on input $\sk$ and $\ct$, outputs $x'\in\bit^l$.
\end{itemize}
\paragraph{\bf Correctness:}
For any $x\in\bit^l$,
\begin{eqnarray*}
\Pr[x\gets\Dec(\ct,\sk):\sk\gets\Gen_1(1^\secp),\pk\gets\Gen_2(\sk),\ct\gets\Enc(\pk,x)]
\ge1-\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For any $x_0,x_1\in\bit^l$, any QPT adversary $\cA$, and any polynomial $t$,
\begin{eqnarray*}
&&|\Pr[1\gets \cA(\pk^{\otimes t},\ct_0):\sk\gets\Gen_1(1^\secp),\pk\gets\Gen_2(\sk),\ct_0\gets\Enc(\pk,x_0)]\\
&&-\Pr[1\gets \cA(\pk^{\otimes t},\ct_1):\sk\gets\Gen_1(1^\secp),\pk\gets\Gen_2(\sk),\ct_1\gets\Enc(\pk,x_1)]|
\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{remark}
Note that the security is defined for adversaries that can have only a single copy of $\ct$.
It is not known whether such a single-copy-ciphertext-secure quantum PKE implies
quantum pseudo one-time pad (\cref{def:OTP}), which assumes the security against adversaries
that can have polynomially many $\ct$.
However, interestingly, as we will see below, EFI pairs can be constructed from 
single-copy-ciphertext-secure quantum PKE.
\end{remark}

\begin{theorem}
If quantum PKE exists then EFI pairs exist.
\end{theorem}

\begin{proof}
Let us take the plaintext length $l$ be 1.
Let $\pk(\sk)$ be the output of $\Gen_2(\sk)$, 
and $\ct_{b,\pk(\sk)}$ be the output of $\Enc(b,\pk(\sk))$ for $b\in\bit$.
Define an algorithm $\StateGen(1^\secp,b)$ that outputs
\begin{eqnarray*}
\rho_b\coloneqq \sum_{\sk}\Pr[\sk\gets\Gen_1(1^\secp)]
\pk(\sk)^{\otimes T}\otimes \ct_{b,\pk(\sk)}
\end{eqnarray*}
as follows. (Here, $T$ is a certain polynomial of $\secp$ specified later.)
\begin{enumerate}
    \item 
    Run $\Gen_1$ to generate
    $\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\lambda)]|\sk\rangle\langle\sk|$.
    \item
    Copy the register:
    $\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\lambda)]|\sk\rangle\langle\sk|^{\otimes T+1}$.
    \item
    Run $\Gen_2$ $T+1$ times:
    $\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\lambda)] \pk(\sk)^{\otimes T+1}$.
    \item
    Add the register $|b\rangle\langle b|:$
    $\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\lambda)] \pk(\sk)^{\otimes T+1}\otimes|b\rangle\langle b|$.
    \item
    Run $\Enc$:
    $\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\lambda)]\pk(\sk)^{\otimes T}\otimes\ct_{b,\pk(\sk)}$.
    Output this state.
\end{enumerate}
It is clear that thus defined $\StateGen$ is QPT.

Moreover, $\rho_b$ is exactly a state that the adversary of quantum PKE receives when $b$ is encrypted.
Therefore, due to the security, 
\begin{eqnarray*}
|\Pr[1\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\le\negl(\secp)
\end{eqnarray*}
for any QPT adversary $\cA$.

Finally, let us show that $\rho_0$ and $\rho_1$ are statistically distinguishable.
To show it, we use the following lemma whose proof is given later.
\begin{lemma}\label{lemma:unbounded_algorithm}
There is a (not necessarily polynomial-time) quantum algorithm $\cQ$ that, on input $T$ copies $\pk(\sk)^{\otimes T}$ of $\pk(\sk)$
with 
$T=\poly(\secp)$,
outputs $\sk^*(\sk)$ such that 
\begin{eqnarray*}
\Pr[b\gets \Dec(\sk^*(\sk),\ct_{b,\pk(\sk)})]\ge \frac{2}{3}-\frac{1}{\poly(\secp)}
\end{eqnarray*}
for both $b\in\bit$ with probability at least $1-2^{-\poly(\secp)}$.
\end{lemma}


The following unbounded adversary $\cA$ can distinguish $\rho_0$ and $\rho_1$.
\begin{enumerate}
    \item 
Apply $\cQ$ on $\rho_b$ to get
\begin{eqnarray*}
\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\secp)]
\otimes|\sk^*(\sk)\rangle\langle\sk^*(\sk)|\otimes \ct_{b,\pk(\sk)}
\end{eqnarray*}
with probability at least $1-2^{-\poly(\secp)}$.
\item
Run $\Dec$ on it. Let $b'\in\bit$ be the output of $\Dec$.
Output $b'$.
\end{enumerate}
It is clear that
\begin{eqnarray*}
\Pr[b\gets\cA(\rho_b)]
&\ge&
(1-2^{-\poly(\secp)})
\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\secp)]
\Pr[b\gets\Dec(\sk^*(\sk),\ct_{b,\pk(\sk)})]\\
&\ge&
(1-2^{-\poly(\secp)})\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\secp)]
\Big(\frac{2}{3}-\frac{1}{\poly(\secp)}\Big)\\
&=&(1-2^{-\poly(\secp)})\Big(\frac{2}{3}-\frac{1}{\poly(\secp)}\Big).
\end{eqnarray*}
Therefore,
\begin{eqnarray*}
|\Pr[1\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\\
&=&
|1-\Pr[0\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\\
&\ge&
\Pr[0\gets\cA(\rho_0)]+\Pr[1\gets\cA(\rho_1)]-1\\
&\ge&
\frac{1}{\poly(\secp)}.
\end{eqnarray*}
\end{proof}

\begin{proof}[Proof of \cref{lemma:unbounded_algorithm}]
Let $\Pi_{b,\sk}$ be a POVM element that corresponds to the accepting event in the following operation:
On input a quantum state $\sigma$, run $b'\gets\Dec(\sk,\Enc(b,\sigma))$. If $b'=b$, accept. Otherwise, reject.
In other words,
\begin{eqnarray*}
\mbox{Tr}(\Pi_{b,\sk}\sigma)=\Pr[b\gets\Dec(\sk,\Enc(b,\sigma))].
\end{eqnarray*}
    
The algorithm $\cQ$ runs as follows.
\begin{enumerate}
    \item
    Compute the set $SK\coloneqq\{\sk~|~\Pr[\sk\gets\Gen_1(1^\secp)]>0\}$.
   \item 
   For $\{\Pi_{b,\sk'}\}_{b\in\bit,\sk'\in SK}$,
    run the shadow tomography algorithm on input $\pk(\sk)^{\otimes T}$.
    The shadow tomography algorithm outputs $\{\eta_{b,\sk'}\}_{b\in\bit,\sk'\in SK}$ such that
$|\eta_{b,\sk'}-\mbox{Tr}(\Pi_{b,\sk'}\pk(\sk))|\le\epsilon$ for each $b\in\bit$ and each $\sk'\in SK$
with probability at least $1-\delta$. 
\item
Find $\sk^*(\sk)$ such that
$\eta_{b,\sk^*(\sk)}\ge\frac{2}{3}$
for both $b\in\bit$. There exists at least one such $\sk^*(\sk)$,
because otherwise
\begin{eqnarray*}
&&\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\secp)]
\Pr[b\gets\Dec(\sk,\Enc(b,\pk(\sk)))]\\
&\le&\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\secp)]
(\eta_{b,\sk}+\epsilon)\\
&\le&\sum_{\sk}\Pr[\sk\gets\Gen_1(1^\secp)]
\Big(\frac{2}{3}+\epsilon\Big)\\
&\le& \frac{2}{3}+\epsilon
\end{eqnarray*}
for a $b\in\bit$, which contradicts the correctness.
\item
Output $\sk^*(\sk)$.
\end{enumerate}
\end{proof}





==> EFIfromPKE_backup.tex <==
\section{EFI from PKE}

\subsection{Ciphertexts are quantum}
In this subsection, we consider the case when ciphertexts are quantum, but
public keys are classical.

\begin{definition}[PKE with quantum ciphertexts]
A PKE scheme with quantum ciphertexts is a tuple of algorithms $(\Gen,\Enc,\Dec)$ such that
\begin{itemize}
    \item 
    $\Gen(1^\secp)\to(\sk,\pk):$
    It is a polynomial-time algorithm that, on input the security parameter $\secp$, outputs
    a classical secret key $\sk$ and a classical public key $\pk$.
    If $\Gen$ is a PPT algorithm, we say that the PKE scheme is type I.
    If $\Gen$ is a QPT algorithm, we say that the PKE scheme is type II.
    \item
    $\Enc(b,\pk)\to\ct:$
    It is a QPT algorithm that, on input a message $b\in\bit$ and $\pk$, outputs
    a quantum ciphertext $\ct_b$.
    \item
    $\Dec(\sk,\ct)\to b':$
    It is a QPT algorithm that, on input $\sk$ and $\ct$, outputs a bit $b'\in\bit$.
\end{itemize}
\paragraph{\bf Correctness:}
For each $b\in\bit$,
\begin{eqnarray*}
\Pr[b=b':(\sk,\pk)\gets\Gen(1^\secp),\ct\gets\Enc(\pk,b),b'\gets\Dec(\ct,\sk)]
\ge1-\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For any QPT adversary $\cA$,
\begin{eqnarray*}
&&|\Pr[1\gets \cA(\pk,\ct_0):(\sk,\pk)\gets\Gen(1^\secp),\ct_0\gets\Enc(\pk,0)]\\
&&-\Pr[1\gets \cA(\pk,\ct_1):(\sk,\pk)\gets\Gen(1^\secp),\ct_1\gets\Enc(\pk,1)]|
\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{theorem}
Type I PKE with quantum ciphertexts implies OWF.
\end{theorem}
It is a folklore. For the convenience of readers, we provide a proof in Appendix.
Because OWF implies EFI, we obtain the following corollary.
\begin{corollary}
Type I PKE with quantum ciphertexts implies EFI.
\end{corollary}

\begin{theorem}
Type II PKE with quantum ciphertexts implies EFI.
\end{theorem}
Note that $Gen$ does no longer imply OWF if it is type II, because
$Gen$ can has quantum randomness that cannot be simulated by a deterministic computation with random input classical seeds.

\begin{proof}
Define
\begin{eqnarray*}
\rho_b\coloneqq \sum_{\sk,\pk}\Pr[(\sk,\pk)\gets \Gen(1^\lambda)]
|\pk\rangle\langle\pk|\otimes \ct_b^{\pk}.
\end{eqnarray*}
This is exactly the state that the adversary of quantum PKE receives when $b$ is encrypted.
Therefore, due to the security, any QPT algorithm can
distinguish $\rho_0$ and $\rho_1$ at most $\negl(\secp)$ advantage.

\if0
Define 
\begin{eqnarray*}
S_b\coloneqq \{(\sk,\pk)~|~\Dec(\sk,\Enc(\pk,b))=b\}.
\end{eqnarray*}
Due to the correctness, for each $b\in\bit$,
\begin{eqnarray*}
\sum_{(\sk,\pk)\in S_b}\Pr[(\sk,\pk)\gets\Gen(1^\secp)]\ge1-\negl.
\end{eqnarray*}
\fi

\if0
We say that $\sk$ is associated with $\pk$ if $\Pr[(\sk,\pk)\gets\Gen(1^\secp)]>0$.
For each $b\in\bit$,
let us define the following set of ``good" $\pk$:
\begin{eqnarray*}
S_b\coloneqq\{\pk~|~\Pr[b\gets\Dec(\sk,\Enc(\pk,b))]\ge\delta~\mbox{for all $\sk$ that is associated with $\pk$.}\}.
\end{eqnarray*}
\fi

\if0
Let us define the following set of ``good'' $(\sk,\pk)$:
\begin{eqnarray*}
S_b\coloneqq\Big\{(\sk,\pk)~|~\Pr[b\gets\Dec(\sk,\Enc(\pk,b))]\ge\frac{1}{2}\Big\}.
\end{eqnarray*}

Due to the correctness, for each $b\in\bit$,
\begin{eqnarray*}
1-\negl(\secp)&\le&\sum_{(\sk,\pk)}\Pr[(\sk,\pk)\gets \Gen(1^\lambda)]\Pr[b\gets\Dec(\sk,\Enc(\pk,b))]\\
&=&\sum_{(\sk,\pk)\in S_b}\Pr[(\sk,\pk)\gets \Gen(1^\lambda)]\Pr[b\gets\Dec(\sk,\Enc(\pk,b))]\\
&&+\sum_{(\sk,\pk)\notin S_b}\Pr[(\sk,\pk)\gets \Gen(1^\lambda)]\Pr[b\gets\Dec(\sk,\Enc(\pk,b))]\\
&\le&\sum_{(\sk,\pk)\in S_b}\Pr[(\sk,\pk)\gets\Gen(1^\secp)]+\frac{1}{2},
\end{eqnarray*}
which means
\begin{eqnarray*}
\sum_{(\sk,\pk)\in S_b}\Pr[(\sk,\pk)\gets\Gen(1^\secp)]\ge\frac{1}{2}-\negl(\secp).
\end{eqnarray*}
\fi

Let $\sk^*(\pk)$ be $\sk$ that maximizes
$\Pr[b\gets\Dec(\sk,\Enc(\pk,b))]$. In other words,
\begin{eqnarray*}
\sk^*(\pk)\coloneqq
\arg\max_{\sk}\Pr[b\gets\Dec(\sk,\Enc(\pk,b))].
\end{eqnarray*}
Then, (with an unbounded-time operation), we can map $\rho_b$ to
\begin{eqnarray*}
\rho_b'\coloneqq\sum_{\sk,\pk}\Pr[(\sk,\pk)\gets \Gen(1^\lambda)]
|\pk\rangle\langle\pk|\otimes|\sk^*(\pk)\rangle\langle\sk^*(\pk)|\otimes \ct_b^{\pk}.
\end{eqnarray*}
If we apply $\Dec$ algorithm on the last two registers, the probability that
the result $b$ is obtained is 
\begin{eqnarray*}
&&\sum_{\sk,\pk}\Pr[(\sk,\pk)\gets \Gen(1^\lambda)]\Pr[b\gets\Dec(\sk^*(\pk),\Enc(\pk,b))]\\
&\ge&\sum_{\sk,\pk}\Pr[(\sk,\pk)\gets \Gen(1^\lambda)]\Pr[b\gets\Dec(\sk,\Enc(\pk,b))]\\
&\ge&1-\negl(\secp).
\end{eqnarray*}
Here, the last inequality comes from the correctness.
In other words, $\rho_0'$ and $\rho_1'$ (and therefore $\rho_0$ and $\rho_1$)
are statistically indistinguishable with the advantage $\ge1-\negl(\secp)$.

\end{proof}

\subsection{Quantum ciphertexts and quantum public keys}

If we apply $\Dec$ algorithm on the last two registers, the probability that
the result $b$ is obtained is 
\begin{eqnarray*}
&&\sum_{\sk,\pk}\Pr[(\sk,\pk)\gets \Gen(1^\secp)]\Pr[b\gets\Dec(\sk^*(\pk),\Enc(\pk,b))]\\
&\ge&\sum_{\sk,\pk}\Pr[(\sk,\pk)\gets \Gen(1^\secp)]\Big(\Pr[b\gets\Dec(\sk,\Enc(\pk,b))]-\frac{1}{p}\Big)\\
&\ge&1-\negl(\secp)-\frac{1}{p}\sum_{\sk,\pk}\Pr[(\sk,\pk)\gets\Gen(1^\secp)]\\
&\ge&1-\negl(\secp)-\frac{1}{p}.
\end{eqnarray*}
Here, the last inequality comes from the correctness.
In other words, $\rho_0'$ and $\rho_1'$ (and therefore $\rho_0$ and $\rho_1$)
are statistically indistinguishable with the advantage $\ge1-\negl(\secp)$.





==> EFIfromSKE.tex <==
\section{EFI from quantum SKE}

\begin{definition}[Quantum SKE]
A quantum SKE scheme is a tuple of algorithms $(\Enc,\Dec)$ such that
\begin{itemize}
\item 
$\Gen(1^\secp)\to\sk:$
It is a QPT algoithm that, on input the security parameter $\secp$, outputs a classical secret key
$\sk$.
    \item 
    $\Enc(\sk,b)\to\ct:$ It is a QPT algorithm that, on input $\sk$
    and $b\in\bit$,
    outputs a quantum ciphertext $\ct$.
    \item
    $\Dec(\ct,\sk)\to b':$ It is a QPT algorithm that, 
    on input $\ct$ and $\sk$, outputs $b'\in\bit$.
\end{itemize}
\paragraph{\bf Correctness:}
For each $b\in\bit$,
\begin{eqnarray*}
\Pr[b\gets\Dec(\sk,\ct):\sk\gets\Gen(1^\secp),\ct\gets\Enc(\sk,b)]\ge1-\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For each $b\in\bit$ and any QPT adversary $\cA$, 
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\ct_0):k\gets\bit^\secp,\ct\gets\Enc(k,x)]\\
&&-\Pr[1\gets\cA((|\psi_1\rangle\otimes...\otimes |\psi_l\rangle)^{\otimes t}):|\psi_1\rangle,...,|\psi_l\rangle\gets \mu_n]|
\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{theorem}
Quantum pseudo one-time pads imply EFI.
\end{theorem}

\begin{proof}
Let us define
\begin{eqnarray*}
\rho_0&\coloneqq&\frac{1}{2^\secp}\sum_{k\in\bit^\secp}\frac{1}{2^l}\sum_{x\in\bit^l}\ct_{k,x}^{\otimes T+1},\\
\rho_1&\coloneqq&\int_{|\psi_1\rangle,...,|\psi_l\rangle\gets\mu_n}(|\psi_1\rangle\langle\psi_1|\otimes...\otimes|\psi_l\rangle\langle\psi_l|)^{\otimes T+1},
\end{eqnarray*}
where $\ct_{k,x}$ is the output of $\Enc(k,x)$ and $T$ is a certain polynomial specified later.
Note that $\rho_1$ cannot be generated efficiently, but another state $\hat{\rho}_1$
that is statistically close to $\rho_1$ can be generated
in QPT by using the quantum design.
We actually use $\hat{\rho}_1$ instead of $\rho_1$.

Due to the security, $\rho_0$ and $\rho_1$ are computationally indistinguishable.
%Let us define
%\begin{eqnarray*}
%k^*(x)\coloneqq\arg\max_{k'\in\bit^\secp}\Pr[x\gets\Dec(k',\ct_{k,x})].
%\end{eqnarray*}

Next we show that $\rho_0$ and $\rho_1$ are statisfically distinguishable.
There is a quantum algorithm that, on input $T$ copies $\ct_{k,x}^{\otimes T}$ of $\ct_{k,x}$
with 
$T=\tilde{O}(nl\log(\delta^{-1})\lambda\epsilon^{-4})$,
outputs $k^*\in\bit^\secp$ such that 
\begin{eqnarray*}
\Pr[x\gets \Dec(k^*,\ct_{k,x})]\ge 
\Pr[x\gets \Dec(k,\ct_{k,x})]-2\epsilon.
\end{eqnarray*}
The algorithm runs as follows.
\begin{enumerate}
    \item 
    Let $\Pi_k^x$ be a POVM element that corresponds to the accepting event in the following operation:
    On input an $nl$-qubit state $\sigma$, run $x'\gets\Dec(k,\sigma)$. If $x'=x$, accept. Otherwise, reject.
    In other words,
    \begin{eqnarray*}
    \mbox{Tr}(\Pi_k^x\sigma)=\Pr[x\gets\Dec(k,\sigma)].
    \end{eqnarray*}
   \item 
   For $\{\Pi_{k'}^x\}_{k'\in\bit^\secp}$,
    run the shadow tomography algorithm on input $\ct_{k,x}^{\otimes T}$.
    The shadow tomography algorithm outputs $\{\eta_{k'}\}_{k'\in\bit^\secp}$ such that
$|\eta_{k'}-\mbox{Tr}(\Pi_{k'}^x\ct_{k,x})|\le\epsilon$ for each $k'\in\bit^\secp$
with probability at least $1-\delta$. 
\item
Find $k^*\coloneqq \arg\max_{k'\in\bit^\secp}\{\eta_{k'}\}_{k'\in\bit^\secp}$, and output $k^*$.
\end{enumerate}
Then, due to the property of the shadow tomography,
\begin{eqnarray*}
\Pr[x\gets\Dec(k^*,\Enc(k,x))]
&\ge& \eta_{k^*}-\epsilon\\
&\ge& \eta_k-\epsilon\\
&\ge& \Pr[x\gets\Dec(k,\Enc(k,x))]-2\epsilon.
\end{eqnarray*}

Then, an unbounded-time operation can map $\rho_0$ to
\begin{eqnarray*}
\rho_0'&\coloneqq&\frac{1}{2^\secp}\sum_{k\in\bit^\secp}\ct_{k,x}\otimes
|k^*(k)\rangle\langle k^*(k)|.
\end{eqnarray*}
If $\Dec$ is applied on it,
the probability of obtaining $x\in\bit^l$ is
\begin{eqnarray*}
\frac{1}{2^\secp}\sum_{k\in\bit^\secp}
\Pr[x\gets\Dec(k^*(k),\ct_{k,x})]
&\ge&
\frac{1}{2^\secp}\sum_{k\in\bit^\secp}
(\Pr[x\gets\Dec(k,\Enc(k,x))]-2\epsilon)\\
&\ge&
1-2\epsilon-\negl(\secp).
\end{eqnarray*}
On the other hand, for $\rho_1$, the same operation gives $x$ with probability
\begin{eqnarray*}
\int_{|\psi_1\rangle,...,|\psi_l\rangle\gets\mu_n}
\Pr[x\gets\Dec(k^*,|\psi_1\rangle\otimes...\otimes|\psi_l\rangle)]
\le2^{-l}.
\end{eqnarray*}


\end{proof}

==> OWSGfromCUSG.tex <==
\section{CUSGs and quantum money}
\label{sec:CUSG}





\subsection{Definition of CUSGs}
\label{sec:CUSG_def}

\begin{definition}[Computationally unclonable states generators (CUSGs)]
A computationally unclonable states generators (CUSG) is a set of algorithms 
$(\KeyGen,\StateGen)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs a classical key $k\in\bit^\secp$.
    \item
    $\StateGen(k)\to |\phi_k\rangle:$
    It is a QPT algorithm that, on input $k$, outputs an $m$-qubit state $|\phi_k\rangle$.
\end{itemize}
We require the computational unclonability as follows.

\paragraph{\bf Computational unclonability:}
For any QPT operation $\cE$ and any polynomial $t$,
\begin{eqnarray*}
\sum_k\Pr[k\gets\KeyGen(1^\secp)]\langle\phi_k|^{\otimes t+1}\cE(|\phi_k\rangle^{\otimes t})|\phi_k\rangle^{\otimes t+1}\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{theorem}
If private-key quantum money schemes exist then CUSGs exist.
\end{theorem}

\begin{proof}
Let $(\mathsf{QM}.\Gen,\mathsf{QM}.\Ver)$
be a private-key quantum money scheme.
From it, we construct a CUSG as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    Choose $k\gets\bit^\secp$.
    Output $k$.
    \item
    $\StateGen(k)\to|\phi_k\rangle:$
    Run $|\phi_k\rangle\gets\mathsf{QM}.\Gen(k)$.
    Output $|\phi_k\rangle$.
\end{itemize}
Assume that it does not satisfy the computational unclonability. Then,
there exists a QPT operation $\cE$ and polynomials $t,t'$ $(t'>t)$ such that
\begin{eqnarray*}
\frac{1}{2^\secp}\sum_k \langle\phi_k|^{\otimes t'}\cE(|\phi_k\rangle^{\otimes t})|\phi_k\rangle^{\otimes t'}
\ge\frac{1}{p}.
\end{eqnarray*}
Then for at least $\frac{1}{2p}$ fraction of $k$, we have
$\langle\phi_k|^{\otimes t'}\cE(|\phi_k\rangle^{\otimes t})|\phi_k\rangle^{\otimes t'}\ge\frac{1}{2p}$.

From the $\cE$, we construct a QPT adversary $\cB$ that breaks the security of quantum money as follows:
On input $|\phi_k\rangle^{\otimes t}$, output $\cE(|\phi_k\rangle^{\otimes t})$.
Then,
\begin{eqnarray*}
&&\sum_k\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
\Pr[\mathsf{Count}(k,\cE(|\phi_t\rangle^{\otimes t}))>t]\\
&\ge&
\sum_{k\in S}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
\Pr[\mathsf{Count}(k,\cE(|\phi_t\rangle^{\otimes t}))>t]\\
&\ge&
\frac{1}{2p}
\Big(\Pr[\mathsf{Count}(k,|\phi_t\rangle^{\otimes t'}))>t]
-\sqrt{1-\frac{1}{2p}}\\
&\ge&
\frac{1}{2p}
\Big(1-
-\sqrt{1-\frac{1}{2p}}\Big),
\end{eqnarray*}
which is non-negligible. Therefore, $\cB$ breaks the security of the quantum money scheme.
\end{proof}

\begin{theorem}
If CUSGs exist then OWSGs exist.
\end{theorem}

\begin{proof}
Let $(\mathsf{CUSG}.\KeyGen,\mathsf{CUSG}.\StateGen)$ be a CUSG.
From it, we construct wOWSG as follows. (From \cref{thm:amplification_OWSG}, it means the existence of a OWSG.)
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    Run $k\gets\mathsf{CUSG}.\KeyGen(1^\secp)$.
    Output $k$.
    \item
    $\StateGen(k)\to|\phi_k\rangle:$
    Run $|\phi_k\rangle\gets\mathsf{CUSG}.\StateGen(k)$.
    Output $|\phi_k\rangle$.
    \item
    $\Ver(k',|\phi_k\rangle)\to\top/\bot:$
    Measure $|\phi_k\rangle$
    with the basis $\{|\phi_{k'}\rangle\langle\phi_{k'}|,I-|\phi_{k'}\rangle\langle\phi_{k'}|\}$.
    If the first result is obtained, output $\top$. Otherwise, output $\bot$.
\end{itemize}
The correctness is clear. Let us show the security.
Assume that it is not secure. Then there exists a QPT adversary $\cA$
and a polynomial $t$ such that for any polynomial $p$,
\begin{eqnarray*}
\sum_{k,k'}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(|\phi_k\rangle^{\otimes t})]|\langle\phi_k|\phi_{k'}\rangle|^2\ge1-\frac{1}{p}.
\end{eqnarray*}
Let us define the set
\begin{eqnarray*}
S\coloneqq\Big\{(k,k')~\Big|~|\langle\phi_k|\phi_{k'}\rangle|^2\ge1-\frac{2}{p}\Big\}.
\end{eqnarray*}
Then, 
\begin{eqnarray*}
\sum_{k,k'}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(|\phi_k\rangle^{\otimes t})]\ge \frac{1}{2}
\end{eqnarray*}
because
\begin{eqnarray*}
1-\frac{1}{p}&\le&
\sum_{k,k'}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(|\phi_k\rangle^{\otimes t})]|\langle\phi_k|\phi_{k'}\rangle|^2\\
&=&
\sum_{(k,k')\in S}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(|\phi_k\rangle^{\otimes t})]|\langle\phi_k|\phi_{k'}\rangle|^2\\
&&+\sum_{(k,k')\notin S}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(|\phi_k\rangle^{\otimes t})]|\langle\phi_k|\phi_{k'}\rangle|^2\\
&\le&
\sum_{(k,k')\in S}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(|\phi_k\rangle^{\otimes t})]\\
&&+\Big(1-\frac{2}{p}\Big)\Big(1-\sum_{(k,k')\in S}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(|\phi_k\rangle^{\otimes t})]\Big),
\end{eqnarray*}
which means the above inequality.

From the $\cA$, let us consider a QPT operation as follows:
On input $|\phi_k\rangle^{\otimes t}$, run $k'\gets\cA(|\phi_k\rangle^{\otimes t})$.
Then run $\phi_{k'}\gets\mathsf{CUSG}.\StateGen(k')$ $t+1$ times, and
output $|\phi_{k'}\rangle^{\otimes t+1}$.
Then,
\begin{eqnarray*}
&&\sum_k\Pr[k\gets\KeyGen(1^\secp)]\langle\phi_k|^{\otimes t+1}\cE(|\phi_k\rangle^{\otimes t})|\phi_k\rangle^{\otimes t+1}\\
&=&
\sum_{k,k'}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(|\phi_k\rangle^{\otimes })]\langle\phi_k|\phi_{k'}\rangle|^{2(t+1)}\\
&\ge&
\sum_{(k,k')\in S}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(|\phi_k\rangle^{\otimes })]\langle\phi_k|\phi_{k'}\rangle|^{2(t+1)}\\
&\ge&
\frac{1}{2}e^{-1},
\end{eqnarray*}
where we have taken $p=2(t+1)$.
It means that the computational unclonability of the CUSG is broken.
\end{proof}

==> OWSGfromQPKE.tex <==
\section{OWSG from QPKE}
\mor{toru}

Quantum PKE is defined as follows.
\begin{definition}[Quantum PKE]
A quantum PKE scheme is a tuple of algorithms $(\Gen_1,\Gen_2,\Enc,\Dec)$ such that
\begin{itemize}
    \item 
    $\Gen_1(1^\secp)\to\sk:$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs
    a classical secret key $\sk$.
    \item
    $\Gen_2(\sk)\to\pk:$
    It is a QPT algorithm that, on input $\sk$, outputs
    a quantum public key $\pk$.
    \item
    $\Enc(x,\pk)\to\ct:$
    It is a QPT algorithm that, on input a message $x\in\bit^l$ and $\pk$, outputs
    a quantum ciphertext $\ct$.
    \item
    $\Dec(\sk,\ct)\to x':$
    It is a QPT algorithm that, on input $\sk$ and $\ct$, outputs $x'\in\bit^l$.
\end{itemize}
\paragraph{\bf Correctness:}
For any $x\in\bit^l$,
\begin{eqnarray*}
\Pr[x\gets\Dec(\ct,\sk):\sk\gets\Gen_1(1^\secp),\pk\gets\Gen_2(\sk),\ct\gets\Enc(\pk,x)]
\ge1-\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For any $x_0,x_1\in\bit^l$, any QPT adversary $\cA$, and any polynomial $t$,
\begin{eqnarray*}
&&|\Pr[1\gets \cA(\pk^{\otimes t},\ct_0):\sk\gets\Gen_1(1^\secp),\pk\gets\Gen_2(\sk),\ct_0\gets\Enc(\pk,x_0)]\\
&&-\Pr[1\gets \cA(\pk^{\otimes t},\ct_1):\sk\gets\Gen_1(1^\secp),\pk\gets\Gen_2(\sk),\ct_1\gets\Enc(\pk,x_1)]|
\le\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For any QPT adversary $\cA$ and any polynomial $t$,
\begin{eqnarray*}
\frac{1}{2^l}\sum_{x\in\bit^l}
\Pr[x\gets \cA(\pk^{\otimes t},\ct):\sk\gets\Gen_1(1^\secp),\pk\gets\Gen_2(\sk),\ct\gets\Enc(\pk,x)]
\le\negl(\secp).
\end{eqnarray*}
\mor{I choose the latter security definition, because it is weaker (right?)}
\end{definition}


\begin{theorem}
QPKE implies OWSGs.
\end{theorem}
\mor{Can we show the inverse?}
\mor{Can we improve QPKE to QPOTP?}

\begin{proof}
Let $(\mathsf{QPKE}.\Gen_1,\mathsf{QPKE}.\Gen_2,\mathsf{QPKE}.\Enc,\mathsf{QPKE}.\Dec)$
be a QPKE scheme. From it, we construct a OWSG as follows.
\begin{itemize}
\item
$\Gen_1(1^\secp)\to k:$
Run $\sk\gets\mathsf{QPKE}.\Gen_1(1^\secp)$.
Output $k\coloneqq\sk$.
\item
$\Gen_2(k)\to\phi_k:$
Parse $k=\sk$.
Run $\pk\gets\mathsf{QPKE}.\Gen_2(\sk)$.
Output $\phi_k\coloneqq \pk$.
\item
$\Ver(\phi_k,k')\to\top/\bot:$
Parse $\phi_k=\pk$.
Choose $x\gets\bit^l$.
Run $\ct\gets\QPKE.\Enc(\pk,x)$.
Run $x'\gets\QPKE.\Dec(k',\ct)$.
If $x'=x$, output $\top$. Otherwise, output $\bot$.
\end{itemize}


Correctness is clear. Let us show the security. Assume that it is not secure. In other words,
for a QPT $\cA$ and a polynomial $p$,
\begin{eqnarray*}
\Pr
\left[x'=x:
\begin{array}{cc}
\sk\gets\mathsf{QPKE}.\Gen_1(1^\secp)\\
\pk\gets\mathsf{QPKE}.\Gen_2(\sk)\\
k'\gets\cA(\pk^{\otimes t})\\
x\gets\bit^l\\
\ct\gets\mathsf{QPKE}.\Enc(\pk,x)\\
x'\gets\mathsf{QPKE}.\Dec(k',\ct)
\end{array}
\right]
\ge\frac{1}{p}.
\end{eqnarray*}
From this $\cA$, let us construct a QPT adversary $\cB$ that breaks
the QPKE scheme as follows.
It, on input $\pk^{\otimes t}$ and $\ct$, runs $\sk'\gets\cA(\pk^{\otimes t})$.
It then runs $x'\gets\mathsf{QPKE}.\Dec(\sk',\ct)$, and outputs $x'$.
The probability that it outputs $x$ is equal to the left-hand-side of the above inequality,
and therefore
the security of OWSG is broken.

\if0
Correctness is clear. Let us show the security. Assume that it is not secure. In other words,
\begin{eqnarray*}
\frac{1}{2^l}\sum_{x\in\bit^l}
f(x)\ge\frac{1}{p}
\end{eqnarray*}
for a QPT $\cA$ and a polynomial $p$,
where
\begin{eqnarray*}
f(x)\coloneqq
\frac{1}{2^n}\sum_{k\in\bit^n}
\sum_{\sk'}\Pr[\sk'\gets\cA(\pk_k^{\otimes t})]
\Pr[x\gets\mathsf{QPKE}.\Dec(\sk',\mathsf{QPKE}.\Enc(x,\pk_k))].
\end{eqnarray*}
Define
\begin{eqnarray*}
S\coloneqq\{x\in\bit^l~|~f(x)\ge\frac{1}{2p}
\}.
\end{eqnarray*}
Then, $\frac{|S|}{2^l}\ge\frac{1}{2p}$, because otherwise,
\begin{eqnarray*}
\frac{1}{p}&\le&
\frac{1}{2^l}\sum_{x\in S}f(x)
+\frac{1}{2^l}\sum_{x\notin S}f(x)\\
&<&\frac{1}{p},
\end{eqnarray*}
which is the contradiction.
Let us choose two $x_0,x_1\in S$.
Then,
\begin{eqnarray*}
\frac{1}{2^n}\sum_{k}
\sum_{\sk'}\Pr[\sk'\gets\cA(\pk_k^{\otimes t})]
\Pr[x_b\gets\mathsf{QPKE}.\Dec(\sk',\mathsf{QPKE}.\Enc(x_b,\pk_k))]
\Big]\ge\frac{1}{2p}
\end{eqnarray*}
for both $b\in\bit$.
\fi


\end{proof}


==> OWSGfromQmoney.tex <==
\section{OWSGs from private-key quantum money}
\label{sec:OWSGsfromQmoney}

\begin{theorem}
If private-key quantum money exists, then OWSGs exist.
\end{theorem}


\begin{proof}
Let $(\mathsf{QM}.\Gen,\mathsf{QM}.\Ver)$ be a private-key quantum money scheme.
From it, we construct a OWSG as follows.
\begin{itemize}
    \item 
    $\Gen_1(1^\secp)\to k:$
    Choose $k\gets\bit^\secp$.
    Output $k$.
    \item
    $\Gen_2(k)\to\phi_k:$
    Run $|\$_k\rangle\gets\mathsf{QM}.\Gen(k)$.
    Output $\phi_k\coloneqq |\$_k\rangle\langle\$_k|$.
    \item
    $\Ver(k',\phi_k)\to\top/\bot:$
    Parse $\phi_k=|\$_k\rangle\langle\$_k|$.
    Measure $|\$_k\rangle$ with the basis
    $\{|\$_{k'}\rangle\langle\$_{k'}|,I-|\$_{k'}\rangle\langle\$_{k'}|\}$,
    and output $\top$ if the first result is obtained.
    Output $\bot$ if the second result is obtained.
    (This measurement is done in the following way: generate $U(|k'\rangle|0...0\rangle)=|\$_{k'}\rangle|\eta_{k'}\rangle$,
    and discard the first register. Then apply $U^\dagger$ on $|\$_k\rangle|\eta_{k'}\rangle$, and measure all qubits
    in the computationl basis. If the result is $k'0...0$, accept. Otherwise, reject.)
\end{itemize}
The correctness is clear. Let us show the security. Assume that it is not secure.
Then, there exists a QPT $\cA$, a polynomial $t$, and a polynomial $p$ such that
\begin{eqnarray}
\frac{1}{2^\secp}\sum_{k,k'}
    \Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    |\langle\$_k|\$_{k'}\rangle|^2
    \ge\frac{1}{p}.
    \label{Qmoney_notsecure}
    \end{eqnarray}
    
    From this $\cA$, we construct a QPT adversary $\cB$ that breaks the security of the private-key quantum money 
    scheme as follows:
    On input $|\$_k\rangle^{\otimes t}$, it runs $k'\gets\cA(|\$_k\rangle^{\otimes t})$.
    It then runs $|\$_{k'}\rangle\gets\mathsf{QM}.\Gen(k')$ $r$ times, where 
  $r$ is a polynomial specified later,
    and outputs $\xi\coloneqq |\$_{k'}\rangle^{\otimes r}$.
    
    Let us show that thus defined $\cB$ breaks the security of the private-key quantum money scheme.
    First, define the set
    \begin{eqnarray*}
    S\coloneqq\Big\{(k,k')\in\bit^\secp\times\bit^\secp~\Big|~|\langle\$_k|\$_{k'}\rangle|^2\ge
    \frac{1}{2p}\Big\}.
    \end{eqnarray*}
    Then, we have
    \begin{eqnarray}
    \frac{1}{2^\secp}\sum_{(k,k')\in S}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]\ge \frac{1}{2p}.
    \label{Qmoney_Sbound}
    \end{eqnarray}
    This is shown as follows.
   \begin{eqnarray*} 
   \frac{1}{p}&\le&
    \frac{1}{2^\secp}\sum_{k,k'}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    |\langle\$_k|\$_{k'}\rangle|^2\\
    &=&\frac{1}{2^\secp}\sum_{(k,k')\in S}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    |\langle\$_k|\$_{k'}\rangle|^2\\
    &&+\frac{1}{2^\secp}\sum_{(k,k')\notin S}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    |\langle\$_k|\$_{k'}\rangle|^2\\
    &\le&
    \frac{1}{2^\secp}\sum_{(k,k')\in S}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    +\frac{1}{2p}.
   \end{eqnarray*} 
   Here, the first inequality is from Eq.~(\ref{Qmoney_notsecure}).
   
  Let us also define  
  \begin{eqnarray*}
  T\coloneqq\Big\{k\in\bit^\secp~\Big|~\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]
  \ge1-\frac{1}{8p}\Big\}.
  \end{eqnarray*}
  Then, 
  \begin{eqnarray}
  \frac{|T|}{2^\secp}\ge 1-\negl(\secp). 
  \label{Qmoney_Tbound}
  \end{eqnarray}
  This is shown as follows.
  \begin{eqnarray*}
  1-\negl(\secp)&\le&\frac{1}{2^\secp}\sum_k\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\\
  &=&\frac{1}{2^\secp}\sum_{k\in T}\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\\
  &&+\frac{1}{2^\secp}\sum_{k\notin T}\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\\
  &\le& \frac{|T|}{2^\secp}+\Big(1-\frac{1}{8p}\Big)\Big(1-\frac{|T|}{2^\secp}\Big).
  \end{eqnarray*}
  Here, the first inequality comes from the correctness of quantum money.
  
  
   
   
  Let us fix $(k,k')$ such that $(k,k')\in S$ and $k\in T$. 
  The probability of having such $(k,k')$ is, from the union bound, Eq.~(\ref{Qmoney_Sbound}), and Eq.~(\ref{Qmoney_Tbound}),
  \begin{eqnarray}
  \frac{1}{2^\secp}\sum_{(k,k')\in S \wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
  &\ge& \frac{1}{2p}+1-\negl(\secp)-1\nonumber\\
  &=& \frac{1}{2p}-\negl(\secp).
  \label{Qmoney_union}
  \end{eqnarray}
  Let 
   $v_j$ be the bit that is 1 if the output of $\mathsf{QM}.\Ver(k,\xi_j)$ is $\top$, and
   is 0 otherwise.
   Then, 
   \begin{eqnarray}
   \Pr[v_j=1]
   &=&\Pr[\top\gets\mathsf{QM}.\Ver(k,\xi_j)]\nonumber\\
   &=&\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_{k'}\rangle)]\nonumber\\
   &\ge&\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]-\sqrt{1-\frac{1}{2p}}\nonumber\\
   &\ge&1-\frac{1}{8p}-\sqrt{1-\frac{1}{2p}}\nonumber\\
   &\ge&\frac{1}{8p}\label{Qmoney_vj}
   \end{eqnarray}
   for each $j\in[1,2,...,r]$.
   Here, in the first inequality, we have used the fact that
   $|\Pr[1\gets\cD(|\$_k\rangle)]-\Pr[1\gets\cD(|\$_{k'}\rangle)]|\le \sqrt{1-\frac{1}{2p}}$ for any algorithm $\cD$.
   This is because $|\langle\$_k|\$_{k'}\rangle|^2\ge\frac{1}{2p}$ for any $(k,k')\in S$.\footnote{Due to the relation between the fidelity and
   the trace distance, we have $\frac{1}{2}\||\$_k\rangle\langle\$_k|-|\$_{k'}\rangle\langle\$_{k'}|\|_1\le \sqrt{1-|\langle\$_k|\$_{k'}\rangle|^2}$,
   which means that $\langle\$_k|\Pi|\$_k\rangle-\langle\$_{k'}|\Pi|\$_{k'}\rangle\le\sqrt{1-|\langle\$_k|\$_{k'}\rangle|^2}$
   for any POVM element $\Pi$.}
   Moreover, in the second inequality, we have used the fact that 
   $\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\ge1-\frac{1}{8p}$ for any $k\in T$.
   Finally, in the last inequality, we have used the Bernoulli's inequality.\footnote{$(1+x)^r\le 1+rx$ for any real $r$ and $x$ such that $0\le r\le1$ and $x\ge-1$.}
   
   
  Let us take $r\ge \max(16p(t+1),16^2p^3)$.
  Then,
    \begin{eqnarray}
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes r})\ge t+1]
    &=&
    \Pr\Big[\sum_{j=1}^r v_j\ge t+1\Big]\nonumber\\
    &\ge&
    \Pr\Big[\sum_{j=1}^r v_j\ge \frac{r}{16p}\Big]\nonumber\\
    &=&
    \Pr\Big[\sum_{j=1}^r v_j\ge \frac{r}{8p} -\frac{r}{16p}\Big]\nonumber\\
    &\ge&
   \Pr\Big[\sum_{j=1}^r v_j\ge E(\sum_{j=1}^r v_j)-\frac{r}{16p}\Big]\nonumber\\
   &\ge&1-2\exp\Big[-\frac{2r}{16^2p^2}\Big]\nonumber\\
   &\ge&1-2e^{-2p}.\label{Qmoney_coundbound}
   \end{eqnarray}
   Here, in the second inequality, we have used Eq.~(\ref{Qmoney_vj}),
   and in the third inequality, we have used Hoeffding's inequality. 
   
The probability that $\cB$ wins is
    \begin{eqnarray*} 
    &&\frac{1}{2^\secp}\sum_{k,k'}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes r})\ge t+1]\\
    &\ge&\frac{1}{2^\secp}\sum_{(k,k')\in S\wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes r})\ge t+1]\\
    &\ge&
   (1-2e^{-2p})
    \frac{1}{2^\secp}\sum_{(k,k')\in S\wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]\\
   &\ge&(1-2e^{-2p})
  \Big(\frac{1}{2p}-\negl(\secp)\Big),
   \end{eqnarray*} 
   which is non-negligible. The $\cB$ therefore breaks the security of the private-key quantum money scheme.
   Here, in the second inequality, we have used Eq.~(\ref{Qmoney_coundbound}),
   and in the last inequality, we have used Eq.~(\ref{Qmoney_union}).

   
   \if0
      The probability that $\cB$ wins is
    \begin{eqnarray*} 
    &&\frac{1}{2^\secp}\sum_{k,k'}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes rt})>t]\\
    &\ge&\frac{1}{2^\secp}\sum_{(k,k')\in S\wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes rt})>t]\\
    &\ge&\frac{1}{2^\secp}\sum_{(k,k')\in S\wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
   \frac{(\tau-\sqrt{1-\delta}) r -(t+1)}{r-(t+1)}\\
   &\ge&\frac{(\tau-\sqrt{1-\delta}) r -(t+1)}{r-(t+1)}
  \Big(\frac{1}{p}-\delta-\tau-\negl(\secp)\Big).
   \end{eqnarray*} 
  \mor{it is not non-negligible}
%   which is non-negligible,
%   and therefore $\cB$ breaks the security of the private-key quantum money scheme.
\fi
\end{proof}

==> OWSGfromQmoney_backup.tex <==
\section{OWSGs from private-key quantum money}
\label{sec:OWSGsfromQmoney}

\begin{theorem}
If private-key quantum money exists, then OWSGs exist.
\end{theorem}
\mor{For general $\mathsf{QM}.\Ver$, amplification of OWSGs seems to be necessary.
If $\mathsf{QM}.\Ver$ is restricted to the inner-product one, the proof exsits.
If the amplification of OWSGs are possible, then even computationally unclonable states generators $\to$ OWSGs
will be shown.}

\if0
\begin{remark}
Note that we consider specific private-key quantum money where
the verification algorithm is the following:
On input the secret key $k$ and an alleged quantum money $\rho$,
measure $\rho$ with the basis $\{|\phi_k\rangle\langle\phi_k|,I-|\phi_k\rangle\langle\phi_k|\}$,
and accept if and only if the result $|\phi_k\rangle\langle\phi_k|$ is obtained.
It is an open problem whether the result is improved to more general verification algorithms.
\end{remark}
\fi

\begin{proof}
Let $(\mathsf{QM}.\Gen,\mathsf{QM}.\Ver)$ be a private-key quantum money scheme.
From it, we construct a OWSG as follows.
\begin{itemize}
    \item 
    $\Gen_1(1^\secp)\to k:$
    Choose $k\gets\bit^\secp$.
    Output $k$.
    \item
    $\Gen_2(k)\to\phi_k:$
    Run $|\$_k\rangle\gets\mathsf{QM}.\Gen(k)$.
    Output $\phi_k\coloneqq |\$_k\rangle\langle\$_k|$.
    \item
    $\Ver(k',\phi_k)\to\top/\bot:$
    Parse $\phi_k=|\$_k\rangle\langle\$_k|$.
    Measure $|\$_k\rangle$ with the basis
    $\{|\$_{k'}\rangle\langle\$_{k'}|,I-|\$_{k'}\rangle\langle\$_{k'}|\}$,
    and output $\top$ if the first result is obtained.
    Output $\bot$ if the second result is obtained.
    (This measurement is done in the following way: generate $U(|k'\rangle|0...0\rangle)=|\$_{k'}\rangle|\eta_{k'}\rangle$,
    and discard the first register. Then apply $U^\dagger$ on $|\$_k\rangle|\eta_{k'}\rangle$, and measure all qubits
    in the computationl basis. If the result is $k'0...0$, accept. Otherwise, reject.)
\end{itemize}
The correctness is clear. Let us show the security. Assume that it is not secure.
Then, there exists a QPT $\cA$, a polynomial $t$, and a polynomial $p$ such that
\begin{eqnarray*}
\frac{1}{2^\secp}\sum_{k,k'}
    \Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    |\langle\$_k|\$_{k'}\rangle|^2
    \ge\frac{1}{p}.
    \end{eqnarray*}
    
    From this $\cA$, we construct a QPT adversary $\cB$ that breaks the security of the private-key quantum money 
    scheme as follows:
    On input $|\$_k\rangle^{\otimes t}$, it runs $k'\gets\cA(|\$_k\rangle^{\otimes t})$.
    It then runs $|\$_{k'}\rangle\gets\mathsf{QM}.\Gen(k')$ $r$ times, where 
  $r$ is a polynomial specified later,
    and outputs $\xi\coloneqq |\$_{k'}\rangle^{\otimes r}$.
    
    Let us show that thus defined $\cB$ breaks the security of the private-key quantum money scheme.
    First, define the set
    \begin{eqnarray*}
    S\coloneqq\Big\{(k,k')\in\bit^\secp\times\bit^\secp~\Big|~|\langle\$_k|\$_{k'}\rangle|^2\ge\delta\Big\},
    \end{eqnarray*}
    where $0<\delta<\frac{1}{p}$ is a parameter specified later.
    Then,
    \begin{eqnarray}
    \frac{1}{2^\secp}\sum_{(k,k')\in S}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]\ge \frac{1}{p}-\delta,
    \end{eqnarray}
    because 
   \begin{eqnarray*} 
   \frac{1}{p}&\le&
    \frac{1}{2^\secp}\sum_{k,k'}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    |\langle\$_k|\$_{k'}\rangle|^2\\
    &=&\frac{1}{2^\secp}\sum_{(k,k')\in S}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    |\langle\$_k|\$_{k'}\rangle|^2\\
    &&+\frac{1}{2^\secp}\sum_{(k,k')\notin S}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    |\langle\$_k|\$_{k'}\rangle|^2\\
    &\le&
    \frac{1}{2^\secp}\sum_{(k,k')\in S}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    +\delta.
   \end{eqnarray*} 
   
  Let us also define  
  \begin{eqnarray*}
  T\coloneqq\Big\{k\in\bit^\secp~\Big|~\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\ge\tau\Big\},
  \end{eqnarray*}
  where $0<\tau<1$ is a parameter specified later.
  Then, 
  \begin{eqnarray}
  \frac{|T|}{2^\secp}\ge \frac{1-\tau-\negl(\secp)}{1-\tau}, 
  \end{eqnarray}
  because 
  \begin{eqnarray*}
  1-\negl(\secp)&\le&\frac{1}{2^\secp}\sum_k\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\\
  &=&\frac{1}{2^\secp}\sum_{k\in T}\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\\
  &&+\frac{1}{2^\secp}\sum_{k\notin T}\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\\
  &\le& \frac{|T|}{2^\secp}+\tau\Big(1-\frac{|T|}{2^\secp}\Big).
  \end{eqnarray*}
  
  
   
   
  Let us fix $(k,k')$ such that $(k,k')\in S$ and $k\in T$. 
  The probability of having such $(k,k')$ is, from the union bound,
  \begin{eqnarray}
  \frac{1}{2^\secp}\sum_{(k,k')\in S \wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
  &\ge& \frac{1}{p}-\delta+\frac{1-\tau-\negl(\secp)}{1-\tau}-1\\
  &=& \frac{1}{p}-\delta-\frac{\negl(\secp)}{1-\tau}.
  \end{eqnarray}
  Let 
   $v_j$ be the bit that is 1 if the output of $\mathsf{QM}.\Ver(k,\xi_j)$ is $\top$, and
   is 0 otherwise.
   Then, 
   \begin{eqnarray}
   \Pr[v_j=1]
   &=&\Pr[\top\gets\mathsf{QM}.\Ver(k,\xi_j)]\\
   &=&\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_{k'}\rangle)]\\
   &\ge&\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]-\sqrt{1-\delta}\\
   &\ge&\tau-\sqrt{1-\delta}
   \end{eqnarray}
   for each $j\in[1,2,...,r]$.
   
   \if0
   From Markov inequality,
   \begin{eqnarray*}
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes rt})> t]
    &=&
   \Pr\Big[\sum_{j=1}^r v_j \ge t+1\Big]
   \ge\frac{(\tau-\sqrt{1-\delta}) r -(t+1)}{r-(t+1)}.
   \end{eqnarray*}
   \fi
   
   Let us take $r$ and $\alpha$ so that
  $t+1\le (\tau-\sqrt{1-\delta})r-\alpha$. 
  From Hoeffding's inequality, 
    \begin{eqnarray*}
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes r})\ge t+1]
    &=&
    \Pr[\sum_{j=1}^r v_j\ge t+1]\\
    &\ge&
    \Pr[\sum_{j=1}^r v_j\ge(\tau-\sqrt{1-\delta})r -\alpha]\\
    &\ge&
   \Pr\Big[\sum_{j=1}^r v_j\ge E(\sum_{j=1}^r v_j)-\alpha\Big]\\
   &\ge&1-e^{-\frac{2\alpha^2}{r}}.
   \end{eqnarray*}
   
   
The probability that $\cB$ wins is
    \begin{eqnarray*} 
    &&\frac{1}{2^\secp}\sum_{k,k'}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes rt})\ge t+1]\\
    &\ge&\frac{1}{2^\secp}\sum_{(k,k')\in S\wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes rt})\ge t+1]\\
    &\ge&
   (1-e^{-\frac{2\alpha^2}{r}})
    \frac{1}{2^\secp}\sum_{(k,k')\in S\wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]\\
   &\ge&(1-e^{-\frac{2\alpha^2}{r}})
  \Big(\frac{1}{p}-\delta-\frac{\negl(\secp)}{1-\tau}\Big).
   \end{eqnarray*} 

Let us take $\delta=\frac{1}{2p}$, $\tau=1-\frac{1}{8p}$,
  $\alpha=\frac{(\tau-\sqrt{1-\delta})r}{2}$, 
  $r\ge \frac{2(t+1)}{\tau-\sqrt{1-\delta}}$. 
   
   \if0
      The probability that $\cB$ wins is
    \begin{eqnarray*} 
    &&\frac{1}{2^\secp}\sum_{k,k'}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes rt})>t]\\
    &\ge&\frac{1}{2^\secp}\sum_{(k,k')\in S\wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
    \Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes rt})>t]\\
    &\ge&\frac{1}{2^\secp}\sum_{(k,k')\in S\wedge k\in T}\Pr[k'\gets\cA(|\$_k\rangle^{\otimes t})]
   \frac{(\tau-\sqrt{1-\delta}) r -(t+1)}{r-(t+1)}\\
   &\ge&\frac{(\tau-\sqrt{1-\delta}) r -(t+1)}{r-(t+1)}
  \Big(\frac{1}{p}-\delta-\tau-\negl(\secp)\Big).
   \end{eqnarray*} 
  \mor{it is not non-negligible}
%   which is non-negligible,
%   and therefore $\cB$ breaks the security of the private-key quantum money scheme.
\fi
\end{proof}

==> OrthogonalOWSG.tex <==
\section{EFI pairs from special OWSGs}
\label{sec:orthogonal}

In this section, we use the following result.
\begin{theorem}[\cite{HMY22}]
\label{theorem:HMY22}
Let $\ket{\psi}$ and $\ket{\phi}$ be orthogonal states, and suppose that a non-uniform QPT adversary $A$ 
with an advice $\ket{\tau}$ distinguishes $\ket{\psi}$ and $\ket{\phi}$ with advantage $\Delta$ without using 
additional ancilla qubits besides $\ket{\tau}$. Then, there exists a QPT unitary $U$ 
such that 
\begin{align*}
\frac{|\bra{y}\bra{\tau}U\ket{x}\ket{\tau}+\bra{x}\bra{\tau}U\ket{y}\ket{\tau}|}{2}=\Delta,
\end{align*}
where  $|x\rangle\coloneqq\frac{|\psi\rangle+|\phi\rangle}{\sqrt{2}}$ 
and $|y\rangle\coloneqq\frac{|\psi\rangle-|\phi\rangle}{\sqrt{2}}$.
Moreover, if $\A$ does not act on some qubits, then $U$ also does not act on those qubits.
\end{theorem}

Our result in this section is as follows.
\begin{theorem}
Consider a special OWSG where $\Gen_2$ runs as follows: it applies a QPT unitary $U$ on
$|k\rangle|0...0\rangle$ to generate $U(|k\rangle|0...0\rangle)=|k\rangle\otimes|\phi_k\rangle$, and outputs $|\phi_k\rangle$.
Moreover, $\langle\phi_k|\phi_{k'}\rangle=0$ is satisfied for any $k\neq k'$.
Then, such a OWSG implies EFI pairs.
\end{theorem}

\begin{proof}
Let $(\mathsf{OWSG}.\Gen_1,\mathsf{OWSG}.\Gen_2,\mathsf{OWSG}.\Ver)$ be such a special OWSG.
From it, we construct EFI pairs $\Gen(b,1^\secp)\to\rho_b$ as follows.
\begin{enumerate}
    \item 
    Run $\mathsf{OWSG}.\Gen_1$ to generate 
    \begin{eqnarray*}
    \sum_{k}\Pr[k\gets\Gen_1(1^\secp)]|k\rangle\langle k|.
    \end{eqnarray*}
    \item
    Add the ancilla state
    \begin{eqnarray*}
    \sum_{k}\Pr[k\gets\Gen_1(1^\secp)]|k\rangle\langle k|\otimes
    \frac{|0\rangle|0...0\rangle+(-1)^b|1\rangle|0...0\rangle}{\sqrt{2}}
    \frac{\langle 0|\langle 0...0|+(-1)^b\langle 1|\langle0...0|}{\sqrt{2}}.
    \end{eqnarray*}
    \item
    Apply $U$ on the first and third registers conditioned that the second register is 1: 
    \begin{eqnarray*}
    \sum_{k}\Pr[k\gets\Gen_1(1^\secp)]|k\rangle\langle k|\otimes
    \frac{|0\rangle|0...0\rangle+(-1)^b|1\rangle|\phi_k\rangle}{\sqrt{2}}
    \frac{\langle 0|\langle 0...0|+(-1)^b\langle 1|\langle\phi_k|}{\sqrt{2}}.
    \end{eqnarray*}
     \item
    Copy the content of the first register to the third register 
    conditioned that the second register is 0: 
    \begin{eqnarray*}
&&    \sum_{k}\Pr[k\gets\Gen_1(1^\secp)]|k\rangle\langle k|\otimes
    \frac{|0\rangle|k0...0\rangle+(-1)^b|1\rangle|\phi_k\rangle}{\sqrt{2}}
    \frac{\langle 0|\langle k0...0|+(-1)^b\langle 1|\langle\phi_k|}{\sqrt{2}}\\
   &\coloneqq&  \sum_{k}\Pr[k\gets\Gen_1(1^\secp)]|k\rangle\langle k|\otimes|\psi_k^b\rangle\langle\psi_k^b|.
    \end{eqnarray*}
    \item
    Trace out the first register: 
    \begin{eqnarray*}
   \sum_{k}\Pr[k\gets\Gen_1(1^\secp)]|\psi_k^b\rangle\langle\psi_k^b|\coloneqq\rho_b.
    \end{eqnarray*}
    Output it.
\end{enumerate}
We first show the statistical distinguishability of $\rho_0$ and $\rho_1$.
Note that $\langle\psi_k^b|\psi_{k'}^{b'}\rangle=0$ for any $k\neq k'$ and $b,b'\in\bit$.
Therefore,
\begin{eqnarray*}
F(\rho_0,\rho_1)=\|\sqrt{\rho_0}\sqrt{\rho_1}\|_1^2=0.
\end{eqnarray*}

We next show the computational indistinguishability of $\rho_0$ and $\rho_1$.
Assume that they are computationally distinguishable.
It means that there exists a QPT adversary $\cA$ and a polynomial $p$ such that
\begin{eqnarray*}
|\Pr[1\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\ge\frac{1}{p}.
\end{eqnarray*}
Define the set 
\begin{eqnarray*}
S\coloneqq\Big\{k\in\bit^\secp~|~|\Pr[1\gets\cA(|\psi_k^0\rangle)]-\Pr[1\gets\cA(|\psi_k^1\rangle)]|\ge\frac{1}{2p}\Big\}.
\end{eqnarray*}
Then, 
\begin{eqnarray*}
\sum_{k\in S}\Pr[k\gets\Gen_1(1^\secp)]\ge\frac{1}{2p},
\end{eqnarray*}
because
\begin{eqnarray*}
\frac{1}{p}&\le&
|\Pr[1\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\\
&=&
|\sum_k\Pr[k\gets\Gen_1(1^\secp)](\Pr[1\gets\cA(|\psi_k^0\rangle)]-\Pr[1\gets\cA(|\psi_k^1\rangle)])|\\
&\le&
\sum_k\Pr[k\gets\Gen_1(1^\secp)]|\Pr[1\gets\cA(|\psi_k^0\rangle)]-\Pr[1\gets\cA(|\psi_k^1\rangle)]|\\
&=&
\sum_{k\in S}\Pr[k\gets\Gen_1(1^\secp)]|\Pr[1\gets\cA(|\psi_k^0\rangle)]-\Pr[1\gets\cA(|\psi_k^1\rangle)]|\\
&&+\sum_{k\notin S}\Pr[k\gets\Gen_1(1^\secp)]|\Pr[1\gets\cA(|\psi_k^0\rangle)]-\Pr[1\gets\cA(|\psi_k^1\rangle)]|\\
&\le&
\sum_{k\in S}\Pr[k\gets\Gen_1(1^\secp)]
+\frac{1}{2p}.
\end{eqnarray*}

We can show that there exists a QPT adversary $\cB$ such that
for any $k\in S$
\begin{eqnarray*}
\Pr[k\gets\cB(|\phi_k\rangle)]\ge\frac{1}{4p^2}.
\end{eqnarray*}
This is shown as follows. Note that $\langle\psi_k^0|\psi_k^1\rangle=0$.
Therefore, from \cref{theorem:HMY22},  there is a QPT unitary $V$ such that
\begin{eqnarray*}
|(\langle0|\langle k0...0|\langle\tau|)V(|1\rangle|\phi_k\rangle|\tau\rangle)
+(\langle1|\langle \phi_k|\langle\tau|)V(|0\rangle|k0...0\rangle|\tau\rangle)|\ge \frac{1}{p}.
\end{eqnarray*}
It means that
\begin{eqnarray*}
|(\langle0|\langle k0...0|\langle\tau|)V(|1\rangle|\phi_k\rangle|\tau\rangle)|\ge\frac{1}{2p}
\end{eqnarray*}
or 
\begin{eqnarray*}
|(\langle1|\langle \phi_k|\langle\tau|)V(|0\rangle|k0...0\rangle|\tau\rangle)|\ge\frac{1}{2p}.
\end{eqnarray*}
Without loss of generality, we assume the former case.
(If the latter case occurs, we have only replace $V$ with $V^\dagger$ in the following argument.)
Let us consider a QPT adversary $\cB$ that, on input $|\phi_k\rangle$, applies
$V$ on $|1\rangle|\phi_k\rangle|\tau\rangle$, measures the first $\secp$ qubits in the computational basis,
and outputs the result.
Then,
\begin{eqnarray*}
\Pr[k\gets\cB(|\phi_k\rangle)]
&=&
\|(I\otimes|k\rangle\langle k|\otimes I)V(|1\rangle|\phi_k\rangle|\tau\rangle)\|^2\\
&\ge&
|(\langle0|\langle k0...0|\langle\tau|)V(|1\rangle|\phi_k\rangle|\tau\rangle)|^2\\
&\ge&\frac{1}{4p^2}.
\end{eqnarray*}

This $\cB$ breaks the security of OWSGs, because
\begin{eqnarray*}
\sum_{k}\Pr[k\gets\Gen_1(1^\secp)]\Pr[k\gets\cB(|\phi_k\rangle)]
&\ge&
\sum_{k\in S}\Pr[k\gets\Gen_1(1^\secp)]\Pr[k\gets\cB(|\phi_k\rangle)]\\
&\ge&
\frac{1}{2p}\frac{1}{4p^2}.
\end{eqnarray*}
\end{proof}








==> QDSfromOWSG.tex <==
\section{QDSs from OWSGs}
\label{sec:QDSfromOWSG}
%checkdone 2022/9/25

\begin{theorem}
If OWSGs exist then QDSs exist.
\end{theorem}

\begin{proof}

\end{proof}


==> RSP.tex <==
\section{Newly obtained results}
\mor{Newly added!!}


\subsection{EFI from the hardness of ${\bf QSRE}$}
\cite{cryptoeprint:2022/1181} constructed EFI pairs from
the assumption that ${\bf QCZK}$ is hard on average against $\BQP$.
Here we construct EFI pairs from the assumption that
${\bf QSRE}\not\subseteq\BQP$.
An advantage of our result is that it does not need any average-case-hard assumption, but
a disadvantage of our result is that the class ${\bf QSRE}$ seems to be stronger than ${\bf QCZK}$
(${\bf QSRE}\subseteq {\bf QSZK}\subseteq{\bf QCZK}$).
Our result can be considered as a quantum analogue of the classical result \cite{C:AppRay16}
where (infinitely-often) OWFs are constructed from the assumption of ${\bf SRE}\not\subseteq{\bf BPP}$.

\begin{definition}[Quantum randomized encoding (${\bf QSRE}$)]
\label{def:QSRE}
A promise problem
$(L_Y,L_N)$ is in quantum randomized encoding
(${\bf QSRE}$) if there exist QPT algorithms $(\Enc,\Sim_Y,\Sim_N)$
and a unbounded-time quantum algorithm $\Dec$ such that
\begin{itemize}
\item
{\bf Security for yes instances:}
For any $x\in L_Y$, 
\begin{eqnarray*}
\|\Enc(x)-\Sim_Y(1^{|x|})\|_1\le\negl(|x|).
\end{eqnarray*}
\item
{\bf Security for no instances:}
For any $x\in L_N$,
\begin{eqnarray*}
\|\Enc(x)-\Sim_N(1^{|x|})\|_1\le\negl(|x|).
\end{eqnarray*}
\item
{\bf Correctness:}
For any $x\in L_Y\cup L_N$,
\begin{eqnarray*}
\Pr[L(x)\gets\Dec(\Enc(x))]\ge1-\negl(|x|),
\end{eqnarray*}
where $L(x)=1$ if $x\in L_Y$ and 
$L(x)=0$ if $x\in L_N$.
\end{itemize}
\end{definition}

\begin{theorem}
If ${\bf QSRE}\not\subseteq\BQP$,
then EFI pairs (\mor{infinitely-often?} secure against uniform QPT adversaries) exist.
\end{theorem}

\begin{proof}
Assume that ${\bf QSRE}\not\subseteq\BQP$.
Then there exists a promise problem
$(L_Y,L_N)$ that is in ${\bf QSRE}$ but not in $\BQP$.
Because $(L_Y,L_N)$ is in ${\bf QSRE}$, there exist
QPT algorithms $(\Enc,\Sim_Y,\Sim_N)$
and a unbounded-time quantum algorithm $\Dec$ that satisfy
the three conditions in \cref{def:QSRE}.
From them, we construct an EFI pair as follows.
\begin{itemize}
    \item $\StateGen(b,1^\secp)\to\rho_b$:
    If $b=0$, run $\rho_0\gets\Sim_Y(1^\secp)$.
    If $b=1$, run $\rho_1\gets\Sim_N(1^\secp)$.
    Output $\rho_b$.
\end{itemize}
We first show the statistical distinguishability of $\rho_0$ and $\rho_1$.
Assume that $\|\rho_0-\rho_1\|_1\le\negl(\secp)$.
Then, for any $x\in L_Y$ and $x'\in L_N$,
\begin{eqnarray*}
&&|\Pr[1\gets \Dec(\Enc(x))]-\Pr[1\gets \Dec(\Enc(x'))]|\\
&\le&|\Pr[1\gets \Dec(\Sim_Y(1^{|x|}))]-\Pr[1\gets \Dec(\Sim_N(1^{|x|}))]|
+\negl(|x|)\\
&\le&\negl(|x|),
\end{eqnarray*}
which contradicts the correctness. Therefore, 
$\|\rho_0-\rho_1\|_1\ge\frac{1}{\poly(\secp)}$.

We next show the computational indistinguishability of $\rho_0$ and $\rho_1$.
Assume that there exists a QPT adversary $\cA$ such that
\begin{eqnarray*}
|\Pr[1\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\ge\frac{1}{\poly(\secp)}.
\end{eqnarray*}
Then, from the $\cA$, we construct a QPT adversary $\cB$ that solves $(L_Y,L_N)$
(which breaks the assumption of $(L_Y,L_N)\not\in\BQP$) as follows\footnote{Here,
we assume 
$\Pr[1\gets\cA(\rho_0)]<\Pr[1\gets\cA(\rho_1)]$
without loss of generality.
If
$\Pr[1\gets\cA(\rho_0)]>\Pr[1\gets\cA(\rho_1)]$,
we have only to modify $\cB$ such that
it outputs 1 if and only if $b'\neq b$.}:
On input $x\in L_Y\cup L_N$, it chooses $b\gets\bit$.
If $b=0$, it runs $b'\gets\cA(\Enc(x))$. 
If $b=1$, it runs $b'\gets\cA(\Sim_N(1^{|x|}))$. 
If $b'=b$, it outputs 1. 
If $b'\neq b$, it outputs 0. 

If $x\in L_Y$,
\begin{eqnarray*}
\Pr[1\gets\cB(x)]
&=&\frac{1}{2}\Pr[0\gets \cA(\Enc(x))]
+\frac{1}{2}\Pr[1\gets \cA(\Sim_N(1^{|x|}))]\\
&\ge&\frac{1}{2}\Pr[0\gets \cA(\rho_0)]
+\frac{1}{2}\Pr[1\gets \cA(\rho_1)]-\negl(|x|)\\
&\ge&\frac{1}{2}\Pr[0\gets \cA(\rho_0)]
+\frac{1}{2}\left(\Pr[1\gets \cA(\rho_0)]+\frac{1}{\poly(|x|)}\right)-\negl(\secp)\\
&\ge&\frac{1}{2}+\frac{1}{\poly(|x|)}.
\end{eqnarray*}
If $x\in L_N$,
\begin{eqnarray*}
\Pr[1\gets\cB(x)]
&=&\frac{1}{2}\Pr[0\gets \cA(\Enc(x))]
+\frac{1}{2}\Pr[1\gets \cA(\Sim_N(1^{|x|}))]\\
&\le&\frac{1}{2}\Pr[0\gets \cA(\rho_1)]
+\frac{1}{2}\Pr[1\gets \cA(\rho_1)]+\negl(|x|)\\
&\le&\frac{1}{2}
+\negl(|x|).
\end{eqnarray*}
We therefore have $(L_Y,L_N)\in\BQP$, which contradicts the assumption.
\end{proof}

\subsection{Preliminaries}
Let $(\mathsf{Alice},\mathsf{Bob})$ be a pair of algorithms. 
$\langle\mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle\to(\rho_A,\rho_B)$
means a classical-communication interactive algorithm between
$\mathsf{Alice}$ and $\mathsf{Bob}$ that outputs $(\rho_A,\rho_B)$,
where $\rho_A$ is the output of $\mathsf{Alice}$ 
and $\rho_B$ is the output of $\mathsf{Bob}$. 
More precisely, it is the following operations.
\begin{enumerate}
    \item 
    $\mathsf{Alice}$ generate $U|0...0\rangle$, where $U$ is a unitary.
    \item
    $\mathsf{Alice}$ measures some qubits of it to get the result (bit string) $a_1$.
    Let $|\psi_1\rangle$ be the post measurement state.
    $\Alice$ sends $a_1$ to $\Bob$.
    \item
    $\Bob$ applies a unitary $U(a_1)$ that depends on $a_1$ to $|0...0\rangle$,
    and measures some qubits of it to get the result $b_1$.
    Let $|\phi_1\rangle$ be the post measurement state.
    $\Bob$ sends $b_1$ to $\Alice$.
     \item
    $\Alice$ applies a unitary $U(b_1)$ that depends on $b_1$ to $|\psi_1\rangle$,
    and measures some qubits of it to get the result $a_2$.
    Let $|\psi_2\rangle$ be the post measurement state.
    $\Alice$ sends $a_2$ to $\Bob$.
      \item
    $\Bob$ applies a unitary $U(a_2)$ that depends on $a_2$ to $|\phi_1\rangle$,
    and measures some qubits of it to get the result $b_2$.
    Let $|\phi_2\rangle$ be the post measurement state.
    $\Bob$ sends $b_2$ to $\Alice$.
    \item
    They repeat such interactions many times. $\Alice$'s final state is $|\Psi_t\rangle$
    and $\Bob$'s final state is $|\Phi_t\rangle$,
    where $t=(a_1,b_1,a_2,b_2,...)$ is the transcript, i.e.,
    the set of all classical messages exchanged between $\Alice$ and $\Bob$.
   \item
   If some qubits of $|\Psi_t\rangle$ is traced out, the state of the remaining qubits
   is $\rho_A$, which is $\Alice$'s output.
   If some qubits of $|\Phi_t\rangle$ is traced out, the state of the remaining qubits
   is $\rho_B$, which is $\Bob$'s output.
\end{enumerate}


\subsection{EFI pairs from LQKE or RSPs}
\begin{definition}[Locally-quantum key exchange (LQKE)]
Locally-quantum key exchange (LQKE) is a set of algorithms
$(\mathsf{Alice},\mathsf{Bob})$ such that
\begin{itemize}
    \item 
    $\langle\mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle\to(a,b):$
    It is a classical-communication interactive protocol
    between a QPT algorithm $\mathsf{Alice}$
    and a QPT algorithm $\mathsf{Bob}$ that outputs $(a,b)$, where
    $a$ is a bit string that is the output of $\mathsf{Alice}$
    and
    $b$ is a bit string that is the output of $\mathsf{Bob}$.
\end{itemize}
We require 
the following two conditions.

\paragraph{\bf Correctness:}
\begin{eqnarray*}
\Pr[a=b:(a,b)\gets\langle \mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle]\ge 1-\negl(\secp).
\end{eqnarray*}

\paragraph{\bf Security:}
Let us consider the following security game between a challenger $\cC$ and an adversary $\cA$.
\begin{enumerate}
    \item 
    $\cC$ runs $(a,b)\gets\langle \mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle$.
    \item
    $\cC$ sends $\cA$ the transcript $t$ (i.e., the set of all classical messages exchanged
    between $\mathsf{Alice}$ and $\mathsf{Bob}$ obtained from the execution of $\langle \mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle$).
    \item
    $\cA$ sends a state $b'$ to $\cC$.
    \item
    $\cC$ outputs $\top$ if $b'=b$.
    $\cC$ outputs $\bot$ if $b'\neq b$.
\end{enumerate}
For any QPT adversary $\cA$, $\Pr[\top\gets\cC]\le\negl(\secp)$.
\end{definition}


\begin{definition}[Remote state preparations (RSPs)]
A remote state preparation (RSP) for a set $\{\rho_i\}_{i\in[N]}$ of states is 
a set of algorithms $(\mathsf{Alice},\mathsf{Bob})$ such that
\begin{itemize}
\item
$\langle\mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle\to(i,\rho_i):$
It is a classical-communication interactive protocol between a PPT $\mathsf{Alice}$ and
a QPT $\mathsf{Bob}$ that outputs $(i,\rho_i)$, where
$i$ is the output of $\mathsf{Alice}$ and $\rho_i$ is the output of $\mathsf{Bob}$.
\end{itemize}
We require the following two conditions.

\paragraph{\bf Correctness:}
\begin{eqnarray*}
\Pr[(i,\rho_i)\gets\langle \mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle]=\frac{1}{N}
\end{eqnarray*}
for all $i\in[N]$.

\paragraph{\bf Security:}
Let us consider the following security game between
a challenger $\cC$ and an adversary $\cA$.
\begin{enumerate}
    \item 
    $\cC$ and $\cA$ run $(i,\sigma)\gets\langle\mathsf{Alice}(1^\secp),\cA\rangle$,
    where $\cC$ honestly runs $\mathsf{Alice}$.
    \item
    $\cA$ sends $i'$ to $\cC$.
    \item
    If the first $\ell$ bits of $i'$ are equal to those of $i$,
    $\cC$ outputs $\top$.
    Otherwise, $\cC$ outputs $\bot$.
    (Here, $\ell$ depends on
which states $\{\rho_i\}_i$ are considered
and which ``classical secret'' of $\rho_i$ should be protected.
See the remark below.)
\end{enumerate}
For any QPT $\cA$,
\begin{eqnarray*}
\Pr[\cC\to\top]\le \negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{remark}
For example, if we are interested in
a RSP of ``random BB84 states'',
$\rho_i=\otimes_{j=1}^m H^{h_j}|b_j\rangle$,
we take
$i=(h,b)\in\bit^m\times\bit^m$, 
and $\ell=m$
in the above definition
(i.e., the security means that $\cA$ cannot learn $h$.)
On the other hand,
if we are interested in
a RSP for ``superpositions of two states'',
$\rho_i=|x_0\rangle+|x_1\rangle$, 
we take
$i=(x_0,x_1)\in\bit^m\times\bit^m$,
and $\ell=2m$ in the above definition
(i.e., the security means that $\cA$ cannot learn both $x_0$ and $x_1$.)
\end{remark}

\begin{theorem}
\label{thm:LQKE}
If LQKE schemes exist, then EFI pairs exist.
\end{theorem}

\begin{remark}
The existence of LQKE schemes imply the existence of
classical KE schemes, and therefore the above theorem also means that
if (quantum-secure classical) KE schemes exist then EFI pairs exist.
\end{remark}

\begin{proof}[Proof of \cref{thm:LQKE}]
For simplicitly, we show the result for the perfectly-correct case.
A similar proof holds for $1-\negl(\secp)$ correct case.
In a LQKE scheme, Alice and Bob run QPT algorithms,
and exchange classical messages over a classical channel.
We can write the entire computation between Alice and Bob
as a single
quantum computation with intermediate measurements by Alice and Bob.
We can then express the quantum computation with a single unitary $U$ 
by ``postponing'' all measurements done by Alice and Bob to the end of the computation.
In other words,
there is a QPT unitary $U$ such that
\begin{eqnarray*}
U|0...0\rangle=\sum_{t}\sqrt{\Pr[t]}|t\rangle|a(t)\rangle|\eta_t\rangle, 
\end{eqnarray*}
where $t$ is the transcript
(i.e., the set of all classical messages exchanged between Alice and Bob),
$\Pr[t]$ is the probability that the transcript $t$ occurs,
$a(t)$ is Alice's output, and
$\{|\eta_t\rangle\}_t$ are some normalized states for Alice's ancilla system and Bob's system.

From the $U$, we construct a statistically-hiding and computationally-binding
canonical quantum bit commitment scheme $\{Q_0,Q_1\}$ as follows.
(Due to \cref{thm:convertingflavors}, we then have a statistically-binding and computationally-hiding
canonical quantum bit commitment scheme which is equivalent to an EFI pair.)
\begin{eqnarray*}
Q_0|0\rangle_{\regC,\regR}&\coloneqq& \sum_t\sqrt{\Pr[t]}
|t,a(t),\eta_t\rangle_{\regC}|t\rangle_{\regR_1}|0\rangle_{\regR_2},\\
Q_1|0\rangle_{\regC,\regR}&\coloneqq& \sum_t\sqrt{\Pr[t]}
|t,a(t),\eta_t\rangle_{\regC}|t\rangle_{\regR_1}|a(t)\rangle_{\regR_2},
\end{eqnarray*}
where $\regR\coloneqq(\regR_1,\regR_2)$.

First we show that $\{Q_0,Q_1\}$ is computationally binding.
Assume that it is not. Then, there exist a QPT unitary $V$, a polynomial $p$,
and an ancilla state
$|\tau\rangle_\regZ$ such that
\begin{eqnarray*}
\|
(\langle 0|Q_1^\dagger)_{\regC,\regR} V_{\regR,\regZ}(Q_0|0\rangle_{\regC,\regR}\otimes|\tau\rangle_\regZ)
\|
\ge\frac{1}{p}.
\end{eqnarray*}
Then,
\begin{eqnarray}
\frac{1}{p^2}
&\le&
\|
(\langle 0|Q_1^\dagger)_{\regC,\regR} V_{\regR,\regZ}(Q_0|0\rangle_{\regC,\regR}\otimes|\tau\rangle_\regZ)
\|^2\nonumber\\
&=&
\Big\|
\Big(\sum_{t'}\sqrt{\Pr[t']}\langle t',a(t'),\eta_{t'}|_{\regC}
\langle {t'}|_{\regR_1}
\langle a(t')|_{\regR_2}\Big)\nonumber\\
&&\times\Big(\sum_{t}\sqrt{\Pr[t]}|t,a(t),\eta_t\rangle_{\regC}V_{\regR,\regZ}
|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ\Big)
\Big\|^2\nonumber\\
&=&
\Big\|
\sum_{t}\Pr[t]
\langle t|_{\regR_1}
\langle a(t)|_{\regR_2}
V_{\regR,\regZ}
|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ
\Big\|^2\nonumber\\
&\le&
\sum_{t}\Pr[t]
\Big\|
\langle t|_{\regR_1}
\langle a(t)|_{\regR_2}
V_{\regR,\regZ}
|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ
\Big\|^2\nonumber\\
&\le&
\sum_{t}\Pr[t]
\Big\|
\langle a(t)|_{\regR_2}
V_{\regR,\regZ}
|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ
\Big\|^2\label{KE_attack}.
\end{eqnarray}
From this $V$, we construct a QPT Eve
that breaks the security of the LQKE
as follows:
Given the transcript $t$, 
it applies $V_{\regR,\regZ}$ on
$|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ$, and measures
the $\regR_2$ register in the computational basis. Output the result.
Then, the probability that Eve
outputs $a(t)$ is equal to Eq.~(\ref{KE_attack}).
Therefore, Eve breaks the security
of the LQKE.

We next show that $\{Q_0,Q_1\}$ is statistically hiding.
There exists a (unbounded-time) unitary $W$ such that
$W(|t\rangle_{\regR_1}|0\rangle_{\regR_2}|0\rangle_\regZ)=
|t\rangle_{\regR_1}|a(t)\rangle_{\regR_2}|0\rangle_\regZ$ for all $t$.
In fact, the following algorithm works.
\begin{enumerate}
    \item 
    Given $t$, $W$ classically computes the
classical description of Alice's final quantum state, i.e. 
the state which Alice gets $a(t)$ if she measures some qubits of.
\item
From the classical description of Alice's final quantum state, $W$ computes $a(t)$.
\item
$W$ writes $a(t)$ on the register $\regR_2$.
\item
$W$ does the inverse of the above computation to reset the state of the registers $\regR_1$ and $\regZ$
to the initial state $|t\rangle_{\regR_1}|0\rangle_\regZ$.
\end{enumerate}
Then, we have
\begin{eqnarray*}
\|W_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ
-Q_1|0\rangle_{\regC,\regR}|0\rangle_\regZ \|_1
=0,
\end{eqnarray*}
which means the statistical hiding.
\end{proof}



\begin{theorem}
If RSPs exist, then EFI pairs exist.
\end{theorem}

\begin{proof}
In a RSP, $\cS$ runs a PPT algorithm and $\cR$ runs a QPT algorithm.
They exchange classical messages over a classical channel.
We can write the entire computation between $\cS$ and $\cR$ as a single
quantum computation with intermediate measurements by $\cS$ and $\cR$.
We can then express the quantum computation with a single unitary $U$ 
by ``postponing'' all measurements done by $\cS$ and $\cR$ to the end of the computation.
In other words,
there is a QPT unitary $U$ such that
\begin{eqnarray*}
U|0\rangle=\sum_t\sqrt{\Pr[t]}|t\rangle|i(t)\rangle|\eta_t\rangle, 
\end{eqnarray*}
where $t$ is the transcript
(i.e., the set of all classical messages exchanged between $\cS$ and $\cR$),
$\Pr[t]$ is the probability that the transcript $t$ occurs,
and $\{|\eta_t\rangle\}_t$ are some normalized states.

From the $U$, we construct a statistically-hiding and computationally-binding
canonical quantum bit commitment scheme $\{Q_0,Q_1\}$ as follows.
\begin{eqnarray*}
Q_0|0\rangle_{\regC,\regR}&\coloneqq& \sum_t\sqrt{\Pr[t]}
|t,i(t),\eta_t\rangle_{\regC}|t\rangle_{\regR_1}|0\rangle_{\regR_2},\\
Q_1|0\rangle_{\regC,\regR}&\coloneqq& \sum_t\sqrt{\Pr[t]}
|t,i(t),\eta_t\rangle_{\regC}|t\rangle_{\regR_1}|i(t)\rangle_{\regR_2}.
\end{eqnarray*}

First we show that $\{Q_0,Q_1\}$ is computationally binding.
Assume that it is not. Then, there exists a QPT unitary $V$ and an ancilla state
$|\tau\rangle_\regZ$ such that
\begin{eqnarray*}
\|
(\langle 0|Q_1^\dagger)_{\regC,\regR} V_{\regR,\regZ}(Q_0|0\rangle_{\regC,\regR}\otimes|\tau\rangle_\regZ)
\|
\ge\frac{1}{p}.
\end{eqnarray*}
Then,
\begin{eqnarray}
\frac{1}{p^2}
&\le&
\|
(\langle 0|Q_1^\dagger)_{\regC,\regR} V_{\regR,\regZ}(Q_0|0\rangle_{\regC,\regR}\otimes|\tau\rangle_\regZ)
\|^2\nonumber\\
&=&
\Big\|
\Big(\sum_{t'}\sqrt{\Pr[t']}\langle t',i(t'),\eta_{t'}|_{\regC}
\langle {t'}|_{\regR_1}
\langle i(t')|_{\regR_2}\Big)\nonumber\\
&&\times\Big(\sum_{t}\sqrt{\Pr[t]}|t,i(t),\eta_t\rangle_{\regC}V_{\regR,\regZ}
|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ\Big)
\Big\|^2\nonumber\\
&=&
\Big\|
\sum_{t}\Pr[t]
\langle t|_{\regR_1}
\langle i(t)|_{\regR_2}
V_{\regR,\regZ}
|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ
\Big\|^2\nonumber\\
&\le&
\sum_{t}\Pr[t]
\Big\|
\langle t|_{\regR_1}
\langle i(t)|_{\regR_2}
V_{\regR,\regZ}
|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ
\Big\|^2\nonumber\\
&\le&
\sum_{t}\Pr[t]
\Big\|
\langle i(t)|_{\regR_2}
V_{\regR,\regZ}
|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ
\Big\|^2\label{RSP_attack}.
\end{eqnarray}
From this $V$, we construct a QPT adversary $\cR^*$ 
that breaks the security of the RSP
as follows:
It first honestly runs the RSP protocol with $\cS$.
Given the transcript $t$, 
it applies $V_{\regR,\regZ}$ on
$|t\rangle_{\regR_1}|0\rangle_{\regR_2}|\tau\rangle_\regZ$, and measure
the $\regR_2$ register in the computational basis. Output the result.
Then, the probability that $\cR^*$
output $i(t)$ is equal to Eq.~(\ref{RSP_attack}).
Therefore, $\cR^*$ breaks the security
of the RSP.

Next we show that $\{Q_0,Q_1\}$ is statistically hiding.
There exists a (unbounded-time) unitary $W$ such that
$W(|t\rangle_{\regR_1}|0\rangle_{\regR_2}|0\rangle_\regZ)=
|t\rangle_{\regR_1}|i(t)\rangle_{\regR_2}|0\rangle_\regZ$.
In fact, the following algorithm works.
\begin{enumerate}
    \item 
    Given $t$, $W$ classically computes 
    the classical description of $\cR$'s state.
    \item
    From the classical description of the state, $W$ computes $i(t)$.
    \item
    $W$ write $i(t)$ on the register $\regR_2$.
    \item
$W$ does the inverse of the above computation to reset the state of the registers $\regR_1$ and $\regZ$.
\end{enumerate}
Then, we have
\begin{eqnarray*}
\|W_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ
-Q_1|0\rangle_{\regC,\regR}|0\rangle_\regZ \|_1
=0,
\end{eqnarray*}
which means the statistical hiding.
\end{proof}


\subsection{ISGs}

\begin{definition}[Interactive states generations (ISGs)]
An interactive states generation (ISG)
is a set of algorithms $(\mathsf{Alice},\mathsf{Bob},\Ver)$ such that
\begin{itemize}
    \item 
    $\langle\mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle\to(\rho_A,\rho_B):$
    It is a classical-communication interactive algorithm between a QPT or PPT algorithm $\mathsf{Alice}$
    and a QPT algorithm $\mathsf{Bob}$ that outputs $(\rho_A,\rho_B)$,
    where $\rho_A$ is the output of $\mathsf{Alice}$ and $\rho_B$ is the output of
    $\mathsf{Bob}$. (If $\mathsf{Alice}$ is PPT, $\rho_A$ is a bit string.)
    \item
$\Ver(\rho_A,\sigma)\to\top/\bot:$ It is a QPT algorithm that, on input 
$\rho_A$ and a quantum state $\sigma$, outputs $\top/\bot$.
\end{itemize}
We require the following two conditions.

\paragraph{\bf Correctness:}
\begin{eqnarray*}
\Pr[\top\gets\Ver(\rho_A,\rho_B):(\rho_A,\rho_B)\gets\langle \mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle]
\ge1-\negl(\secp).
\end{eqnarray*}

\paragraph{\bf Security:}
Let us consider the following security game between a challenger $\cC$ and an adversary $\cA$.
\begin{enumerate}
    \item 
    $\cC$ runs $(\rho_A,\rho_B)\gets\langle \mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle$.
    \item
    $\cC$ sends $\cA$ the transcript $t$ (i.e., the set of all classical messages exchanged
    between $\mathsf{Alice}$ and $\mathsf{Bob}$ obtained from the execution of $\langle \mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle$).
    \item
    $\cA$ sends a state $\sigma$ to $\cC$.
    \item
    $\cC$ runs $\Ver(\rho_A,\sigma)$,
    and outputs its output.
\end{enumerate}
For any QPT adversary $\cA$, $\Pr[\top\gets\cC]\le\negl(\secp)$.
\end{definition}



\begin{definition}[Semi-quantum tokenized signature \cite{cryptoeprint:2022/228}]
A semi-quantum tokenized signature scheme is a set of
algorithms $(\mathsf{Sen},\mathsf{Rec},\mathsf{QV},\Sign,\mathsf{CV})$ 
such that
\begin{itemize}
\item
 $\langle\mathsf{Sen}(1^\secp),\mathsf{Rec}(1^\secp)\rangle\to
 (\pk,|\mathsf{qt}\rangle_\pk):$
It is a classical-communication protocol between a PPT
algorithm $\mathsf{Sen}$ and a QPT algorithm $\mathsf{Rec}$. 
At the end of interaction the $\mathsf{Sen}$ outputs a classical
public key $\pk$ and $\mathsf{Rec}$ outputs a quantum state $|\mathsf{qt}\rangle_\pk$.   
\item 
$\mathsf{QV}(\pk,|\mathsf{qt}\rangle_\pk)\to 
(b,|\mathsf{qt}\rangle_\pk'):$
It is a QPT algorithm that, on input $\pk$ and 
a candidate token $|\mathsf{qt}\rangle_\pk$,
outputs a token $|\mathsf{qt}\rangle_\pk'$
and a bit $b\in\bit$.
\item
$\Sign(\pk,|\mathsf{qt}\rangle_\pk,b)\to
\sigma_b:$ 
It is a QPT algorithm that, on input $\pk$, a candidate token
$|\mathsf{qt}\rangle_\pk$ and a bit $b\in\bit$,
outputs a classical string $\sigma_b$.
\item
$\mathsf{CV}(\pk,\sigma_b,b)\to b':$
It is a classical polynomial-time deterministic algorithm that, on input
$\pk$, $\sigma_b$ and a bit $b\in\bit$,
outputs a bit $b'\in\bit$.
\end{itemize}
We require the following two properties. (\cite{cryptoeprint:2022/228} requires
other more properties, but here we write only the ones necessary for our result.)

\paragraph{\bf Correctness:}
\begin{eqnarray*}
\Pr[(1,|\mathsf{qt}\rangle_\pk')\gets \mathsf{QV}(\pk,|\mathsf{qt}\rangle_\pk):(\pk,|\mathsf{qt}\rangle_\pk)\gets\langle\mathsf{Sen}(1^\secp),\mathsf{Rec}(1^\secp)\rangle]
\ge1-\negl(\secp).
\end{eqnarray*}

\paragraph{\bf Security:}
For any QPT adversary $\cA$,
\begin{eqnarray*}
\Pr[1\gets\mathsf{CV}(\pk,\sigma_0,0)\wedge 1\gets\mathsf{CV}(\pk,\sigma_1,1):
(\pk,(\sigma_0,\sigma_1))\gets\langle\mathsf{Sen}(1^\secp),\cA\rangle
]
\le\negl(\secp).
\end{eqnarray*}

\end{definition}


\begin{definition}[Semi-quantum money (SQM)~\cite{CoRR:RadSat19}]
\end{definition}

\begin{definition}[Public-key semi-quantum money (PKSQM)\cite{STOC:Shmueli22}]
A public-key semi-quantum money scheme (PKSQM) is a set of algorithms
$(\mathsf{Bank},\mathsf{Rec},\mathsf{QV},\mathsf{GenCert},\mathsf{CV})$
such that
\begin{itemize}
    \item 
    $\langle\mathsf{Bank}(1^\secp),\mathsf{Rec}(1^\secp)\rangle\to(\pk,\$_\pk):$
    It is an interactive protocol between the PPT $\mathsf{Bank}$
    and the QPT $\mathsf{Rec}$. The output of $\mathsf{Bank}$ is $\pk$
    and the output of $\mathsf{Rec}$ is $\$_\pk$.
    \item
    $\mathsf{QV}(\pk,\$)\to(b,\$'):$
    It is a QPT algorithm that, on input $\pk$ and a candidate banknote $\$$,
    outputs a bit $b\in\bit$ and a quantum state $\$'$.
    \item
    $\mathsf{GenCert}(\pk,\$)\to\mathsf{crt}:$
    It is a QPT algorithm that, on input $\pk$ and a candidate banknote $\$$,
    outputs a bit string $\mathsf{crt}$.
     \item
    $\mathsf{CV}(\pk,\mathsf{crt})\to b:$
    It is a classical deterministic polynomial-time algorithm that, 
    on input $\pk$ and $\mathsf{crt}$,
    outputs a bit $b\in\bit$.
\end{itemize}
We require the following properties. (The definition in \cite{STOC:Shmueli22} actually
requires more properties, but here we write only ones necessary for our results.)

\paragraph{\bf Correctness:}
\begin{eqnarray*}
\Pr[\top\gets\mathsf{QV}(\pk,\$_\pk):(\pk,\$_\pk)\gets\langle\mathsf{Bank}(1^\secp),\mathsf{Rec}(1^\secp)\rangle]
\ge1-\negl(\secp).
\end{eqnarray*}

\paragraph{\bf Security:}
For any QPT $\mathsf{Rec}^*$,
\begin{eqnarray*}
\Pr[1\gets\mathsf{QV}(\pk,\$)\wedge 1\gets\mathsf{CV}(\pk,\mathsf{crt}):
(\pk,(\$,\mathsf{crt}))\gets\langle\mathsf{Bank}(1^\secp),\mathsf{Rec}^*\rangle]
\le\negl(\secp).
\end{eqnarray*}
\end{definition}


\begin{theorem}
If LQKE schemes exist, then ISGs exist.
\end{theorem}

\begin{proof}
As $(\mathsf{Alice},\mathsf{Bob})$ of an ISG,
we take that of a LQKE scheme.
As $\Ver$ of the ISG, we take the following algorithm:
It outputs $\top$ if and only if $b=b'$.
\end{proof}

\begin{theorem}
If RSPs exist, then ISGs exist.
\end{theorem}

\begin{proof}
As $(\mathsf{Alice},\mathsf{Bob})$ of an ISG,
we take that of a RSP.
$\Ver$ is the algorithm that outputs $\top$ if and only if
$\sigma$ corresponds to $i$.
Assume that thus constructed ISG is broken by a QPT adversary $\cA$.
Then, from the $\cA$, we can construct
a QPT adversary $\cB$ that breaks the RSP as follows:
It honestly runs $\mathsf{Bob}$ of the RSP.
Then from the transcript, it generate $\rho_i$.
\end{proof}

\begin{theorem}
If semi-quantum money schemes exist, then ISGs exist.
\end{theorem}



\begin{theorem}
If public-key semi-quantum money schemes exist, then ISGs exist.
\end{theorem}

\begin{proof}
As the interactive protocol of a ISG,
we take that of a PKSQM.
$\rho_A$ is Alice's output (a bit string $\pk$),
and
$\rho_B$ is Bob's output (a quantum state $\$_\pk$).
$\Ver$ is the algorithm that outputs $\top$ if and only if
$\top\mathsf{QVer}(\pk,\sigma)$.
Assume that thus constructed LQSG is broken by a QPT adversary $\cA$.
Then, it is clear that the $\cA$ also breaks the RKSQM.
\end{proof}

\begin{theorem}
If classical channel certified deletion exists then ISGs exist.
\end{theorem}

\begin{theorem}
If one-shot signatures exist then ISGs exist.
\end{theorem}

\begin{theorem}
If quantum lightning exist then ISGs exist.
\end{theorem}

\begin{theorem}
If semi-quantum tokenized signatures exist then ISGs exist.
\end{theorem}



\subsection{State transformations}
\begin{definition}[State transformations (STs)]
A state transformation (ST) is a set of algorithms $(\StateGen,\Ver)$ such that
\begin{itemize}
\item
$\StateGen(1^\secp)\to\rho_{\regC,\regA}:$
It is a QPT algorithm that, on input the security parameter $\secp$, outputs 
a state $\rho_{\regC,\regA}$ over the two registers $\regC$ and $\regA$.
($\regC$ is called the challenger register and
$\regA$ is called the adversary register.)
\item
$\Ver(\rho'_{\regC,\regA})\to\top/\bot:$
It is a QPT algorithm that, on input a quantum state $\rho'_{\regC,\regA}$
over the registers $\regC$ and $\regA$,
outputs $\top/\bot$.
\end{itemize}

Let us consider the following security game between a challenger
$\cC$ and an adversary $\cA$.
\begin{enumerate}
    \item 
    $\cC$ runs $\rho_{\regC,\regA}\gets\StateGen(1^\secp)$.
    \item
    $\cC$ sends the register $\regA$ to $\cA$.
    \item
    $\cA$ returns the register $\regA$ to $\cC$.
    \item
    $\cC$ runs $\Ver$ on the state,
    and outputs the result.
\end{enumerate}

We require the following two properties.

\paragraph{\bf Statistical insecurity:}
There exists a unbounded adversary $\cA$ such that
$\Pr[\cC\to\top]\ge\frac{1}{\poly(\secp)}$.

\paragraph{\bf Computational security:}
For any QPT adversary $\cA$,
$\Pr[\cC\to\top]\le\negl(\secp)$.
\end{definition}

\begin{theorem}
If EFI pairs exist, then STs exist.
\end{theorem}

\begin{proof}
Let $\{Q_0,Q_1\}$ be a computationally-binding and statistically-hiding
quantum canonical bit commitment.
If an EFI pair exists, such a commitment exists.
From the commitment, we construct a ST as follows.
\begin{itemize}
\item 
$\StateGen(1^\secp)\to\rho_{\regC,\regA}:$
Generate $Q_0|0\rangle_{\regC,\regR}$,
and output $\rho_{\regC,\regA}\coloneqq Q_0|0\rangle_{\regC,\regR}$.
\item
$\Ver(\rho_{\regC,\regA}')\to\top/\bot:$
Parse
$\rho_{\regC,\regA}=Q_0|0\rangle_{\regC,\regR}$.
Apply $Q_1^\dagger$ on the state, and measure all qubits.
If all the results are 0, output $\top$. Otherwise, output $\bot$.
\end{itemize}
The computational security comes from
the computational binding, 
and
the statistical insecurity comes from
the statistical hiding. 
\end{proof}

\begin{theorem}
If OWSGs exist, then STs exist.
\end{theorem}

\begin{proof}
Let $(\mathsf{OWSG}.\KeyGen,\mathsf{OWSG}.\StateGen,\mathsf{OWSG}.\Ver)$ be a OWSG.
From it, we construct a ST as follows.
\begin{itemize}
\item 
$\StateGen(1^\secp)\to\rho_{\regC,\regA}:$
Run $\mathsf{OWSG}.\KeyGen$ and $\mathsf{OWSG}.\StateGen$ to
generate 
\begin{eqnarray*}
\sum_k\Pr[k\gets\mathsf{OWSG}.\KeyGen(1^\secp)]|k\rangle\langle k|_\regC
\otimes 
(\phi_k^{\otimes t})_\regA,
\end{eqnarray*}
and output it as $\rho_{\regC,\regA}$.
\item
$\Ver(\rho_{\regC,\regA}')\to\top/\bot:$
Measure $\regC$ to get $k$,
and measure $\regA$ to get $k'$.
Run $\mathsf{OWSG}.\Ver(k',\phi_k)$,
and output the result.
\end{itemize}
The computational security comes from the security of the OWSG.
The statistical insecurity comes from the fact that OWSG is broken by
a unbounded adversary by using the shadow tomography.
\end{proof}

\begin{theorem}
If ISGs exist, then STs exist.
\end{theorem}

\begin{proof}
Let $(\mathsf{Alice},\mathsf{Bob},\mathsf{ISG}.\Ver)$ be an ISG.
\if0
We can express $\langle\mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle$
with a single QPT unitary $U$ by ``postponing'' all measurements done by 
$\mathsf{Alice}$ and $\mathsf{Bob}$ to the end of the algorithm.
In other words,
there is a QPT unitary $U$ such that
\begin{eqnarray*}
U|0...0\rangle=\sum_t\sqrt{\Pr[t]}|t\rangle|\Psi_t\rangle|\Phi_t\rangle, 
\end{eqnarray*}
where $t$ is the transcript,
$\Pr[t]$ is the probability that the transcript $t$ occurs,
$|\Psi_t\rangle$ and $|\Phi_t\rangle$ are the final states of $\mathsf{Alice}$
and $\mathsf{Bob}$ when the transcript is $t$, respectively.
The output state 
$\rho_A$ $(\rho_B)$ 
of $\mathsf{Alice}$ ($\mathsf{Bob}$) 
is obtained if
some qubits of $|\Psi_t\rangle$ $(|\Phi_t\rangle)$ are traced out.
\fi

From it, we construct a ST as follows.
\begin{itemize}
    \item 
    $\StateGen(1^\secp)\to\rho_{\regC,\regA}:$
    Run $\langle\mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle$
    to generate
    \begin{eqnarray*}
\sum_t \Pr[t] 
(\rho_A(t)
\otimes
\rho_B(t))_\regC
\otimes |t\rangle\langle t|_{\regA},
\end{eqnarray*}
and output it as $\rho_{\regC,\regA}$.
Here $t$ is the transcript and $\Pr[t]$ is the probability that
the transcript $t$ occurs.
\item
$\Ver(\rho_{\regC,\regA}')\to\top/\bot:$
Apply $\mathsf{ISG}.\Ver$ on $\rho_A(t)$ and the state
of $\regA$.
Output the result.
\end{itemize}
The computational security comes from the security of the ISG.
The statistical insecurity comes from the fact that
$\rho_A$ and $\rho_B$ can be generated from the transcript in a unbounded time.
(Repeat $\langle\mathsf{Alice}(1^\secp),\mathsf{Bob}(1^\secp)\rangle$ many times
until the transcript $t$ occurs.)
\end{proof}

==> SCCU.tex <==
\section{SCCUs}
\label{sec:SCCU}
\mor{kono section subete kentoutyuu}

\subsection{Definition of SCCUs}
\begin{definition}[Statistically-clonable but computationally-unclonable states generators (SCCUs)]
A statistically-clonable but computationally-unclonable states generator (SCCU) is a set of algorithms
$(\KeyGen,\StateGen)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$ It is a QPT algorithm that, on input the security parameter $\secp$, outputs
    a classical key $k\in\bit^\kappa$.
    \item
    $\StateGen(k)\to|\phi_k\rangle:$ It is a QPT algorithm that, on input $k$,
    outputs an $m$-qubit state $|\phi_k\rangle$.
\end{itemize}
We require the following two properties.

\paragraph{\bf $t_1$-statistical-clonability:}
There exists a (unbounded-time) quantum operation $\cE$ such that
\begin{eqnarray*}
\langle\phi_k|^{\otimes t_1+1}\cE(|\phi_k\rangle^{\otimes t_1})|\phi_k\rangle^{\otimes t_1+1}\ge1-\negl(\secp)
\end{eqnarray*}
for all $k$.

\paragraph{\bf $t_2$-computational-unclonability:}
For any QPT quantum operation $\cE$,
\begin{eqnarray*}
\sum_k\Pr[k\gets\KeyGen(1^\secp)]\langle\phi_k|^{\otimes t_2+1}\cE(|\phi_k\rangle^{\otimes t_2})|\phi_k\rangle^{\otimes t_2+1}\le\negl(\secp).
\end{eqnarray*}
\end{definition}


\subsection{EFI pairs from SCCUs}
\begin{theorem}
If SCCUs with any $t_1$ and $t_2$ such that $t_2\ge t_1\ge 1$ exist then EFI pairs exist.
\end{theorem}

\begin{proof}
Let $(\mathsf{SCCU}.\KeyGen,\mathsf{SCCU}.\StateGen)$
be a SCCU with any $t_1$ and $t_2$ such that $t_2\ge t_1\ge1$. 
Without loss of generality, we can assume that
$\mathsf{SCCU}.\KeyGen$ is the following algorithm:
first apply a QPT unitary $U$ on $|0...0\rangle$ to generate 
\begin{eqnarray*}
U|0...0\rangle=\sum_{k}\sqrt{\Pr[k\gets\mathsf{SCCU}.\KeyGen(1^\secp)]}|k\rangle|\mu_k\rangle, 
\end{eqnarray*}
and trace out the second register,
where $\{|\mu_k\rangle\}_k$ are some normalized states.
Moreover, without loss of generality, we can also assume that $\mathsf{SCCU}.\StateGen$ is the following algorithm:
first apply a QPT unitary $V_k$ that depends on $k$ on $|0...0\rangle$ to generate 
$V_k|0...0\rangle=|\phi_k\rangle|\eta_k\rangle$, and then trace out the second register.

From the SCCU, we construct statistically-hiding and computationally-binding canonical quantum bit
commitment scheme $\{Q_0,Q_1\}$. From \cref{thm:convertingflavors}, we then have
statistically-binding and computationally-hiding canonical quantum bit commitment scheme, which is equivalent to an EFI pair.
We define $\{Q_0,Q_1\}$ as follows.
\begin{eqnarray*}
Q_0|0\rangle_{\regC,\regR}&\coloneqq& \sum_{k}\sqrt{\Pr[k]}|k,\mu_k\rangle_{\regC}|\phi_k\rangle_{\regR_1}^{\otimes t_2-t_1}|\phi_k\rangle_{\regR_2}^{\otimes t_1}\otimes|0\rangle_{\regR_3},\\
Q_1|0\rangle_{\regC,\regR}&\coloneqq& \sum_{k}\sqrt{\Pr[k]}|k,\mu_k\rangle_{\regC}|\phi_k\rangle_{\regR_1}^{\otimes t_2-t_1}|\phi_k\rangle_{\regR_2}^{\otimes t_1}\otimes|\phi_k\rangle_{\regR_3},\\
\end{eqnarray*}
where $\Pr[k]\coloneqq\Pr[k\gets\mathsf{SCCU}.\KeyGen(1^\secp)]$
and $\regR\coloneqq(\regR_1,\regR_2,\regR_3)$.
If $t_2=t_1$, we ignore the register $\regR_1$.
It is clear that $\{Q_0,Q_1\}$ are implementable in QPT in a natural way.

First let us show its computational binding.
Assume that it is not computational binding. Then there exists a QPT unitary $U$, an ancilla state $|\tau\rangle_\regZ$,
and a polynomial $p$ such that
\begin{eqnarray*}
\|(\langle 0|Q_1^\dagger)_{\regC,\regR} U_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|\tau\rangle_{\regZ}\|\ge\frac{1}{p}.
\end{eqnarray*}
Then we have
\begin{eqnarray}
\frac{1}{p^2}&\le&
\|(\langle 0|Q_1^\dagger)_{\regC,\regR} U_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|\tau\rangle_{\regZ}\|^2\nonumber\\
&=&
\Big\|\Big(\sum_k\sqrt{\Pr[k]}\langle k,\mu_k|_\regC\langle \phi_k|_{\regR_1,\regR_2}^{\otimes t_2}\langle\phi_k|_{\regR_3}\Big)\nonumber\\
&&\times U_{\regR,\regZ}
\Big(\sum_k\sqrt{\Pr[k]}|k,\mu_k\rangle_\regC|\phi_k\rangle_{\regR_1,\regR_2}^{\otimes t_2}|0\rangle_{\regR_3}|\tau\rangle_\regZ\Big)\Big\|^2\nonumber\\
&=&
\Big\|\sum_k\Pr[k]
\langle \phi_k|_{\regR_1,\regR_2}^{\otimes t_2}\langle\phi_k|_{\regR_3}
U_{\regR,\regZ}
|\phi_k\rangle_{\regR_1,\regR_2}^{\otimes t_2}|0\rangle_{\regR_3}|\tau\rangle_\regZ\Big\|^2\nonumber\\
&\le&
\sum_k\Pr[k]
\Big\|
\langle \phi_k|_{\regR_1,\regR_2}^{\otimes t_2}\langle\phi_k|_{\regR_3}
U_{\regR,\regZ}
|\phi_k\rangle_{\regR_1,\regR_2}^{\otimes t_2}|0\rangle_{\regR_3}|\tau\rangle_\regZ\Big\|^2.
\label{SCCU_B}
\end{eqnarray}
From this $U_{\regR,\regZ}$, we construct a QPT adversary $\cB$ that breaks
the $t_2$-computational unclonability of SCCU as follows:
On input $|\phi_k\rangle^{\otimes t_2}$, apply $U_{\regR,\regZ}$ on $|\phi_k\rangle_{\regR_1,\regR_2}^{\otimes t_2}|0\rangle_{\regR_2}|\tau\rangle_\regZ$,
and output the state of the register $\regR$. 
The probability that the $\cB$ breaks $t_2$-computational-unclonability is equal to Eq.~(\ref{SCCU_B}),
which is non-negligible.
The $\cB$ therefore breaks $t_2$-computational-unclonability of the SCCU.

Next let us show the statistical hiding of $\{Q_0,Q_1\}$.
From the $t_1$-statistical clonability of SCCU,
there exists a (unbounded-time) quantum operation $\cE$ such that
\begin{eqnarray*}
\langle\phi_k|^{\otimes t_1+1}\cE(|\phi_k\rangle^{\otimes t_1})|\phi_k\rangle^{\otimes t_1+1}\ge1-\negl(\secp)
\end{eqnarray*}
for all $k$.
Let $U$ be the unitary version of $\cE$. In other words,
\begin{eqnarray*}
U_{\regR_2,\regZ,\regZ'}|\phi_k\rangle^{\otimes t_1}_{\regR_2}|0\rangle_{\regZ}|0\rangle_{\regZ'}&=&
\sqrt{1-\epsilon_k}|\phi_k\rangle^{\otimes t_1}_{\regR_2}|\phi_k\rangle_{\regZ}|junk_k\rangle_{\regZ'}\\
&&+\sum_{i}\sqrt{\epsilon_{k,i}}|\eta_{k,i}\rangle_{\regR_2,\regZ}|junk_{k,i}\rangle_{\regZ'},
\end{eqnarray*}
where $1-\epsilon_k\ge1-\negl(\secp)$, $|junk_k\rangle$ and $|junk_{k,i}\rangle$ are normalized states, and
$\{|\phi_k\rangle^{\otimes t_1+1}\}\cup\{|\eta_{k,i}\rangle\}_i$
is an orthonormal basis.
Let us define $V_{\regR_2,\regR_3,\regZ,\regZ'}$ by a unitary that applies
$U_{\regR_2,\regZ,\regZ'}$ and then swaps $\regR_3$ and $\regZ$.
Define $W_{\regR_2,\regR_3,\regZ,\regZ'}\coloneqq U_{\regR_2,\regZ,\regZ'}^\dagger V_{\regR_2,\regR_3,\regZ,\regZ'}$.

Then,
\begin{eqnarray*}
&&\Big((\langle0|Q_1^\dagger)_{\regC,\regR}\langle 0|_\regZ\langle0|_{\regZ'}\Big)
\Big(W_{\regR_2,\regR_3,\regZ,\regZ'}Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ|0\rangle_{\regZ'}\Big)\\
&=&
\Big((\langle0|Q_1^\dagger)_{\regC,\regR}\langle 0|_\regZ\langle0|_{\regZ'}U_{\regR_2,\regZ,\regZ'}^\dagger\Big)
\Big(V_{\regR_2,\regR_3,\regZ,\regZ'}Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ|0\rangle_{\regZ'}\Big)\\
&=&
\Big(\sum_k\sqrt{\Pr[k]}\langle k,\mu_k|_\regC\langle\phi_k|_{\regR_1}^{\otimes t_2-t_1}
\Big[\sqrt{1-\epsilon_k}\langle \phi_k|_{\regR_2}^{\otimes t_1}
\langle \phi_k|_{\regZ}\langle junk_k|_{\regZ'}
\langle \phi_k|_{\regR_3}\\
&&+\sum_{i}\sqrt{\epsilon_{k,i}}\langle\eta_{k,i}|_{\regR_2,\regZ}\langle junk_{k,i}|_{\regZ'}\langle\phi_k|_{\regR_3} \Big]\Big)\\
&&\times\Big(\sum_k\sqrt{\Pr[k]}|k,\mu_k\rangle_{\regC}|\phi_k\rangle_{\regR_1}^{\otimes t_2-t_1}
\Big[\sqrt{1-\epsilon_k}|\phi_k\rangle_{\regR_2}^{\otimes t_1}|0\rangle_{\regZ}|junk_k\rangle_{\regZ'}|\phi_k\rangle_{\regR_3}\\
&&+\sum_i\sqrt{\epsilon_{k,i}}|\eta_{k,i}'\rangle_{\regR_2,\regR_3}|0\rangle_{\regZ}|junk_{k,i}\rangle_{\regZ'}\Big]\Big)\\
&=&
\sum_k\Pr[k]
\sqrt{1-\epsilon_k}\\
&\ge&
\sum_k\Pr[k]
(1-\epsilon_k)\\
&\ge&
1-\negl(\secp).
\end{eqnarray*}
Therefore we have
\begin{eqnarray*}
&&\|\mbox{Tr}_\regR(Q_0|0\rangle_{\regC,\regR})
-\mbox{Tr}_\regR(Q_1|0\rangle_{\regC,\regR})\|_1\\
&=&
\|\mbox{Tr}_{\regR,\regZ}(Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ)
-\mbox{Tr}_{\regR,\regZ}(Q_1|0\rangle_{\regC,\regR}|junk_k\rangle_\regZ)\|_1\\
&=&
\|\mbox{Tr}_{\regR,\regZ}(U_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ)
-\mbox{Tr}_{\regR,\regZ}(Q_1|0\rangle_{\regC,\regR}|junk_k\rangle_\regZ)\|_1\\
&\le&
\|U_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ
-Q_1|0\rangle_{\regC,\regR}|junk_k\rangle_\regZ\|_1\\
&\le&\negl(\secp),
\end{eqnarray*}
which shows the statistical hiding of $\{Q_0,Q_1\}$.
\end{proof}




==> amplification.tex <==
\section{Amplification}
\label{sec:amplification}
\mor{kakikake}

\begin{definition}[Weak OWSGs]
A OWSG is called a weak OWSG if the security definition is replaced with the following one:
There exists a polynomial $p$ such that for any QPT adversary $\cA$ and any polynomial $t$,
\begin{eqnarray*}
\Pr[\top\gets\Ver(k',\phi_k):k\gets\Gen_1(1^\secp),\phi_k\gets\Gen_2(k),k'\gets\cA(\phi_k^{\otimes t})]
\le 1-\frac{1}{p}.
\end{eqnarray*}
\end{definition}

\begin{theorem}
If weak OWSGs exist, then (standard) OWSGs exist.
\end{theorem}

\begin{proof}
Let $(\mathsf{W}.\Gen_1,\mathsf{W}.\Gen_2,\mathsf{W}.\Ver)$ be a weak OWSG.
From it, we construct a (standard) OWSG as follows.
\begin{itemize}
    \item 
    $\Gen_1(1^\secp)\to k:$ Run $k\gets\mathsf{W}.\Gen_1$ $r$ times. Output $k\coloneqq(k_1,k_2,...,k_l)$.
    \item
   $\Gen_2(k)\to\phi_k:$ Parse $k=(k_1,...,k_r)$. Run $\phi_{k_i}\gets\mathsf{W}.\Gen_2(k_i)$ for each $i\in[1,2,...,r]$. 
   Output $\phi_k\coloneqq \phi_{k_1}\otimes...\otimes\phi_{k_r}$.
\item
$\Ver(k',\phi_k)\to\top/\bot:$
Parse $k'=(k'_1,...,k'_r)$. Parse $\phi_k=\phi_{k_1}\otimes...\otimes\phi_{k_r}$.
Run $\mathsf{W}.\Ver(k'_i,\phi_{k'})$ for each $i\in[1,2,...,r]$.
If all results are $\top$, output $\top$.
Otherwise, output $\bot$.
\end{itemize}
The correctness is clear. Assume that it is not secure.
Then, there exists a QPT adversary $\cA$, a polynomial $t$, and a polynomial $p$ such that
\begin{eqnarray*}
\Pr[\top\gets\Ver(k',\phi_k):k\gets\Gen_1(1^\secp),\phi_k\gets\Gen_2(k),k'\gets\cA(\phi_k^{\otimes t})]
\ge \frac{1}{p}.
\end{eqnarray*}




\end{proof}

==> backup.tex <==
\section{QPOTP}
\label{sec:QPOTP}
In this section, we first define (IND-based) QPOTP (\cref{sec:QPOTP_def}).
We then show that QPOTP implies OWSGs (\cref{sec:OWSGfromQPOTP}),
and that single-copy-secure QPOTP implies EFI pairs (\cref{sec:EFIfromQPOTP}).

\subsection{Definition of QPOTP}
\label{sec:QPOTP_def}

Quantum pseudo one-time pad is defined as follows.
\begin{definition}[(IND-based) quantum pseudo one-time pad (QPOTP)]
\label{def:OTP}
An (IND-based) quantum pseudo one-time pad (QPOTP) scheme with the key length $\kappa$ \takashi{Probably we can introduce $\KeyGen$ for QPOTP as well.} and
the plaintext length $l$ ($l>\kappa$) is a set of algorithms $(\Enc,\Dec)$ such that
\begin{itemize}
    \item 
    $\Enc(k,x)\to\ct:$ It is a QPT algorithm that, on input a classical secret key $k\in\bit^\kappa$ and 
    a classical plaintext message $x\in\bit^l$,
    outputs an $ln$-qubit quantum ciphertext $\ct$.
    \item
    $\Dec(\ct,k)\to x':$ It is a QPT algorithm that, on input $\ct$ and $k$, outputs $x'\in\bit^l$.
\end{itemize}
\paragraph{\bf Correctness:}
For any $x\in\bit^l$,
\begin{eqnarray*}
\Pr[x\gets\Dec(k,\ct):k\gets\bit^\kappa,\ct\gets\Enc(k,x)]\ge1-\negl(\secp).
\end{eqnarray*}
\paragraph{\bf Security:}
For any $x_0,x_1\in\bit^l$, any QPT adversary $\cA$, and any polynomial $t$,
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\ct_0^{\otimes t}):k\gets\bit^\kappa,\ct_0\gets\Enc(k,x_0)]\\
&&-\Pr[1\gets\cA(\ct_1^{\otimes t}):k\gets\bit^\kappa,\ct_1\gets\Enc(k,x_1)]|
\le\negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{remark}
We say that the scheme is single-copy-secure if the security holds only for $t=1$.
\end{remark}

\begin{remark}
Note that the definition of the security given in \cite{cryptoeprint:2021/1663} is different from the above one.
We consider the IND-based version of the security, while
the security definition of \cite{cryptoeprint:2021/1663} is as follows:
For any $x\in\bit^l$, any QPT adversary $\cA$, and any polynomial $t$,
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\ct^{\otimes t}):k\gets\bit^\kappa,\ct\gets\Enc(k,x)]\\
&&-\Pr[1\gets\cA((|\psi_1\rangle\otimes...\otimes|\psi_l\rangle)^{\otimes t})
:|\psi_1\rangle,...,|\psi_l\rangle\gets\mu_n]|
\le\negl(\secp),
\end{eqnarray*}
where $|\psi\rangle\gets\mu_n$ means the Haar random sampling of $n$-qubit states.
However, it is clear that the security definition of \cite{cryptoeprint:2021/1663} implies
our IND-based security, and therefore if QPOTP of \cite{cryptoeprint:2021/1663} exists,
that of \cref{def:OTP} exists.
\end{remark}

\begin{remark}
QPOTP is constructed from PRSGs~\cite{cryptoeprint:2021/1663}.
\end{remark}

\subsection{OWSGs from QPOTP}
\label{sec:OWSGfromQPOTP}

\begin{theorem}
QPOTP imply OWSGs.
\end{theorem}

\begin{proof}
Let $(\mathsf{OTP}.\Enc,\mathsf{OTP}.\Dec)$ be a QPOTP. From it, we construct a OWSG as follows.
\begin{itemize}
    \item 
    $\Gen_1(1^\secp)\to k:$
    $k\gets\bit^\kappa$.
    Output $k$.
    \item
    $\Gen_2(k)\to\phi_k:$
    Choose $x\gets\bit^l$.
    Run $\ct_{k,x}\gets \mathsf{OTP}.\Enc(k,x)$.
    Output $\phi_k\coloneqq \ct_{k,x}\otimes |x\rangle\langle x|$.
    \item
    $\Ver(k',\phi_k)\to\top/\bot:$
    Parse $\phi_k=\ct_{k,x}\otimes|x\rangle\langle x|$.
    Run $x'\gets\mathsf{OTP}.\Dec(k',\ct_{k,x})$.
    If $x'=x$, output $\top$. Otherwise, output $\bot$.
\end{itemize}

The correctness is clear. Let us show the security. Assume that it is not secure.
It means that there exists a QPT adversary $\cA$ and a polynomial $t$ such that
\begin{eqnarray}
\Pr\left[x'=x:
\begin{array}{cc}
    k\gets\bit^\kappa\\
    x\gets\bit^l\\
    \ct_{k,x}\gets \mathsf{OTP}.\Enc(k,x)\\
    k'\gets\cA((\ct_{k,x}\otimes |x\rangle\langle x|)^{\otimes t})\\
    x'\gets\mathsf{OTP}.\Dec(k',\ct_{k,x})
    \end{array}
    \right]\ge\frac{1}{\poly(\secp)}.
    \label{eq:OWSGfromQPOTP1}
    \end{eqnarray}
    From this $\cA$, we construct a QPT adversary $\cB$ that breaks the security of QPOTP as follows.
    Let $b\in\bit$ be the parameter of the following security game.
   \begin{enumerate}
       \item 
       $\cB$ chooses $x_0,x_1\gets\bit^l$, and sends them to the challenger $\cC$.
       \item
       $\cC$ chooses $k\gets\bit^\kappa$.
       \item
       $\cC$ runs $\ct_{k,x_b}\gets\mathsf{OTP}.\Enc(k,x_b)$ $t+1$ times.
       \item
       $\cC$ sends $\ct_{k,x_b}^{\otimes t+1}$ to $\cB$.
       \item
      $\cB$ runs $k'\gets\cA((\ct_{k,x_b}\otimes|x_0\rangle\langle x_0|)^{\otimes t})$. 
      \item
     $\cB$ runs $x'\gets\mathsf{OTP}.\Dec(k',\ct_{k,x_b})$. 
     If $x'=x_0$, $\cB$ outputs $b'=0$.
     Otherwise, it outputs $b'=1$.
   \end{enumerate} 
   It is clear that $\Pr[b'=0|b=0]$ is equivalent to the left-hand-side of Eq.~(\ref{eq:OWSGfromQPOTP1}), and therefore it is non-negligible.
   On the other hand,
   \begin{eqnarray*}
   \Pr[b'=0|b=1]&=&\frac{1}{2^{2l}}\sum_{x_0,x_1}\frac{1}{2^\kappa}\sum_k
   \sum_{k'}\Pr[k'\gets\cA((\ct_{k,x_1}\otimes|x_0\rangle\langle x_0|)^{\otimes t})]\\
&&\times    \Pr[x_0 \gets\mathsf{OTP}.\Dec(k',\ct_{k,x_1})]\\
&\le&\frac{1}{2^{2l}}\sum_{x_0,x_1}\frac{1}{2^\kappa}\sum_k
   \sum_{k'}\Pr[x_0 \gets\mathsf{OTP}.\Dec(k',\ct_{k,x_1})]\\
&=&\frac{1}{2^l}\sum_{k'}\sum_{x_0}
\Pr[x_0 \gets\mathsf{OTP}.\Dec(k',\frac{1}{2^{\kappa+l}}\sum_{k,x_1}\ct_{k,x_1})]\\
&=&\frac{1}{2^l}\sum_{k'}\\
&=&\frac{2^\kappa}{2^l}.
   \end{eqnarray*}
\end{proof}

\subsection{EFI pairs from single-copy-secure QPOTP}
\label{sec:EFIfromQPOTP}

\if0
\begin{definition}[ITS encryption scheme~\cite{LC19}]
An ITS encryption scheme is a set of algorithms $(\Gen,\Enc,\Dec)$ as follows.
\begin{itemize}
    \item 
    $\Gen(1^\secp)\to k:$
    It is a PPT algorithm that, on input the security parameter $\secp$, outputs $k$.
    \item
    $\Enc(k,\rho)\to \rho':$
    It is a QPT algorithm that, on input $k$ and a quantum state $\rho$, outputs a quantum state $\rho'$.
    \item
   $\Dec(k,\rho')\to \rho'':$ 
   It is a QPT algorithm that, on input $k$ and a quantum state $\rho'$, outputs a quantum state $\rho''$.
\end{itemize}
We require the following correctness and security.

\paragraph{\bf Correctness:}
The scheme is $\gamma$-correct if for any $\rho_{AB}$,
\begin{eqnarray*}
\mathbb{E}_{k\gets \Gen(1^\secp)}\|(\Dec^k_A\otimes I_B)(\Enc^k_A\otimes I_B)\rho_{AB}-\rho_{AB}\|_1
\le\gamma,
\end{eqnarray*}
where $\Dec^k$ and $\Enc^k$ are quantum operations that correspond to 
$\Dec$ and $\Enc$ with input $k$, respectively.
\end{definition}

\paragraph{\bf Security:}
The scheme is $\epsilon$-secure if for any $\rho_{AB},\sigma_{AB}$ with 
$\mbox{Tr}_A(\rho_{AB})=\mbox{Tr}_A(\sigma_{AB})$,
\begin{eqnarray*}
\|
\sum_k\Pr[k\gets\Gen(1^\secp)](\Enc^k_A\otimes I_B)\rho_{AB}
-\sum_k\Pr[k\gets\Gen(1^\secp)](\Enc^k_A\otimes I_B)\sigma_{AB}
\|_1
\le\gamma.
\end{eqnarray*}
\fi


\begin{theorem}
Single-copy-secure QPOTP with $\kappa\ge 2l+\log(1-\negl(\secp))$ implies EFI pairs.
\end{theorem}

\begin{proof}
Let $(\mathsf{QPOTP}.\Enc,\mathsf{QPOTP}.\Dec)$ be a QPOTP.
From it, we construct an EFI pair $\Gen(1^\secp,b)\to\rho_b$ as a QPT algorithm that outputs
\begin{eqnarray*}
\rho_0&\coloneqq&\frac{1}{2^{2n+\kappa}}\sum_{k,x,z}\ct_{k,(x,z)}\otimes
\Big[(X^xZ^z\otimes I)|\Psi\rangle\langle\Psi|(X^xZ^z\otimes I)\Big],\\
\rho_1&\coloneqq&\frac{1}{2^{2n+\kappa}}\sum_{k,x,z}\ct_{k,(x,z)}\otimes
\Big[(X^xZ^z\otimes I)\Big(|0^n\rangle\langle0^n|\otimes\frac{I^{\otimes n}}{2^n}\Big)|(X^xZ^z\otimes I)\Big],
\end{eqnarray*}
where $\ct_{k,(x,z)}\gets\Enc(k,(x,z))$, $2n=l$ and $|\Psi\rangle$ is the maximally-entangld state on two $n$-qubit registers.

First let us show the computational indistinguishability of $\rho_0$ and $\rho_1$.
Let us define
\begin{eqnarray*}
\rho_0'&\coloneqq&\frac{1}{2^{2n+\kappa}}\sum_{k,x,z}\ct_{k,(0^n,0^n)}\otimes
\Big[(X^xZ^z\otimes I)|\Psi\rangle\langle\Psi|(X^xZ^z\otimes I)\Big],\\
\rho_1'&\coloneqq&\frac{1}{2^{2n+\kappa}}\sum_{k,x,z}\ct_{k,(0^n,0^n)}\otimes
\Big[(X^xZ^z\otimes I)\Big(|0^n\rangle\langle0^n|\otimes\frac{I^{\otimes n}}{2^n}\Big)(X^xZ^z\otimes I)\Big].
\end{eqnarray*}
Then, for any QPT adversary $\cA$,
\begin{eqnarray*}
&&|\Pr[1\gets\cA(\rho_0)]
-\Pr[1\gets\cA(\rho_0')]|\\
&\le&
\frac{1}{2^{2n}}\sum_{x,z}\Big|
\Pr\Big[1\gets\cA\Big(\frac{1}{2^\kappa}\sum_k\ct_{k,(x,z)}\otimes
\Big[(X^xZ^z\otimes I)|\Psi\rangle\langle\Psi|(X^xZ^z\otimes I)\Big]\Big)\Big]\\
&&-\Pr\Big[1\gets\cA\Big(\frac{1}{2^\kappa}\sum_k\ct_{k,(0^n,0^n)}\otimes
\Big[(X^xZ^z\otimes I)|\Psi\rangle\langle\Psi|(X^xZ^z\otimes I)\Big]\Big)\Big]
\Big|\\
&\le&\negl(\secp),
\end{eqnarray*}
and
\begin{eqnarray*}
|\Pr[1\gets\cA(\rho_1)]
-\Pr[1\gets\cA(\rho_1')]|
\le\negl(\secp)
\end{eqnarray*}
in a similar way.
Moreover, $\rho_0'=\rho_1'$, because
\begin{eqnarray*}
\rho_0'&=&\frac{1}{2^\kappa}\sum_{k}\ct_{k,(0^n,0^n)}\otimes
\frac{1}{2^{2n}}\sum_{x,z}
\Big[(X^xZ^z\otimes I)|\Psi\rangle\langle\Psi|(X^xZ^z\otimes I)\Big],\\
\rho_1'&=&\frac{1}{2^\kappa}\sum_k\ct_{k,(0^n,0^n)}\otimes
\frac{1}{2^{2n}}\sum_{x,z}
\Big[(X^xZ^z\otimes I)\Big(|0^n\rangle\langle0^n|\otimes\frac{I^{\otimes n}}{2^n}\Big)(X^xZ^z\otimes I)\Big].
\end{eqnarray*}
Hence we have
\begin{eqnarray*}
|\Pr[1\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\le\negl(\secp)
\end{eqnarray*}
for any QPT adversary $\cA$.

Next let us show the statistical distinguishability of $\rho_0$ and $\rho_1$.
It can be shown in a similar way as in \cite{LC19}.
From QPOTP, construct an ITS encryption scheme as follows.
\begin{itemize}
    \item 
    $\Gen(1^\secp)\to k:$
    Choose $k\gets\bit^\kappa$.
    Output $k$.
    \item
    $\Enc(k,\rho_{AB})\to\rho'_{AB}:$
    Choose $x,z\gets\bit^n$.
    Run $\ct_{k,(x,z)}\gets\mathsf{QPOTP}.\Enc(k,(x,z))$.
    Output 
   \begin{eqnarray*} 
    \rho_{AB}'\coloneqq \ct_{k,(x,z)}\otimes\Big([(X^xZ^z)_A\otimes I_B]\rho_{AB}[(X^xZ^z)_A\otimes I_B]\Big).
   \end{eqnarray*} 
    \item
   $\Dec(k,\rho_{AB}')\to\rho_{AB}:$ 
   Parse
   \begin{eqnarray*}
   \rho_{AB}'= \ct_{k,(x,z)}\otimes\Big([(X^xZ^z)_A\otimes I_B]\rho_{AB}[(X^xZ^z)_A\otimes I_B]\Big).
   \end{eqnarray*}
   Run $(x,z)\gets\mathsf{QPOTP}.\Dec(k,\ct_{k,(x,z)})$.
   Obtain $\rho_{AB}$ by correcting the Pauli one-time pad.
   Output $\rho_{AB}$.
\end{itemize}
It satisfies the correctness with $\gamma=\negl(\secp)$.
If $\kappa\ge 2n+\log(1-\gamma-\sqrt{2\epsilon})$, from the theorem of \cite{LC19},
$\|\rho_0-\rho_1\|_1\ge\epsilon$.
If we take $\epsilon=\frac{1}{\poly(\secp)}$,
$\kappa\ge 2n+\log(1-\negl(\secp)) 
\ge 2n+\log(1-\negl(\secp)-\frac{1}{\poly(\secp)})$. 
\end{proof}




==> backup2.tex <==
\section{Quantum money}
\label{sec:money}
%checkdone2022/9/27

In this section, we first define private-key quantum money (\cref{sec:money_def}).
We then construct OWSGs from quantum money schemes (\cref{sec:OWSGfromQmoney}).

\subsection{Definition of private-key quantum money}
\label{sec:money_def}
Private-key quantum money is defined as follows.
\begin{definition}[Private-key quantum money]
A private-key quantum money scheme is a set of algorithms 
$(\KeyGen,\Mint,\Ver)$ such that 
\begin{itemize}
\item
$\KeyGen(1^\secp)\to k:$
It is a QPT algorithm that, on input the security parameter $\secp$,
outputs a classical secret key $k\in\bit^\kappa$.
\item
$\Mint(k)\to \$_k:$
It is a QPT algorithm that, on input
$k$, outputs an $m$-qubit quantum state $\$_k$.
\item
$\Ver(k,\rho)\to\top/\bot:$
It is a QPT algorithm that, on input $k$ and a quantum
state $\rho$, outputs $\top/\bot$.
\end{itemize}
We require the following correctness and security.

\paragraph{\bf Correctness:}
\begin{eqnarray*}
\Pr[\top\gets\Ver(k,\$_k):k\gets\KeyGen(1^\secp),\$_k\gets\Mint(k)]
\ge1-\negl(\secp).
\end{eqnarray*}

\paragraph{\bf Security:}
For any QPT adversary $\cA$ and any polynomial $t$,
\begin{eqnarray*}
\Pr\Big[\bigwedge_{i=1}^{t+1}
(\top\gets\Ver(k,\xi_i))
:k\gets\KeyGen(1^\secp),\$_k\gets\Mint(k),
\xi\gets\cA(\$_k^{\otimes t})\Big]
\le\negl(\secp),
\end{eqnarray*}
where $\xi$ is a quantum state on $t+1$ registers, 
$R_1,...,R_{t+1}$, each of which is of $m$ qubits,
and
$\xi_j\coloneqq\mbox{Tr}_{R_1,...,R_{j-1},R_{j+1},...,R_{t+1}}(\xi)$.
\end{definition}

\begin{remark}
The above definition is different from that in \cite{C:JiLiuSon18}
in the following three points.
First, the secret key is uniformly sampled in \cite{C:JiLiuSon18},
while here it is sampled by a QPT algorithm.
Second, money states are pure in \cite{C:JiLiuSon18},
while here we consider mixed states.
Finally, in \cite{C:JiLiuSon18},
the definition of the security is as follows:
For any QPT adversary $\cA$ and any polynomial $t$,
\begin{eqnarray*}
\Pr\Big[\mathsf{Count}(k,\xi)>t
:k\gets\bit^\secp,|\$_k\rangle\gets\Mint(k),\xi\gets\cA(|\$_k\rangle^{\otimes t})\Big]
\le\negl(\secp),
\end{eqnarray*}
where $\xi$ is a quantum state on $l$ registers, $R_1,...,R_l$, each of which is of $m$ qubits,
and $\mathsf{Count}$ is the following QPT algorithm:
on input $\xi$, it runs $\top/\bot\gets\Ver(k,\xi_j)$ for each $j\in[1,2,...,l]$, where
$\xi_j\coloneqq\mbox{Tr}_{R_1,...,R_{j-1},R_{j+1},...,R_l}(\xi)$,
and outputs the total number of $\top$.
It is easy to check that our security definition is weaker than
that \cite{C:JiLiuSon18}, i.e., if the security of \cite{C:JiLiuSon18} is satisfied,
then ours is also satisfied. Considering such a weaker definition allows us to get a stronger result.
(Remember that we want to construct OWSGs from quantum money, and therefore it is better
if we construct OWSGs from quantum money with a weaker definition.)
\end{remark}

\if0
\begin{remark}
In the original definition of \cite{C:JiLiuSon18}, $\Gen_1$ is a PPT algorithm.
Here, we generalize it to a QPT algorithm.
\end{remark}
\fi

\begin{remark}
Private-key quantum money is
constructed 
from PRSGs~\cite{C:JiLiuSon18}.
\end{remark}

We consider the following restriction for quantum money.

\begin{definition}[Symmetric-verifiability]
We say that a private-key quantum money scheme satisfies the symmetric-verifiability
if $\Pr[\top\gets\Ver(k,\$_{k'})]=\Pr[\top\gets\Ver(k',\$_{k})]$
for all $k\neq k'$.
\end{definition}

\begin{remark}
For example, if all money states are pure, and $\Ver(\alpha,\rho)$ is the following algorithm,
the symmetric-verifiability is satisfied:
Measure $\rho$ with the basis $\{|\$_{\alpha}\rangle\langle\$_\alpha|,I-|\$_\alpha\rangle\langle\$_\alpha|\}$.
If the first result is obtained, output $\top$. Otherwise, output $\bot$.
\end{remark}

The following theorem shows that if all money states are pure,
we can assume without loss of generality that quantum money schemes satisfy the symmetric-verifiability.

\begin{theorem}
If private-key quantum money schemes with pure money states
exist, then private-key quantum money schemes with pure money states and
symmetric-verifiability exist.
\end{theorem}

\begin{proof}
Let $(\mathsf{QM}.\KeyGen,\mathsf{QM}.\Mint,\mathsf{QM}.\Ver)$ be a private-key quantum money scheme with pure money states.
From it, we construct another private-key quantum money scheme 
$(\mathsf{QM}.\KeyGen',\mathsf{QM}.\Mint',\mathsf{QM}.\Ver')$ 
as follows.
$\mathsf{QM}.\KeyGen'$ and $\mathsf{QM}.\Mint'$ are not changed.
$\mathsf{QM}.\Ver'$ is defined as follows.
\begin{itemize}
    \item
    $\Ver(k,\rho)\to\top/\bot:$
    Measure $\rho$ with the basis
    $\{|\$_{k}\rangle\langle\$_{k}|,I-|\$_{k}\rangle\langle\$_{k}|\}$,
    and output $\top$ if the first result is obtained.
    Output $\bot$ if the second result is obtained.
    (This measurement is done in the following way: generate $U(|k\rangle|0...0\rangle)=|\$_{k}\rangle|\eta_{k}\rangle$,
    and discard the first register. Then apply $U^\dagger$ on $\rho\otimes |\eta_{k}\rangle\langle\eta_k|$, and measure all qubits
    in the computational basis. If the result is $k0...0$, accept. Otherwise, reject.)
\end{itemize}
The correctness is clear. Let us show the security. Assume that it is not secure.
Then, there exists a QPT operation $\cE$, a polynomial $t$, and a polynomial $p$ such that
\begin{eqnarray*}
\sum_{k}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \langle\$_k|^{\otimes t+1}\cE(|\$_{k}\rangle^{\otimes t})|\$_k\rangle^{\otimes t+1}
    \ge\frac{1}{p}.
    \end{eqnarray*}
   Define the set
    \begin{eqnarray*}
    S\coloneqq\Big\{k\in\bit^\kappa~\Big|~\langle\$_k|^{\otimes t+1}\cE(|\$_k\rangle^{\otimes t})|\$_{k}\rangle^{\otimes t+1}\ge
    \frac{1}{2p}\Big\}.
    \end{eqnarray*}
    Then, we have
    \begin{eqnarray}
    \sum_{k\in S}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\ge \frac{1}{2p}.
    \label{Qmoney_pure_Sbound}
    \end{eqnarray}
    This is shown as follows.
 \begin{eqnarray*}
\frac{1}{p}
&\le&\sum_{k}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \langle\$_k|^{\otimes t+1}\cE(|\$_{k}\rangle^{\otimes t})|\$_k\rangle^{\otimes t+1}\\
&=&\sum_{k\in S}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \langle\$_k|^{\otimes t+1}\cE(|\$_{k}\rangle^{\otimes t})|\$_k\rangle^{\otimes t+1}\\
&&+\sum_{k\notin S}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \langle\$_k|^{\otimes t+1}\cE(|\$_{k}\rangle^{\otimes t})|\$_k\rangle^{\otimes t+1}\\
&\le&\sum_{k\in S}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
+\frac{1}{2p},
    \end{eqnarray*}
    which gives Eq.~(\ref{Qmoney_pure_Sbound}).
  Let us also define the set
  \begin{eqnarray*}
  T\coloneqq\Big\{k\in\bit^\kappa~\Big|~\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]
  \ge1-\frac{1}{8p(t+1)}\Big\}.
  \end{eqnarray*}
  Then, 
  \begin{eqnarray}
  \sum_{k\in T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\ge 1-\negl(\secp). 
  \label{Qmoney_pure_Tbound}
  \end{eqnarray}
  This is shown as follows.
  \begin{eqnarray*}
  1-\negl(\secp)&\le&\sum_k\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\\
  &=&\sum_{k\in T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\\
  &&+\sum_{k\notin T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\Pr[\top\gets\mathsf{QM}.\Ver(k,|\$_k\rangle)]\\
  &\le&\sum_{k\in T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\\
  &&+\Big(1-\frac{1}{8p(t+1)}\Big)\Big(1-\sum_{k\in T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\Big),
  \end{eqnarray*}
  which gives Eq.~(\ref{Qmoney_pure_Tbound}).
  The probability that $k\in S\cap T$ 
  is, from the union bound, Eq.~(\ref{Qmoney_pure_Sbound}), and Eq.~(\ref{Qmoney_pure_Tbound}),
  \begin{eqnarray}
  \sum_{k\in S \cap T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
  &\ge& \frac{1}{2p}+1-\negl(\secp)-1\nonumber\\
  &=& \frac{1}{2p}-\negl(\secp).
  \label{Qmoney_union}
  \end{eqnarray}
  
  
      Let us show that the above $\cE$ breaks the security of the original private-key quantum money scheme.
    Let $\xi_i\coloneqq \mbox{Tr}_{R_1,...,R_{i-1},R_{i+1},...,R_{t+1}}(\cE(|\$_k\rangle^{\otimes t}))$.
    The probability that the $\cE$ breaks the security of the original private-key quantum money scheme is
    \begin{eqnarray*}
&&    \sum_{k}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr\Big[\bigwedge_{i=1}^{t+1}(\top\gets\mathsf{QM}.\Ver(k,\xi_{i}))\Big]\\
    &\ge&
    \sum_{k\in S\cap T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr\Big[\bigwedge_{i=1}^{t+1}(\top\gets\mathsf{QM}.\Ver(k,\xi_{i}))\Big]\\
    &\ge&
    \sum_{k\in S\cap T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Big(\Pr\Big[\bigwedge_{i=1}^{t+1}(\top\gets\mathsf{QM}.\Ver(k,|\$_{k}\rangle))\Big]-\sqrt{1-\frac{1}{2p}}~\Big)\\
    &\ge&
    \sum_{k\in S\cap T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Big(\Big(1-\frac{1}{8p(t+1)}\Big)^{t+1}-\sqrt{1-\frac{1}{2p}}~\Big)\\
     &\ge&
    \Big(\frac{1}{2p}-\negl(\secp)\Big)
    \Big(1-\frac{1}{8p}-\Big(1-\frac{1}{4p}\Big)\Big),
    \end{eqnarray*}
    which is non-negligible.
    $\cE$ therefore breaks the security of the original private-key quantum money scheme.
   
\end{proof}


\subsection{OWSGs from quantum money}
\label{sec:OWSGfromQmoney}

\begin{theorem}
If private-key quantum money schemes with symmetric-verifiability
exist, then OWSGs exist.
\end{theorem}
\mor{there is a mistake here.}

\begin{proof}
Let $(\mathsf{QM}.\KeyGen,\mathsf{QM}.\Mint,\mathsf{QM}.\Ver)$ be a private-key quantum money scheme.
From it, we construct a wOWSG as follows.
(Due to \cref{thm:amplification_OWSG}, it means the existene of OWSGs.)
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    Run $k\gets\mathsf{QM}.\KeyGen(1^\secp)$.
    Output $k$.
    \item
    $\StateGen(k)\to\phi_k:$
    Run $\$_k\gets\mathsf{QM}.\Mint(k)$ $r$ times.
    Output $\phi_k\coloneqq \$_k^{\otimes r}$.
    \item
    $\Ver(k',\phi_k)\to\top/\bot:$
    Parse $\phi_k=\$_k^{\otimes r}$.
    Run $v\gets\mathsf{QM}.\Ver(k',\$_k)$ for each $\$_k$ of $\phi_k$.
    If all results are $\top$, output $\top$.
    Otherwise, output $\bot$.
\end{itemize}
The correctness is clear. Let us show the security. Assume that it is not secure.
Then, for any polynomial $p$, there exists a QPT adversary $\cA$ and a polynomial $t$ such that 
\begin{eqnarray*}
\sum_{k,k'}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr[k'\gets\cA(\$_k^{\otimes rt})]
\Pr[\top\gets\mathsf{QM}.\Ver(k',\$_k)]^{r}
    \ge1-\frac{1}{p}.
    \end{eqnarray*}
    Let us define the set
    \begin{eqnarray*}
    S\coloneqq\Big\{(k,k')\in\bit^\kappa\times\bit^\kappa~\Big|~
    \Pr[\top\gets\mathsf{QM}.\Ver(k',\$_k)]^r\ge
    1-\delta\Big\}.
    \end{eqnarray*}
    Then, we have
    \begin{eqnarray}
    \sum_{(k,k')\in S}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr[k'\gets\cA(\$_k^{\otimes rt})]\ge 1- \frac{1}{\delta p}.
    \label{Qmoney_Sbound}
    \end{eqnarray}
    This is because
 \begin{eqnarray*}
1-\frac{1}{p}&\le&
\sum_{k,k'}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr[k'\gets\cA(\$_k^{\otimes t})]
\Pr[\top\gets\mathsf{QM}.\Ver(k',\$_k)]^r\\
&=&
\sum_{(k,k')\in S}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr[k'\gets\cA(\$_k^{\otimes t})]
\Pr[\top\gets\mathsf{QM}.\Ver(k',\$_k)]^r\\
&&+
\sum_{(k,k')\notin S}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr[k'\gets\cA(\$_k^{\otimes t})]
\Pr[\top\gets\mathsf{QM}.\Ver(k',\$_k)]^r\\
&\le&
\sum_{(k,k')\in S}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr[k'\gets\cA(\$_k^{\otimes t})]\\
&&+
\Big(1-\delta\Big)\sum_{(k,k')\notin S}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr[k'\gets\cA(\$_k^{\otimes t})]\\
 &=&
\sum_{(k,k')\in S}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr[k'\gets\cA(\$_k^{\otimes t})]\\
&&+
\Big(1-\delta\Big)
\Big(1-\sum_{(k,k')\in S}
\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
    \Pr[k'\gets\cA(\$_k^{\otimes t})]\Big),
    \end{eqnarray*}
    which gives Eq.~(\ref{Qmoney_Sbound}).
     
    
    From this $\cA$, we construct a QPT adversary $\cB$ that breaks the security of the private-key quantum money 
    scheme as follows:
    On input $\$_k^{\otimes rt}$, it runs $k'\gets\cA(\$_k^{\otimes rt})$.
    It then runs $\$_{k'}\gets\mathsf{QM}.\Mint(k')$ $rt+1$ times, 
    and outputs $\xi\coloneqq \$_{k'}^{\otimes rt+1}$.
   
    Let us show that thus defined $\cB$ breaks the security of the private-key quantum money scheme.
  The probability that the $\cB$ breaks the quantum money scheme is
     \begin{eqnarray*}
&&     \sum_{k,k'}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
     \Pr[k'\gets\cA(\$_k^{\otimes rt})]
     \Pr[\top\gets\mathsf{QM}.\Ver(k,\$_{k'})]^{rt+1}\\
     &=&
      \sum_{k,k'}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
     \Pr[k'\gets\cA(\$_k^{\otimes rt})]
     \Pr[\top\gets\mathsf{QM}.\Ver(k',\$_k)]^{rt+1}\\
      &\ge&
      \sum_{(k,k')\in S}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
     \Pr[k'\gets\cA(\$_k^{\otimes rt})]
     \Pr[\top\gets\mathsf{QM}.\Ver(k',\$_k)]^{rt+1}\\
    &\ge&\Big(1-\frac{1}{\delta p}\Big)\Big(1-\delta\Big)^{\frac{rt+1}{r}}\\
    &\ge&\Big(1-\frac{1}{\delta p}\Big)\Big(1-\frac{\delta(rt+1)}{r}\Big)\\
\end{eqnarray*}   
where $r<rt+1$.
$\delta=\frac{r}{rt+1}$
   
\end{proof}





==> backup3.tex <==
\section{SVOWSGs}
\label{sec:SVOWSG}

In this section, we define SVOWSGs (\cref{sec:SVOWSG_def}), and show that SVOWSGs are equivalent to EFI pairs (\cref{sec:SVOWSG_EFI}).
We also provide a preliminaries section (\cref{sec:SVOWSG_pre}) to give two results used for our proofs.

\subsection{Preliminaries}
\label{sec:SVOWSG_pre}

Let us first explain quantum shadow tomography~\cite{Shadow1,Shadow2},
which we will use later.
The following result gives the best parameters \cite{Shadow_best}.
\begin{theorem}[Quantum shadow tomography~\cite{Shadow_best}]
\label{theorem:shadow}
Let $0<\epsilon<\frac{1}{2}$.
Consider $M$ different POVM elements $E_1,E_2,...,E_M$, i.e.,
$0\le E_i\le I$ for each $i\in\{1,2,...,M\}$.
There exists a (not necessarily polynomial-time) quantum algorithm that, on input
the 
$T$ copies $\rho^{\otimes T}$ of a $d$-dimensional quantum state $\rho$ with
\begin{eqnarray*}
T=\frac{[(\log M)^2+\log(\frac{\log d}{\delta\epsilon})]\log d}{\epsilon^4}
\times O\left(\log\left(\frac{\log d}{\delta\epsilon}\right)\right),
\end{eqnarray*}
outputs $(\eta_1,...,\eta_M)$
such that
$|\eta_j-\mbox{Tr}(E_j\rho)|\le\epsilon$ for all $j\in\{1,2,...,M\}$
with probability at
least $1-\delta$. 
\end{theorem}
In particular, if we take $\epsilon=O(\frac{1}{\poly(\secp)})$,
$\delta=O(\frac{1}{2^{\poly(\secp)}})$, 
$M=O(2^{\poly(\secp)})$, 
and $d=O(2^{\poly(\secp)})$, 
we have $T=O(\poly(\secp))$.


We also use the following result.
\begin{theorem}[\cite{Montanaro19}]
\label{theorem:Montanaro}
Let $\{\rho_i\}_i$ be a set of states.
Define the POVM measurement $\{\mu_i\}_i$ with
$\mu_i\coloneqq\Sigma^{1/2}\rho_i\Sigma^{1/2}$,
where $\Sigma\coloneqq \sum_i\rho_i$,
and the inverse is taken on the support of $\Sigma$.
Then,
$\max_i(1-\mbox{Tr}(\mu_i\rho_i))\le\sum_{i\neq j}F(\rho_i,\rho_j)$.
\end{theorem}


\subsection{Definition of SVOWSGs}
\label{sec:SVOWSG_def}

SVOWSGs are defined as follows.
\begin{definition}[Secretly-verifiable OWSGs (SVOWSGs)]
A secretly-verifiable OWSG (SVOWSG) is a set of algorithms $(\KeyGen,\StateGen)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs a key $k\in\bit^\kappa$.
    \item
    $\StateGen(k)\to\phi_k:$
    It is a QPT algorithm that, on input $k$, outputs an $m$-qubit state $\phi_k$.
\end{itemize}
We require the following two properties.

\paragraph{\bf Statistical invertibility:}
There exists a polynomial $p$ such that, for any $k\neq k'$,
\begin{eqnarray*}
\frac{1}{2}\|\phi_k-\phi_{k'}\|_1\ge\frac{1}{p}.
\end{eqnarray*}


\paragraph{\bf Computational non-invertibility:}
For any QPT adversary $\cA$ and any polynomial $t$, 
\begin{eqnarray*}
\Pr[k\gets\cA(\phi_k^{\otimes t}):k\gets\KeyGen(1^\secp),\phi_k\gets\StateGen(k)]\le \negl(\secp).
\end{eqnarray*}
\end{definition}

\begin{remark}
The definition of SVOWSGs is different from that of OWSGs in the following two points.
First, it does not have any verification algorithm that allows the public verification.\footnote{We call it ``secretly-verifiable'' OWSGs even though there is no verification algorithm in the syntax because we can think of the check of $k'\overset{?}{=}k$ as a secret verification algorithm. }
Second, the correctness of OWSGs is replaced with
the statistical invertibility.
The reason of introducing statistical invertibility is to avoid statistically-secure constructions.
(In other words, if states $\{\phi_k\}_k$ are close with each other, it is statistically impossible to 
find the correct $k$.)
For example, a SVOWSG without the statistical invertibility
can be trivially constructed by taking
$\StateGen(k)\to\frac{I^{\otimes m}}{2^m}$ for all $k$. Note that SVOWSGs and OWSGs are incomparable since OWSGs do not necessarily satisfy the statistical invertibility.\footnote{Generally speaking, ``secretly-verifiable'' XX is weaker than publicly-verifiable XX in many contexts of cryptography, and therefore this may be slightly confusing. But we do not have any good idea to avoid the confusion.}
\end{remark}

The following lemma shows that the statistical invertibility with advantage $\frac{1}{\poly(\secp)}$
can be amplified to $1-2^{-q}$ for any polynomial $q$.
\begin{lemma}
\label{lemma:SVOWSG_amp}
If a SVOWSG exists
then
a SVOWSG with statistical invertibility larger than $1-2^{-q}$ with any polynomial $q$ exists.
\end{lemma}

\begin{proof}
Let $(\KeyGen,\StateGen)$ be a SVOWSG with statistical invertibility larger than $\frac{1}{p}$,
where $p$ is a polynomial.
From it, we construct a new SVOWSG ($\KeyGen',\StateGen'$) as follows:
\begin{itemize}
    \item 
    $\KeyGen'(1^\secp)\to k$:
    Run $k\gets\KeyGen(1^\secp)$, and output $k$.
    \item
    $\StateGen'(k)\to\phi_k':$
    Run $\phi_k\gets \StateGen(k)$ $4pq$ times, and output
    $\phi_k'\coloneqq \phi_k^{\otimes 4pq}$.
\end{itemize}
First, for any $k\neq k'$,
\begin{eqnarray*}
\frac{1}{2}\|\phi_k'-\phi_{k'}'\|_1
&=&\frac{1}{2}\|\phi_k^{\otimes 4pq}-\phi_{k'}^{\otimes 4pq}\|_1\\
&\ge& 1-\exp(-4qp\|\phi_k-\phi_{k'}\|_1/4)\\
&\ge& 1-\exp(-q)\\
&\ge& 1-2^{-q},
\end{eqnarray*}
which shows the statistical invertibility of $(\KeyGen',\StateGen')$ with the advantage
larger than $1-2^{-q}$.
Second, from the computational non-invertibility of $(\KeyGen,\StateGen)$, 
\begin{eqnarray*}
&&\Pr[k\gets\cA(\phi_k'^{\otimes t}):k\gets\KeyGen'(1^\secp),\phi_k'\gets\StateGen'(k)]\\
&=&\Pr[k\gets\cA(\phi_k^{\otimes 4pqt}):k\gets\KeyGen(1^\secp),\phi_k\gets\StateGen(k)]\\
&\le& \negl(\secp).
\end{eqnarray*}
for any QPT adversary $\cA$ and any polynomial $t$, 
which shows the computational non-invertibility of $(\KeyGen',\StateGen')$.
\end{proof}


\subsection{Equivalence of SVOWSGs and EFI pairs}
\label{sec:SVOWSG_EFI}

\begin{theorem}
SVOWSGs exist if and only if EFI pairs exist.
\end{theorem}

\begin{proof}
First, let us show that if
EFI pairs exist then SVOWSGs exist.
Let $\mathsf{EFI}.\Gen(1^\secp,b)\to\rho_b$ be an EFI pair.
As is explained in \cref{remark:EFI}, we can assume without loss of generality that
$\frac{1}{2}\|\rho_0-\rho_1\|_1\ge1-\negl(\secp)$,
which means $F(\rho_0,\rho_1)\le\negl(\secp)$.
From the EFI pair, we construct a SVOWSG as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    Choose $k\gets\bit^\secp$, and ouput $k$.
    \item
    $\StateGen(k)\to\phi_k:$
    Run $\mathsf{EFI}.\Gen(1^\secp,k_i)\to\rho_{k_i}$ for each $i\in[\secp]$.
    Output $\phi_k\coloneqq \bigotimes_{i=1}^\secp \rho_{k_i}$.
\end{itemize}

The statistical invertibility is easily shown as follows. 
If $k\neq k'$, there exists a $j\in[\secp]$ such that $k_j\neq k_j'$.
Then,
\begin{eqnarray*}
F(\phi_k,\phi_{k'})&=&\prod_{i=1}^\secp F(\rho_{k_i},\rho_{k_i'})\\
&\le& F(\rho_{k_j},\rho_{k_j'})\\
&\le&\negl(\secp),
\end{eqnarray*}
which means $\frac{1}{2}\|\phi_k-\phi_{k'}\|_1\ge1-\negl(\secp)$.
This shows the statistical invertibility.

Let us next show the computational non-invertibility.
From the standard hybrid argument (\mor{see Appendix??}), and the computational indistinguishability of $\rho_0$ and $\rho_1$, we have
\begin{eqnarray*}
|\Pr[k\gets\cA(\phi_k^{\otimes t})]-\Pr[k\gets\cA(\phi_{0^\secp}^{\otimes t})]|\le\negl(\secp)
\end{eqnarray*}
for any $k$ and any polynomial $t$.
Hence
\begin{eqnarray*}
&&\Pr[k\gets\cA(\phi_k^{\otimes t}):k\gets\KeyGen(1^\secp),\phi_k\gets\StateGen(k)]\\
&=&\frac{1}{2^\secp}\sum_{k\in\bit^\secp}\Pr[k\gets\cA(\phi_k^{\otimes t})]\\
&\le&\frac{1}{2^\secp}\sum_{k\in\bit^\secp}(\Pr[k\gets\cA(\phi_{0^\secp}^{\otimes t})]+\negl(\secp))\\
&=&\frac{1}{2^\secp}+\negl(\secp),
\end{eqnarray*}
which shows the computational non-invertibility.


Next let us show that
if SVOWSGs exist then EFI pairs exist.
Let $(\mathsf{SVOWSG}.\KeyGen,\mathsf{SVOWSG}.\StateGen)$ be a SVOWSG.
Without loss of generality, we can assume that
$\mathsf{SVOWSG}.\KeyGen$ is the following algorithm:
first apply a QPT unitary $U$ on $|0...0\rangle$ to generate 
\begin{eqnarray*}
U|0...0\rangle=\sum_{k\in\bit^\secp}\sqrt{\Pr[k\gets\mathsf{SVOWSG}.\KeyGen(1^\secp)]}|k\rangle|\mu_k\rangle, 
\end{eqnarray*}
and trace out the second register,
where $\{|\mu_k\rangle\}_k$ are some states.
Moreover, without loss of generality, we can also assume that $\mathsf{SVOWSG}.\StateGen$ is the following algorithm:
first apply a QPT unitary $V_k$ that depends on $k$ on $|0...0\rangle$ to generate 
$V_k|0...0\rangle=|\psi_k\rangle_{AB}$, and trace out the register $A$.

From the SVOWSG, we want to construct an EFI pair.
For that goal, we construct a statistically-hiding and computationally-binding commitment scheme from
SVOWSG. Due to the equivalence between different flavors of commitments~\cite{HMY22,cryptoeprint:2020/1488}, we then have
a statistically-binding and computationally-hiding commitment scheme, which is equivalent to an EFI pair.
From the SVOWSG, we construct
a statistically-hiding and computationally-binding commitment scheme $\{Q_0,Q_1\}$ as follows.
\begin{eqnarray*}
Q_0|0\rangle_{CR}&\coloneqq&\sum_{k\in\bit^\secp}\sqrt{\Pr[k]} 
(|k\rangle|\mu_k\rangle)_{C1}
|\psi_k\rangle_{C2R2}^{\otimes t}|0\rangle_{R3},\\
Q_1|0\rangle_{CR}&\coloneqq& \sum_{k\in\bit^\secp}\sqrt{\Pr[k]}
(|k\rangle|\mu_k\rangle)_{C1}
|\psi_k\rangle_{C2R2}^{\otimes t}|k\rangle_{R3},
\end{eqnarray*}
where $\Pr[k]\coloneqq\Pr[k\gets\mathsf{SVOWSG}.\KeyGen(1^\secp)]$, $C2$ is the combination of all ``$A$ registers'' of $|\psi_k\rangle$,
$R2$ is the combination of all ``$B$ registers'' of $|\psi_k\rangle$,
$C\coloneqq(C1,C2)$ and $R\coloneqq(R2,R3)$.

Let us first show the computational binding of $\{Q_0,Q_1\}$.
Assume that it is not computationally binding. Then, there exists a QPT unitary $U$, an ancilla state $|\tau\rangle$,
and a polynomial $p$ such that
\begin{eqnarray*}
\|
(\langle 0|Q_1^\dagger)_{CR} U_{RZ}(Q_0|0\rangle_{CR}\otimes|\tau\rangle_Z)
\|^2
\ge\frac{1}{p}.
\end{eqnarray*}
Then,
\begin{eqnarray}
\frac{1}{p}
&\le&
\|
(\langle 0|Q_1^\dagger)_{CR} U_{RZ}(Q_0|0\rangle_{CR}\otimes|\tau\rangle_Z)
\|^2\nonumber\\
&\le&
\Big\|
\Big(\sum_{k'}\sqrt{\Pr[k']}\langle k',\mu_{k'}|_{C1}\langle\psi_{k'}|^{\otimes t}_{C2R2}\langle k'|_{R3}\Big)\nonumber\\
&&\times\Big(\sum_{k}\sqrt{\Pr[k]}|k,\mu_k\rangle_{C1}U_{RZ}|\psi_k\rangle^{\otimes t}_{C2R2}|0\rangle_{R3}|\tau\rangle_Z\Big)
\Big\|^2\nonumber\\
&=&
\Big\|
\sum_{k}\Pr[k]
\langle\psi_{k}|^{\otimes t}_{C2R2}\langle k|_{R3}
U_{RZ}|\psi_k\rangle^{\otimes t}_{C2R2}|0\rangle_{R3}|\tau\rangle_Z
\Big\|^2\nonumber\\
&\le&
\sum_{k}\Pr[k]
\Big\|
\langle\psi_{k}|^{\otimes t}_{C2R2}\langle k|_{R3}
U_{RZ}|\psi_k\rangle^{\otimes t}_{C2R2}|0\rangle_{R3}|\tau\rangle_Z
\Big\|^2\nonumber\\
&\le&
\sum_{k}\Pr[k]
\Big\|
\langle k|_{R3}
U_{RZ}|\psi_k\rangle^{\otimes t}_{C2R2}|0\rangle_{R3}|\tau\rangle_Z
\Big\|^2.
\label{POWSG_B}
\end{eqnarray}
Let us consider the following QPT adversary $\cB$:
On input the $R2$ register of $|\psi_k\rangle^{\otimes t}_{C2R2}$, apply $U_{RZ}$ on
$|\psi_k\rangle_{C2R2}^{\otimes t}|0\rangle_{R3}|\tau\rangle_Z$, and measure
the $R3$ register in the computational basis. Output the result.
Then, the probability that $\cB$
correctly outputs $k$ is equal to Eq.~(\ref{POWSG_B}).
Therefore, $\cB$ breaks the security of the SVOWSG.


Let us next show the statistical hiding of $\{Q_0,Q_1\}$.
Let us consider the following quantum (not necessarily polynomial-time) algorithm, 
$\mathsf{Shadow}(\{\Pi_k\}_k,\rho^{\otimes t})\to k^*$ that,
on input a POVM measurement $\{\Pi_k\}_k$ and $t$ copies of a state $\rho$, outputs $k^*\in\bit^\secp$.
\begin{enumerate}
    \item 
On input $\rho^{\otimes t}$, run the shadow tomography algorithm (\cref{theorem:shadow}) to get
$\{\eta_k\}_{k\in\bit^\secp}$ such that $|\mbox{Tr}(\Pi_k\rho)-\eta_k|\le\frac{1}{\poly(\secp)}$ for each $k\in\bit^\secp$.
\item
If there is a $k^*$ such that $\eta_{k^*}\ge 1-\frac{1}{\poly(\secp)}$, output the $k^*$.
\end{enumerate}

From \cref{lemma:SVOWSG_amp}, we can assume without loss of generality that
$\frac{1}{2}\|\phi_k-\phi_{k'}\|_1\ge1-2^{-3\secp}$
for any $k\neq k'$.
Then,
from \cref{lemma:SVOWSG_equivalence}, there exists a (not necessarily QPT) POVM measurement 
$\{\Pi_k\}_k$ such that
$\mbox{Tr}(\Pi_k \phi_k)\ge1-\negl(\secp)$ and
$\mbox{Tr}(\Pi_{k'} \phi_k)\le\negl(\secp)$ for all $k\neq k'$.
Therefore, due to the correctness of the shadow tomography algorithm,
$\Pr[k\gets\mathsf{Shadow}(\{\Pi_{k'}\}_{k'},\phi_k^{\otimes t})]\ge1-\negl(\secp)$
for all $k$.
Let $U$ be a unitary that implements $\mathsf{Shadow}$. In other words,
\begin{eqnarray*}
U_{R2Z}|\psi_k\rangle^{\otimes t}_{C2R2}|0...0\rangle_Z
&=&(1-\epsilon_k)|k\rangle|junk_k\rangle+\sum_{k':k'\neq k} \epsilon_{k'}|k'\rangle|junk_{k'}\rangle,
\end{eqnarray*}
where $Z$ is the ancilla register, $\epsilon_k\le\negl(\secp)$,
and $|junk_k\rangle$ are ``junk'' states.
Let $V$ be the following unitary:
\begin{enumerate}
    \item 
    Apply $U$ on $|\psi_k\rangle^{\otimes t}_{C2R2}|0...0\rangle_Z$:
    \begin{eqnarray*}
U_{R2Z}|\psi_k\rangle^{\otimes t}_{C2R2}|0...0\rangle_Z
=(1-\epsilon_k)|k\rangle|junk_k\rangle+\sum_{k':k'\neq k} \epsilon_{k'}|k'\rangle|junk_{k'}\rangle.
    \end{eqnarray*}
    \item
    Add a $\secp$-qubit ancilla register $Z'$:
    \begin{eqnarray*}
(1-\epsilon_k)|k\rangle|junk_k\rangle|0^\secp\rangle_{Z'}+\sum_{k':k'\neq k} \epsilon_{k'}|k'\rangle|junk_{k'}\rangle|0^\secp\rangle_{Z'}.
    \end{eqnarray*}
     \item
    Copy the content of the first register to the register $Z'$:
    \begin{eqnarray*}
(1-\epsilon_k)|k\rangle|junk_k\rangle|k\rangle_{Z'}+\sum_{k':k'\neq k} \epsilon_{k'}|k'\rangle|junk_{k'}\rangle|k'\rangle_{Z'}.
    \end{eqnarray*}
      \item
    Apply $U^\dagger$:
    \begin{eqnarray*}
(1-\epsilon_k)U^\dagger(|k\rangle|junk_k\rangle)|k\rangle_{Z'}
+\sum_{k':k'\neq k} \epsilon_{k'}U^\dagger(|k'\rangle|junk_{k'}\rangle)|k'\rangle_{Z'}.
    \end{eqnarray*}
\end{enumerate}
Then, as we will show later,
\begin{eqnarray}
\|V_{R2ZZ'}|\psi_k\rangle^{\otimes t}_{C2R2}|0\rangle_Z|0\rangle_{Z'}
-|\psi_k\rangle^{\otimes t}_{C2R2}|0\rangle_Z|k\rangle_{Z'} \|_1
&\le&\negl(\secp).
\label{SVOWSG_V}
\end{eqnarray}
Let $W$ be a unitary that applies $V$ and then swap the register $R3$ and $Z'$.
Then,
\begin{eqnarray*}
\|W_{R2ZZ'}Q_0|0\rangle_{CR}|0\rangle_Z|0\rangle_{Z'}
-Q_1|0\rangle_{CR}|0\rangle_Z|0\rangle_{Z'} \|_1
&\le&\negl(\secp).
\end{eqnarray*}
Therefore,
\begin{eqnarray*}
&&\|\mbox{Tr}_{R}(Q_0|0\rangle_{CR})
-\mbox{Tr}_{R}(Q_1|0\rangle_{CR})\|_1\\
&=&
\|\mbox{Tr}_{RZZ'}(Q_0|0\rangle_{CR}|0\rangle_Z|0\rangle_{Z'})
-\mbox{Tr}_{RZZ'}(Q_1|0\rangle_{CR}|0\rangle_Z|0\rangle_{Z'})\|_1\\
&=&
\|\mbox{Tr}_{RZZ'}(W_{RZZ'}Q_0|0\rangle_{CR}|0\rangle_Z|0\rangle_{Z'})
-\mbox{Tr}_{RZZ'}(Q_1|0\rangle_{CR}|0\rangle_Z|0\rangle_{Z'})\|_1\\
&\le&
\|\mbox{Tr}_R(Q_1|0\rangle_{CR})-\mbox{Tr}_R(Q_1|0\rangle_{CR})\|_1+\negl(\secp)\\
&=&
\negl(\secp),
\end{eqnarray*}
which shows the statistical hiding of $\{Q_0,Q_1\}$.

Let us show Eq.~(\ref{SVOWSG_V}).
\begin{eqnarray*}
&&\|V|\psi_k\rangle_{C2R2}^{\otimes t}|0\rangle_Z|0\rangle_{Z'}
-|\psi_k\rangle_{C2R2}^{\otimes t}|0\rangle_Z|k\rangle_{Z'}
\|_1\\
&=&
\|
(1-\epsilon_k)U^\dagger(|k\rangle|junk_k\rangle)|k\rangle_{Z'}
+\sum_{k'\neq k}\epsilon_{k'}U^\dagger(|k'\rangle|junk_{k'}\rangle)|k'\rangle_{Z'}
-|\psi_k\rangle_{C2R2}^{\otimes t}|0\rangle_Z|k\rangle_{Z'}
\|_1\\
&=&
\|
(1-\epsilon_k)(|k\rangle|junk_k\rangle)|k\rangle_{Z'}
+\sum_{k'\neq k}\epsilon_{k'}(|k'\rangle|junk_{k'}\rangle)|k'\rangle_{Z'}
-U|\psi_k\rangle_{C2R2}^{\otimes t}|0\rangle_Z|k\rangle_{Z'}
\|_1\\
&=&
\|
(1-\epsilon_k)(|k\rangle|junk_k\rangle)|k\rangle_{Z'}
+\sum_{k'\neq k}\epsilon_{k'}(|k'\rangle|junk_{k'}\rangle)|k'\rangle_{Z'}\\
&&-(1-\epsilon_k)(|k\rangle|junk_k\rangle)|k\rangle_{Z'}
-\sum_{k'\neq k}\epsilon_{k'}(|k'\rangle|junk_{k'}\rangle)|k\rangle_{Z'}
\|_1\\
&=&
\|
\sum_{k'\neq k}\epsilon_{k'}(|k'\rangle|junk_{k'}\rangle)|k'\rangle_{Z'}
-\sum_{k'\neq k}\epsilon_{k'}(|k'\rangle|junk_{k'}\rangle)|k\rangle_{Z'}
\|_1\\
&\le&
\|
\sum_{k'\neq k}\epsilon_{k'}(|k'\rangle|junk_{k'}\rangle)|k'\rangle_{Z'}\|_1
+\|\sum_{k'\neq k}\epsilon_{k'}(|k'\rangle|junk_{k'}\rangle)|k\rangle_{Z'}
\|_1\\
&\le&\negl(\secp).
\end{eqnarray*}

\end{proof}




\begin{lemma}
\label{lemma:SVOWSG_equivalence}
If $\frac{1}{2}\|\phi_k-\phi_{k'}\|_1\ge1-2^{-3\secp}$ for any $k\neq k'$,
then the following holds:
there exists a (not necessarily QPT) POVM measurement $\{\Pi_k\}_{k\in\bit^\secp}$ such that
$\mbox{Tr}(\Pi_k\phi_k)\ge1-\negl(\secp)$
and $\mbox{Tr}(\Pi_{k'}\phi_k)\le\negl(\secp)$ for all $k\neq k'$.
\end{lemma}

\begin{proof}
$\frac{1}{2}\|\phi_k-\phi_{k'}\|_1
\ge1-2^{-3\secp}$
means
$F(\phi_k,\phi_{k'})\le 2^{-3\secp+1}$.
From \cref{theorem:Montanaro},
\begin{eqnarray*}
\max_k(1-\mbox{Tr}(\mu_k\phi_k))
&\le& \sum_{k\neq k'}F(\phi_k,\phi_{k'})\\
&\le& 2^{-3\secp+1}(2^{2\secp}-2^\secp)\\
&\le& 2^{-\secp+1},
\end{eqnarray*}
which means $\mbox{Tr}(\mu_k \phi_k)\ge1-2^{-\secp+1}$ and
$\mbox{Tr}(\mu_{k'} \phi_k)\le 2^{-\secp+1}$ for any $k'\neq k$.
\end{proof}


==> backup4.tex <==
\begin{proof}[Proof of \cref{thm:QPOTP_OWSG}]
Let $(\mathsf{OTP}.\KeyGen,\mathsf{OTP}.\Enc,\mathsf{OTP}.\Dec)$ be a QPOTP scheme. From it, we construct a wOWSG as follows.
(From \cref{thm:amplification_OWSG}, it is enough for the existence of OWSGs.)
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    Run $k\gets\mathsf{OTP}.\KeyGen(1^\secp)$.
    Output $k$.
    \item
    $\StateGen(k)\to\phi_k:$
    Choose $x\gets\bit^\ell$.
    Run $\ct_{k,x}\gets \mathsf{OTP}.\Enc(k,x)$.
    Output $\phi_k\coloneqq \ct_{k,x}\otimes |x\rangle\langle x|$.
    \item
    $\Ver(k',\phi_k)\to\top/\bot:$
    Parse $\phi_k=\ct_{k,x}\otimes|x\rangle\langle x|$.
    Run $x'\gets\mathsf{OTP}.\Dec(k',\ct_{k,x})$.
    If $x'=x$, output $\top$. Otherwise, output $\bot$.
\end{itemize}

The correctness is clear. Let us show the security. Assume that it is not secure.
It means that for any polynomial $p$ there exist a QPT adversary $\cA$ and a polynomial $t$ such that
\begin{eqnarray}
\Pr\left[x'=x:
\begin{array}{cc}
    k\gets\mathsf{OTP}.\KeyGen(1^\secp)\\
    x\gets\bit^\ell\\
    \ct_{k,x}\gets \mathsf{OTP}.\Enc(k,x)\\
    k'\gets\cA((\ct_{k,x}\otimes |x\rangle\langle x|)^{\otimes t})\\
    x'\gets\mathsf{OTP}.\Dec(k',\ct_{k,x})
    \end{array}
    \right]\ge1-\frac{1}{p}.
    \label{eq:OWSGfromQPOTP1}
    \end{eqnarray}
    From this $\cA$, we construct a QPT adversary $\cB$ that breaks the security of QPOTP as follows.
    Let $b\in\bit$ be the parameter of the following security game.
   \begin{enumerate}
       \item 
       $\cB$ chooses $x_0,x_1\gets\bit^\ell$, and sends them to the challenger $\cC$.
       \item
       $\cC$ runs $k\gets\mathsf{OTP}.\KeyGen(1^\secp)$.
       \item
       $\cC$ runs $\ct_{k,x_b}\gets\mathsf{OTP}.\Enc(k,x_b)$ $t+1$ times.
       \item
       $\cC$ sends $\ct_{k,x_b}^{\otimes t+1}$ to $\cB$.
       \item
      $\cB$ runs $k'\gets\cA((\ct_{k,x_b}\otimes|x_0\rangle\langle x_0|)^{\otimes t})$. 
      \item
     $\cB$ runs $x'\gets\mathsf{OTP}.\Dec(k',\ct_{k,x_b})$. 
     If $x'=x_0$, $\cB$ outputs $b'=0$.
     Otherwise, it outputs $b'=1$.
   \end{enumerate} 
   It is clear that $\Pr[b'=0|b=0]$ is equivalent to the left-hand-side of Eq.~(\ref{eq:OWSGfromQPOTP1}).
   On the other hand,
   \begin{eqnarray*}
&&   \Pr[b'=0|b=1]\\
&=&
\frac{1}{2^{2\ell}}\sum_{x_0,x_1,k,k'}
   \Pr[k\gets\mathsf{OTP}.\KeyGen(1^\secp)]
   \Pr[k'\gets\cA((\ct_{k,x_1}\otimes|x_0\rangle\langle x_0|)^{\otimes t})]\\
&&\times    \Pr[x_0 \gets\mathsf{OTP}.\Dec(k',\ct_{k,x_1})]\\
&\le&\frac{1}{2^{2\ell}}\sum_{x_0,x_1,k,k'}
   \Pr[k\gets\mathsf{OTP}.\KeyGen(1^\secp)]
   \Pr[x_0 \gets\mathsf{OTP}.\Dec(k',\ct_{k,x_1})]\\
&=&\frac{1}{2^\ell}\sum_{k'}\sum_{x_0}
\Pr\Big[x_0 \gets\mathsf{OTP}.\Dec\Big(k',\frac{1}{2^{\ell}}\sum_{k,x_1}\Pr[k\gets\mathsf{OTP}.\KeyGen(1^\secp)]\ct_{k,x_1}\Big)\Big]\\
&=&\frac{1}{2^\ell}\sum_{k'}\\
&=&\frac{2^\kappa}{2^\ell}\\
&\le&\frac{1}{2}.
   \end{eqnarray*}
   Therefore 
$|\Pr[b'=0|b=0]-\Pr[b'=0|b=1]|$ is non-negligible, which means that the $\cB$ breaks the security of
the QPOTP.
\end{proof}


==> backup5.tex <==
\section{SV-SI-OWSGs}
\label{sec:SVOWSG}

In this section, we define SV-SI-OWSGs (\cref{sec:SVOWSG_def}), and show that SV-SI-OWSGs are equivalent to EFI pairs (\cref{sec:SVOWSG_EFI}).
We also show that private-key quantum money schemes where money states are pure and statistically distinguishable imply
SV-SI-OWSGs.
We also provide a preliminaries section (\cref{sec:SVOWSG_pre}) to give two results used for our proofs.

\subsection{Preliminaries}
\label{sec:SVOWSG_pre}

Let us first explain quantum shadow tomography~\cite{Shadow1,Shadow2},
which we will use later.
The following result gives the best parameters \cite{Shadow_best}.
\begin{theorem}[Quantum shadow tomography~\cite{Shadow_best}]
\label{theorem:shadow}
Let $0<\epsilon<\frac{1}{2}$.
Consider $M$ different POVM elements $E_1,E_2,...,E_M$, i.e.,
$0\le E_i\le I$ for each $i\in\{1,2,...,M\}$.
There exists a (not necessarily polynomial-time) quantum algorithm that, on input
the 
$T$ copies $\rho^{\otimes T}$ of a $d$-dimensional quantum state $\rho$ with
\begin{eqnarray*}
T=\frac{[(\log M)^2+\log(\frac{\log d}{\delta\epsilon})]\log d}{\epsilon^4}
\times O\left(\log\left(\frac{\log d}{\delta\epsilon}\right)\right),
\end{eqnarray*}
outputs $(\eta_1,...,\eta_M)$
such that
$|\eta_j-\mbox{Tr}(E_j\rho)|\le\epsilon$ for all $j\in\{1,2,...,M\}$
with probability at
least $1-\delta$. 
\end{theorem}
In particular, if we take $\epsilon=O(\frac{1}{\poly(\secp)})$,
$\delta=O(\frac{1}{2^{\poly(\secp)}})$, 
$M=O(2^{\poly(\secp)})$, 
and $d=O(2^{\poly(\secp)})$, 
we have $T=O(\poly(\secp))$.


We also use the following result.
\begin{theorem}[\cite{Montanaro19}]
\label{theorem:Montanaro}
Let $\{\rho_i\}_i$ be a set of states.
Define the POVM measurement $\{\mu_i\}_i$ with
$\mu_i\coloneqq\Sigma^{-1/2}\rho_i\Sigma^{-1/2}$,
where $\Sigma\coloneqq \sum_i\rho_i$,
and the inverse is taken on the support of $\Sigma$.
Then,
$\max_i(1-\mbox{Tr}(\mu_i\rho_i))\le\sum_{i\neq j}F(\rho_i,\rho_j)$.
\end{theorem}


\subsection{Definition of SV-SI-OWSGs}
\label{sec:SVOWSG_def}

We first define secretly-verifiable OWSGs (SV-OWSGs) as follows.
\begin{definition}[Secretly-verifiable OWSGs (SV-OWSGs)]\label{def:SV-OWSG}
A secretly-verifiable OWSG (SV-OWSG) is a set of algorithms $(\KeyGen,\StateGen,\Ver)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs a key $k\in\bit^\kappa$.
    \item
    $\StateGen(k)\to\phi_k:$
    It is a QPT algorithm that, on input $k$, outputs an $m$-qubit state $\phi_k$.
    \item
    $\Ver(k',k)\to\top/\bot:$
    It is a QPT algorithm that, on input $k$ and $k'$, outputs $\top/\bot$.
\end{itemize}
We require the following two properties.

\paragraph{\bf Correctness:}
\begin{eqnarray*}
\Pr[\top\gets\Ver(k,k):k\gets\KeyGen(1^\secp)]\ge 1-\negl(\secp).
\end{eqnarray*}

\paragraph{\bf Security:}
For any QPT adversary $\cA$ and any polynomial $t$, 
\begin{eqnarray*}
\Pr[\top\gets\Ver(k',k):k\gets\KeyGen(1^\secp),\phi_k\gets\StateGen(k),k'\gets\cA(\phi_k^{\otimes t})]\le \negl(\secp).
\end{eqnarray*}
\end{definition}

The following lemma shows that, without loss of generality, $\Ver$ can be replaced with the algorithm
of just checking whether $k=k'$ or not.
\begin{lemma}\label{lemma:SVOWSG_amp}
Let $(\KeyGen,\StateGen,\Ver)$ be a SV-OWSG.
Then, the following SV-OWSG $(\KeyGen',\StateGen',\Ver')$ exists.
\begin{itemize}
    \item 
    $\KeyGen'$ and $\StateGen'$ are the same as $\KeyGen$ and $\StateGen$, respectively.
    \item
    $\Ver'(k',k)\to\top/\bot:$
    On input $k$ and $k'$, output $\top$ if $k=k'$.
    Otherwise, output $\bot$.
\end{itemize}
\end{lemma}

\begin{proof}
The correctness of $(\KeyGen',\StateGen',\Ver')$ is clear.
Let us show the security. Assume that it is not secure.
Then there exist a QPT adversary $\cA$, a polynomial $t$, and a polynomial $p$ such that
\begin{eqnarray*}
\sum_k\Pr[k\gets\KeyGen(1^\secp)]\Pr[k\gets\cA(\phi_k^{\otimes t})]\ge \frac{1}{p}.
\end{eqnarray*}
Define the set
\begin{eqnarray*}
S\coloneqq\Big\{k~\Big|~\Pr[k\gets\cA(\phi_k^{\otimes t})]\ge \frac{1}{2p}\Big\}.
\end{eqnarray*}
Then, we have
\begin{eqnarray*}
\sum_{k\in S}\Pr[k\gets\KeyGen(1^\secp)]> \frac{1}{2p}.
\end{eqnarray*}
This is because
\begin{eqnarray*}
\frac{1}{p}&\le&\sum_k\Pr[k\gets\KeyGen(1^\secp)]\Pr[k\gets\cA(\phi_k^{\otimes t})]\\
&=&\sum_{k\in S}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k\gets\cA(\phi_k^{\otimes t})]\\
&&+\sum_{k\notin S}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k\gets\cA(\phi_k^{\otimes t})]\\
&<&\sum_{k\in S}\Pr[k\gets\KeyGen(1^\secp)]+\frac{1}{2p}.
\end{eqnarray*}

Also define the set
\begin{eqnarray*}
T\coloneqq\Big\{k~\Big|~\Pr[\top\gets\Ver(k,k)]\ge 1-\frac{1}{p}\Big\}.
\end{eqnarray*}
Then, we have
\begin{eqnarray*}
\sum_{k\in T}\Pr[k\gets\KeyGen(1^\secp)]> 1-\negl(\secp).
\end{eqnarray*}
This is because
\begin{eqnarray*}
1-\negl(\secp)&\le&\sum_{k}\Pr[k\gets\KeyGen(1^\secp)]\Pr[\top\gets\Ver(k,k)]\\
&=&\sum_{k\in T}\Pr[k\gets\KeyGen(1^\secp)]\Pr[\top\gets\Ver(k,k)]\\
&&+\sum_{k\notin T}\Pr[k\gets\KeyGen(1^\secp)]\Pr[\top\gets\Ver(k,k)]\\
&<&\sum_{k\in T}\Pr[k\gets\KeyGen(1^\secp)]\\
&&+\Big(1-\frac{1}{p}\Big)\Big(1-\sum_{k\in T}\Pr[k\gets\KeyGen(1^\secp)]\Big).
\end{eqnarray*}
Here, the first inequality is from the correctness of $(\KeyGen,\StateGen,\Ver)$.
From the union bound, we have
\begin{eqnarray*}
\sum_{k\in S\cap T}\Pr[k\gets\KeyGen(1^\secp)]> \frac{1}{2p}-\negl(\secp).
\end{eqnarray*}


From the $\cA$, we construct a QPT adversary that breaks the security of $(\KeyGen,\StateGen,\Ver)$ as follows:
On input $\phi_k^{\otimes t}$, run $k'\gets\cA(\phi_k^{\otimes t})$.
Output $k'$.
Then, the probability that $\cB$ breaks the security is
\begin{eqnarray*}
&&\sum_{k,k'}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k'\gets\cA(\phi_k^{\otimes t})]\Pr[\top\gets\Ver(k',k)]\\
&\ge&\sum_k\Pr[k\gets\KeyGen(1^\secp)]\Pr[k\gets\cA(\phi_k^{\otimes t})]\Pr[\top\gets\Ver(k,k)]\\
&\ge&\sum_{k\in S\cap T}\Pr[k\gets\KeyGen(1^\secp)]\Pr[k\gets\cA(\phi_k^{\otimes t})]\Pr[\top\gets\Ver(k,k)]\\
&\ge&\frac{1}{2p}\Big(1-\frac{1}{p}\Big)\Big(\frac{1}{2p}-\negl(\secp)\Big),
\end{eqnarray*}
which is non-negligible.
Therefore $\cB$ breaks the security of
$(\KeyGen,\StateGen,\Ver)$.
\end{proof}

Note that statistically-secure SV-OWSGs are easy to realize.
For example, consider the following construction:
\begin{itemize}
\item
$\KeyGen(1^\secp):$ Sample $k\gets\bit^\secp$.
\item
$\StateGen(k):$ Output $\frac{I^{\otimes m}}{2^m}$.
\item
$\Ver(k',k):$ Output $\top$ if $k'=k$. Otherwise, output $\bot$.
\end{itemize}
We therefore need a constraint to have a meaningful primitive.
We define secretly-verifiable and statistically-invertible OWSGs (SV-SI-OWSGs) as follows.
Introducing the statistical invertibility allows us to avoid trivial constructions with
the statistical security.

\begin{definition}[Secretly-verifiable and statistically-invertible OWSGs (SV-SI-OWSGs)]
A secretly-verifiable and statistically-invertible OWSG (SV-SI-OWSG) is a set of algorithms $(\KeyGen,\StateGen)$ as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    It is a QPT algorithm that, on input the security parameter $\secp$, outputs a key $k\in\bit^\kappa$.
    \item
    $\StateGen(k)\to\phi_k:$
    It is a QPT algorithm that, on input $k$, outputs an $m$-qubit state $\phi_k$.
\end{itemize}
We require the following two properties.

\paragraph{\bf Statistical invertibility:}
There exists a polynomial $p$ such that, for any $k\neq k'$,
\begin{eqnarray*}
\frac{1}{2}\|\phi_k-\phi_{k'}\|_1\ge\frac{1}{p}.
\end{eqnarray*}

\paragraph{\bf Computational non-invertibility:}
For any QPT adversary $\cA$ and any polynomial $t$, 
\begin{eqnarray*}
\Pr[k\gets\cA(\phi_k^{\otimes t}):
k\gets\KeyGen(1^\secp),\phi_k\gets\StateGen(k)]\le \negl(\secp).
\end{eqnarray*}
\end{definition}




The following lemma shows that the statistical invertibility with advantage $\frac{1}{\poly(\secp)}$
can be amplified to $1-2^{-q}$ for any polynomial $q$.
\begin{lemma}
\label{lemma:SVOWSG_amp}
If a SV-SI-OWSG exists
then
a SV-SI-OWSG with statistical invertibility larger than $1-2^{-q}$ with any polynomial $q$ exists.
\end{lemma}

\begin{proof}
Let $(\KeyGen,\StateGen)$ be a SV-SI-OWSG with statistical invertibility larger than $\frac{1}{p}$,
where $p$ is a polynomial.
From it, we construct a new SV-SI-OWSG ($\KeyGen',\StateGen'$) as follows:
\begin{itemize}
    \item 
    $\KeyGen'(1^\secp)\to k$:
    Run $k\gets\KeyGen(1^\secp)$, and output $k$.
    \item
    $\StateGen'(k)\to\phi_k':$
    Run $\phi_k\gets \StateGen(k)$ $2pq$ times, and output
    $\phi_k'\coloneqq \phi_k^{\otimes 2pq}$.
\end{itemize}
First, for any $k\neq k'$,
\begin{eqnarray*}
\frac{1}{2}\|\phi_k'-\phi_{k'}'\|_1
&=&\frac{1}{2}\|\phi_k^{\otimes 2pq}-\phi_{k'}^{\otimes 2pq}\|_1\\
&\ge& 1-\exp(-2qp\|\phi_k-\phi_{k'}\|_1/4)\\
&\ge& 1-\exp(-q)\\
&\ge& 1-2^{-q},
\end{eqnarray*}
which shows the statistical invertibility of $(\KeyGen',\StateGen')$ with the advantage
larger than $1-2^{-q}$.
Second, from the computational non-invertibility of $(\KeyGen,\StateGen)$, 
\begin{eqnarray*}
&&\Pr[k\gets\cA(\phi_k'^{\otimes t}):k\gets\KeyGen'(1^\secp),\phi_k'\gets\StateGen'(k)]\\
&=&\Pr[k\gets\cA(\phi_k^{\otimes 2pqt}):k\gets\KeyGen(1^\secp),\phi_k\gets\StateGen(k)]\\
&\le& \negl(\secp)
\end{eqnarray*}
for any QPT adversary $\cA$ and any polynomial $t$, 
which shows the computational non-invertibility of $(\KeyGen',\StateGen')$.
\end{proof}

The following lemma shows that the statistical invertibility 
is equivalent to the existence of a (unbounded) adversary that can find
the correct $k$ given many copies of $\phi_k$ except for a negligible error.
\begin{lemma}
\label{lemma:SVOWSG_equivalence}
The statistical invertibility is satisfied if and only if the 
following is satisfied:
There exists a 
(not necessarily QPT) POVM measurement $\{\Pi_k\}_{k\in\bit^\kappa}$ 
and a polynomial $t$ such that
$\mbox{Tr}(\Pi_k\phi_k^{\otimes t})\ge1-\negl(\secp)$
and $\mbox{Tr}(\Pi_{k'}\phi_k^{\otimes t})\le\negl(\secp)$ for all $k\neq k'$.

\if0
If $\frac{1}{2}\|\phi_k-\phi_{k'}\|_1\ge1-2^{-3\secp}$ for any $k\neq k'$,
then the following holds:
there exists a (not necessarily QPT) POVM measurement $\{\Pi_k\}_{k\in\bit^\secp}$ such that
$\mbox{Tr}(\Pi_k\phi_k)\ge1-\negl(\secp)$
and $\mbox{Tr}(\Pi_{k'}\phi_k)\le\negl(\secp)$ for all $k\neq k'$.
\fi
\end{lemma}

\begin{proof}
First, we show the if part.
Assume that
there exists a 
POVM measurement $\{\Pi_k\}_{k\in\bit^\kappa}$ and a polynomial $t$ such that
$\mbox{Tr}(\Pi_k\phi_k^{\otimes t})\ge1-\negl(\secp)$
and $\mbox{Tr}(\Pi_{k'}\phi_k^{\otimes t})\le\negl(\secp)$ for all $k\neq k'$.
Then,
\begin{eqnarray*}
\frac{1}{2}\|\phi_k^{\otimes t}-\phi_{k'}^{\otimes t}\|_1
&\ge&
\Tr(\Pi_k \phi_k^{\otimes t})
-\Tr(\Pi_k \phi_{k'}^{\otimes t})\\
&\ge&
1-\negl(\secp)
-\negl(\secp)\\
&=&1-\negl(\secp).
\end{eqnarray*}
for all $k\neq k'$.
Therefore,
\begin{eqnarray*}
\frac{t}{2}\|\phi_k-\phi_{k'}\|_1
&\ge&
\frac{1}{2}\|\phi_k^{\otimes t}-\phi_{k'}^{\otimes t}\|_1\\
&\ge&
1-\negl(\secp),
\end{eqnarray*}
which means
\begin{eqnarray*}
\frac{1}{2}\|\phi_k-\phi_{k'}\|_1
&\ge&
\frac{1}{t}-\negl(\secp)\\
&\ge&
\frac{1}{2t}
\end{eqnarray*}
for all $k\neq k'$.

Next, we show the only if part.
Assume that the statistical invertibility is satisfied.
Then, there exists a polynomial $p$ such that
$\frac{1}{2}\|\phi_k-\phi_{k'}\|_1\ge\frac{1}{p}$
for all $k\neq k'$.
Let $t\coloneqq 6p\kappa$. Then,
\begin{eqnarray*}
\frac{1}{2}\|\phi_k^{\otimes t}-\phi_{k'}^{\otimes t}\|_1
&\ge&
1-e^{-t\frac{\|\phi_k-\phi_{k'}\|_1}{4}}\\
&\ge&
1-e^{-3\kappa}\\
&\ge&
1-2^{-3\kappa},
\end{eqnarray*}
which 
means
$F(\phi_k^{\otimes t},\phi_{k'}^{\otimes t})\le 2^{-3\kappa+1}$.
From \cref{theorem:Montanaro},
\begin{eqnarray*}
\max_k(1-\mbox{Tr}(\mu_k\phi_k^{\otimes t}))
&\le& \sum_{k\neq k'}F(\phi_k^{\otimes t},\phi_{k'}^{\otimes t})\\
&\le& 2^{-3\kappa+1}(2^{2\kappa}-2^\kappa)\\
&\le& 2^{-\kappa+1},
\end{eqnarray*}
which means $\mbox{Tr}(\mu_k \phi_k^{\otimes t})\ge1-2^{-\kappa+1}$ and
$\mbox{Tr}(\mu_{k'} \phi_k^{\otimes t})\le 2^{-\kappa+1}$ for any $k'\neq k$.
\end{proof}



\subsection{Equivalence of SV-SI-OWSGs and EFI Pairs}
\label{sec:SVOWSG_EFI}

\begin{theorem}\label{thm:SVSIOWSG_EFI}
SV-SI-OWSGs exist if and only if EFI pairs exist.
\end{theorem}
This Theorem is shown by combining the following two theorems.

\begin{theorem}\label{thm:SVSIOWSGfromEFI}
If EFI pairs exist then SV-SI-OWSGs exist.
\end{theorem}

\begin{theorem}\label{thm:EFIfromSVSIOWSG}
If 
SV-SI-OWSGs exist
then EFI pairs exist. 
\end{theorem}

\begin{proof}[Proof of \cref{thm:SVSIOWSGfromEFI}]
We show that if
EFI pairs exist then SV-SI-OWSGs exist.
Let $\mathsf{EFI}.\StateGen(1^\secp,b)\to\rho_b$ be an EFI pair.
As is explained in \cref{remark:EFI}, we can assume without loss of generality that
$\frac{1}{2}\|\rho_0-\rho_1\|_1\ge1-\negl(\secp)$,
which means $F(\rho_0,\rho_1)\le\negl(\secp)$.
From the EFI pair, we construct a SV-SI-OWSG as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    Choose $k\gets\bit^\kappa$, and ouput $k$.
    \item
    $\StateGen(k)\to\phi_k:$
    Run $\mathsf{EFI}.\StateGen(1^\secp,k_i)\to\rho_{k_i}$ for each $i\in[\kappa]$.
    Output $\phi_k\coloneqq \bigotimes_{i=1}^\kappa \rho_{k_i}$.
\end{itemize}

The statistical invertibility is easily shown as follows. 
If $k\neq k'$, there exists a $j\in[\kappa]$ such that $k_j\neq k_j'$.
Then,
\begin{eqnarray*}
F(\phi_k,\phi_{k'})&=&\prod_{i=1}^\kappa F(\rho_{k_i},\rho_{k_i'})\\
&\le& F(\rho_{k_j},\rho_{k_j'})\\
&\le&\negl(\secp),
\end{eqnarray*}
which means $\frac{1}{2}\|\phi_k-\phi_{k'}\|_1\ge1-\negl(\secp)$.
This shows the statistical invertibility.

Let us next show the computational non-invertibility.
From the standard hybrid argument, and the computational indistinguishability of $\rho_0$ and $\rho_1$, we have
\begin{eqnarray}
|\Pr[k\gets\cA(\phi_k^{\otimes t})]-\Pr[k\gets\cA(\phi_{0^\kappa}^{\otimes t})]|\le\negl(\secp)
\label{SVSIOWSGsfromEFI_hybrid}
\end{eqnarray}
for any $k$ and any polynomial $t$.
(It will be shown later.)

Hence
\begin{eqnarray*}
&&\Pr[k\gets\cA(\phi_k^{\otimes t}):k\gets\KeyGen(1^\secp),\phi_k\gets\StateGen(k)]\\
&=&\frac{1}{2^\kappa}\sum_{k\in\bit^\kappa}\Pr[k\gets\cA(\phi_k^{\otimes t})]\\
&\le&\frac{1}{2^\kappa}\sum_{k\in\bit^\kappa}(\Pr[k\gets\cA(\phi_{0^\kappa}^{\otimes t})]+\negl(\secp))\\
&=&\frac{1}{2^\kappa}+\negl(\secp),
\end{eqnarray*}
which shows the computational non-invertibility.


Let us show Eq.~(\ref{SVSIOWSGsfromEFI_hybrid}).
For each $z\in\bit^{\kappa t}$,
define $\Phi_z\coloneqq\bigotimes_{i=1}^{\kappa t}\rho_{z_i}$.
Let $z,z'\in\bit^{\kappa t}$ be two bit strings 
such that, for a $j\in[\kappa t]$, $z_j=0$, $z'_j=1$, and $z_i=z'_i$ for all $i\neq j$.
Then, we can show that
\begin{eqnarray*}
|\Pr[1\gets\cA(\Phi_z)]
-\Pr[1\gets\cA(\Phi_{z'})]|\le\negl(\secp)
\end{eqnarray*}
for any QPT adversary $\cA$. 
In fact, assume that
\begin{eqnarray*}
|\Pr[1\gets\cA(\Phi_z)]
-\Pr[1\gets\cA(\Phi_{z'})]|\ge \frac{1}{\poly(\secp)}
\end{eqnarray*}
for a QPT adversary $\cA$. 
Then, from this $\cA$, we can construct a QPT adversary $\cB$ that breaks the security of
the EFI pair as follows:
On input $\rho_b$, run $b'\gets \cA((\bigotimes_{i=1}^{j-1}\rho_{z_i})\otimes \rho_b \otimes(\bigotimes_{i=j+1}^{\kappa t}\rho_{z_i}))$,
and output $b'$.
Because
$\Pr[b'=1|b=0]=\Pr[1\gets\cA(\Phi_z)]$
and
$\Pr[b'=1|b=1]=\Pr[1\gets\cA(\Phi_{z'})]$,
the $\cB$ breaks the security of the EFI pair.

By applying the operation that change 0 to 1 in polynomial times, we can always 
map $0^{\kappa t}$ to $k^t$ for any $k\in\bit^\kappa$, and therefore Eq.~(\ref{SVSIOWSGsfromEFI_hybrid}) is shown.
\end{proof}



\begin{proof}[Proof of \cref{thm:EFIfromSVSIOWSG}]
We show that
if SV-SI-OWSGs exist then EFI pairs exist.
Let $(\mathsf{OWSG}.\KeyGen,\mathsf{OWSG}.\StateGen)$ be a SV-SI-OWSG.
Without loss of generality, we can assume that
$\mathsf{OWSG}.\KeyGen$ is the following algorithm:
first apply a QPT unitary $U$ on $|0...0\rangle$ to generate 
\begin{eqnarray*}
U|0...0\rangle=\sum_{k}\sqrt{\Pr[k\gets\mathsf{OWSG}.\KeyGen(1^\secp)]}|k\rangle|\mu_k\rangle, 
\end{eqnarray*}
and trace out the second register,
where $\{|\mu_k\rangle\}_k$ are some normalized states.
Moreover, without loss of generality, we can also assume that $\mathsf{OWSG}.\StateGen$ is the following algorithm:
first apply a QPT unitary $V_k$ that depends on $k$ on $|0...0\rangle$ to generate 
$V_k|0...0\rangle=|\psi_k\rangle_{\regA,\regB}$, and trace out the register $\regA$.

From the SV-SI-OWSG, we want to construct an EFI pair.
For that goal, we construct a statistically-hiding and computationally-binding canonical quantum bit commitment scheme from
SV-SI-OWSG. Due to \cref{thm:convertingflavors} (the equivalence between different flavors of commitments), we then have
a statistically-binding and computationally-hiding canonical quantum bit commitment scheme, which is equivalent to an EFI pair.
From the SV-SI-OWSG, we construct
a statistically-hiding and computationally-binding canonical quantum bit commitment scheme $\{Q_0,Q_1\}$ as follows.
\begin{eqnarray*}
Q_0|0\rangle_{\regC,\regR}&\coloneqq&\sum_{k}\sqrt{\Pr[k]} 
(|k\rangle|\mu_k\rangle)_{\regC_1}
|\psi_k\rangle_{\regC_2,\regR_2}^{\otimes t}|0\rangle_{\regR_3},\\
Q_1|0\rangle_{\regC,\regR}&\coloneqq& \sum_{k}\sqrt{\Pr[k]}
(|k\rangle|\mu_k\rangle)_{\regC_1}
|\psi_k\rangle_{\regC_2,\regR_2}^{\otimes t}|k\rangle_{\regR_3},
\end{eqnarray*}
where $\Pr[k]\coloneqq\Pr[k\gets\mathsf{OWSG}.\KeyGen(1^\secp)]$, $\regC_2$ is the combination of all ``$\regA$ registers'' of $|\psi_k\rangle$,
$\regR_2$ is the combination of all ``$\regB$ registers'' of $|\psi_k\rangle$,
$\regC\coloneqq(\regC_1,\regC_2)$ and $\regR\coloneqq(\regR_2,\regR_3)$.
Moreover, $t$ is a polynomial specified later.
It is clear that such $\{Q_0,Q_1\}$ is implemented in QPT in a natural way.

Let us first show the computational binding of $\{Q_0,Q_1\}$.
Assume that it is not computationally binding. Then, there exists a QPT unitary $U$, an ancilla state $|\tau\rangle$,
and a polynomial $p$ such that
\begin{eqnarray*}
\|
(\langle 0|Q_1^\dagger)_{\regC,\regR} U_{\regR,\regZ}(Q_0|0\rangle_{\regC,\regR}\otimes|\tau\rangle_\regZ)
\|
\ge\frac{1}{p}.
\end{eqnarray*}
Then,
\begin{eqnarray}
\frac{1}{p^2}
&\le&
\|
(\langle 0|Q_1^\dagger)_{\regC,\regR} U_{\regR,\regZ}(Q_0|0\rangle_{\regC,\regR}\otimes|\tau\rangle_\regZ)
\|^2\nonumber\\
&=&
\Big\|
\Big(\sum_{k'}\sqrt{\Pr[k']}\langle k',\mu_{k'}|_{\regC_1}\langle\psi_{k'}|^{\otimes t}_{\regC_2,\regR_2}\langle k'|_{\regR_3}\Big)\nonumber\\
&&\times\Big(\sum_{k}\sqrt{\Pr[k]}|k,\mu_k\rangle_{\regC_1}U_{\regR,\regZ}|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}|0\rangle_{\regR_3}|\tau\rangle_\regZ\Big)
\Big\|^2\nonumber\\
&=&
\Big\|
\sum_{k}\Pr[k]
\langle\psi_{k}|^{\otimes t}_{\regC_2,\regR_2}\langle k|_{\regR_3}
U_{\regR,\regZ}|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}|0\rangle_{\regR_3}|\tau\rangle_\regZ
\Big\|^2\nonumber\\
&\le&
\Big(
\sum_{k}\Pr[k]
\Big\|\langle\psi_{k}|^{\otimes t}_{\regC_2,\regR_2}\langle k|_{\regR_3}
U_{\regR,\regZ}|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}|0\rangle_{\regR_3}|\tau\rangle_\regZ
\Big\|\Big)^2\nonumber\\
&\le&
\sum_{k}\Pr[k]
\Big\|
\langle\psi_{k}|^{\otimes t}_{\regC_2,\regR_2}\langle k|_{\regR_3}
U_{\regR,\regZ}|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}|0\rangle_{\regR_3}|\tau\rangle_\regZ
\Big\|^2\nonumber\\
&\le&
\sum_{k}\Pr[k]
\Big\|
\langle k|_{\regR_3}
U_{\regR,\regZ}|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}|0\rangle_{\regR_3}|\tau\rangle_\regZ
\Big\|^2.
\label{POWSG_B}
\end{eqnarray}
In the third inequality, we have used Jensen's inequality.\footnote{For a real convex function $f$, $f(\sum_i p_i x_i)\le\sum_i p_i f(x_i)$.}
From this $U$, we construct a QPT adversary $\cB$ that breaks the computational non-invertibility of the SV-SI-OWSG as follows:
On input the $\regR_2$ register of $|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}$, apply $U_{\regR,\regZ}$ on
$|\psi_k\rangle_{\regC_2,\regR_2}^{\otimes t}|0\rangle_{\regR_3}|\tau\rangle_\regZ$, and measure
the $\regR_3$ register in the computational basis. Output the result.
Then, the probability that $\cB$
correctly outputs $k$ is equal to Eq.~(\ref{POWSG_B}).
Therefore, $\cB$ breaks the computational non-invertibility of the SV-SI-OWSG.


Let us next show the statistical hiding of $\{Q_0,Q_1\}$.
In the following, we construct a (not necessarily QPT) unitary $W_{\regR,\regZ}$ such that
\begin{eqnarray}
\|W_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ
-Q_1|0\rangle_{\regC,\regR}|0\rangle_\regZ \|_1
&\le&\negl(\secp).
\label{SVOWSG_V}
\end{eqnarray}
Then, we have
\begin{eqnarray*}
&&\|\mbox{Tr}_{\regR}(Q_0|0\rangle_{\regC,\regR})
-\mbox{Tr}_{\regR}(Q_1|0\rangle_{\regC,\regR})\|_1\\
&=&
\|\mbox{Tr}_{\regR,\regZ}(Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ)
-\mbox{Tr}_{\regR,\regZ}(Q_1|0\rangle_{\regC,\regR}|0\rangle_\regZ)\|_1\\
&=&
\|\mbox{Tr}_{\regR,\regZ}(W_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ)
-\mbox{Tr}_{\regR,\regZ}(Q_1|0\rangle_{\regC,\regR}|0\rangle_\regZ)\|_1\\
&\le&
\|W_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_\regZ
-Q_1|0\rangle_{\regC,\regR}|0\rangle_\regZ\|_1\\
&\le&
\negl(\secp),
\end{eqnarray*}
which shows the statistical hiding of $\{Q_0,Q_1\}$.

Now we explain how to construct $W_{\regR,\regZ}$.
\mor{Shadow tukawazuni sonomama POVM sokuteisureba?}
From \cref{lemma:SVOWSG_equivalence}, there exists a (not necessarily QPT) POVM measurement 
$\{\Pi_k\}_k$ and a polynomial $r$ such that
$\mbox{Tr}(\Pi_k \phi_k^{\otimes r})\ge1-\negl(\secp)$ and
$\mbox{Tr}(\Pi_{k'} \phi_k^{\otimes r})\le\negl(\secp)$ for all $k\neq k'$.
With this POVM measurement $\{\Pi_k\}_k$, we construct
the following quantum (not necessarily polynomial-time) algorithm, which we call $\mathsf{Shadow}$. 
\paragraph{$\mathsf{Shadow}(\rho^{\otimes t})\to k^*$}: 
\begin{enumerate}
    \item 
On input $t$ copies of a state $\rho$,
run the shadow tomography algorithm (\cref{theorem:shadow}) to get
$\{\eta_k\}_{k\in\bit^\kappa}$ such that $|\mbox{Tr}(\Pi_k\rho)-\eta_k|\le\frac{1}{\poly(\secp)}$ for each $k\in\bit^\kappa$.
\item
If there is a $k^*$ such that $\eta_{k^*}\ge 1-\frac{1}{\poly(\secp)}$, output the $k^*$.
\end{enumerate}
Due to the correctness of the shadow tomography algorithm,
there exists a polynomial $t$ such that
$\Pr[k\gets\mathsf{Shadow}(\phi_k^{\otimes t})]\ge1-\negl(\secp)$
for all $k$.

Let $U_{\regR_2,\regZ}$ be a unitary that implements $\mathsf{Shadow}$. In other words,
\begin{eqnarray*}
U_{\regR_2,\regZ}|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}|0...0\rangle_\regZ
&=&\sqrt{1-\epsilon_k}|k\rangle|junk_k\rangle+\sum_{k':k'\neq k} \sqrt{\epsilon_{k'}}|k'\rangle|junk_{k'}\rangle,
\end{eqnarray*}
\mor{k atereru kara, $\ket{\psi_k}$ tukurerukara, $U$ wa cloner ni natteru. Yotte $|\psi_k\rangle$ wa tyokkou.}
where $\regZ$ is the ancilla register, $\epsilon_k$ is a real number such that $1-\epsilon_k\ge1-\negl(\secp)$,
and $|junk_k\rangle$ are ``junk'' states that are normalized.
Let $V_{\regR,\regZ}$ be the following unitary:\footnote{For simplicity, we define $V_{\regR,\regZ}$ by explaining how it acts on
$|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}|0...0\rangle_\regZ|0\rangle_{\regR_3}$, but it is clear from the explanation how $V_{\regR,\regZ}$ is defined.}
\begin{enumerate}
    \item 
    Apply $U_{\regR_2,\regZ}$ on $|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}|0...0\rangle_\regZ|0\rangle_{\regR_3}$:
    \begin{eqnarray*}
U_{\regR_2,\regZ}|\psi_k\rangle^{\otimes t}_{\regC_2,\regR_2}|0...0\rangle_\regZ|0\rangle_{\regR_3}
&=&\Big[\sqrt{1-\epsilon_k}|k\rangle|junk_k\rangle\\
&&+\sum_{k':k'\neq k} \sqrt{\epsilon_{k'}}|k'\rangle|junk_{k'}\rangle\Big]|0\rangle_{\regR_3}.
    \end{eqnarray*}
    \item
    Copy the content of the first register to the register $\regR_3$:
     \begin{eqnarray*}
\sqrt{1-\epsilon_k}|k\rangle|junk_k\rangle|k\rangle_{\regR_3}
+\sum_{k':k'\neq k} \sqrt{\epsilon_{k'}}|k'\rangle|junk_{k'}\rangle|k'\rangle_{\regR_3}.
    \end{eqnarray*}
\end{enumerate}
Define $W_{\regR,\regZ}\coloneqq U_{\regR_2,\regZ}^\dagger V_{\regR,\regZ}$.

Let us show that thus constructed $W_{\regR,\regZ}$ satisfies Eq.~(\ref{SVOWSG_V}).
\begin{eqnarray*}
&&\Big((\langle 0|Q_1^\dagger)_{\regC,\regR}\langle 0|_{\regZ}\Big)
\Big(W_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_{\regZ}\Big)\\
&=&\Big((\langle 0|Q_1^\dagger)_{\regC,\regR}\langle 0|_{\regZ}\Big)
\Big(U_{\regR_2,\regZ}^\dagger V_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_{\regZ}\Big)\\
&=&\Big((\langle 0|Q_1^\dagger)_{\regC,\regR}\langle 0|_{\regZ}
U_{\regR_2,\regZ}^\dagger 
\Big)
\Big(
V_{\regR,\regZ}Q_0|0\rangle_{\regC,\regR}|0\rangle_{\regZ}\Big)\\
&=&
\Big(\sum_k\sqrt{\Pr[k]}(\langle k|\langle \mu_k|)_{\regC_1}
\Big[\sqrt{1-\epsilon_k}\langle k|\langle junk_k|\langle k|_{\regR_3}
+\sum_{k'\neq k}\sqrt{\epsilon_{k'}}\langle k'|\langle junk_{k'}|\langle k|_{\regR_3}\Big]\Big)\\
&&\times\Big(\sum_k\sqrt{\Pr[k]}(| k\rangle|\mu_k\rangle)_{\regC_1}
\Big[\sqrt{1-\epsilon_k}| k\rangle | junk_k\rangle| k\rangle_{\regR_3}
+\sum_{k'\neq k}\sqrt{\epsilon_{k'}}| k'\rangle| junk_{k'}\rangle| k'\rangle_{\regR_3}\Big]\Big)\\
&=&
\sum_k\Pr[k]
(1-\epsilon_k)\\
&\ge&1-\negl(\secp).
\end{eqnarray*}

\end{proof}


\subsection{SV-SI-OWSGs from quantum money}
\label{sec:SVSIOWSGfromQmoney}

\begin{theorem}
If private-key quantum money schemes with pure money states that satisfy
$\frac{1}{2}\||\$_k\rangle\langle\$_k|-|\$_{k'}\rangle\langle\$_{k'}|\|_1\ge\frac{1}{\poly(\secp)}$
for all $k\neq k'$
exist,
then SV-SI-OWSGs exist.
\end{theorem}

\begin{proof}
Let $(\mathsf{QM}.\KeyGen,\mathsf{QM}.\Mint,\mathsf{QM}.\Ver)$
be a private-key quantum money scheme with pure money states that satisfies
$\frac{1}{2}\||\$_k\rangle\langle\$_k|-|\$_{k'}\rangle\langle\$_{k'}|\|_1\ge\frac{1}{\poly(\secp)}$
for all $k\neq k'$.
From it, we construct a SV-SI-OWSGs as follows.
\begin{itemize}
    \item 
    $\KeyGen(1^\secp)\to k:$
    Run $k\gets\mathsf{QM}.\KeyGen(1^\secp)$, and output $k$.
    \item
   $\StateGen(k)\to |\phi_k\rangle:$ 
   Run $|\$_k\rangle\gets\mathsf{QM}.\Mint(k)$, and output $|\phi_k\rangle\coloneqq|\$_k\rangle$.
\end{itemize}

The statistical invertibility is clear.
Let us show the computational non-invertibility.
Assume that it does not satisfy computational non-invertibility.
Then,
there exists a QPT adversary $\cA$, a polynomial $t$, and a polynomial $p$ such that
\begin{eqnarray*}
\sum_k\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\Pr[k\gets\cA(|\$_k\rangle^{\otimes t})]\ge\frac{1}{p}.
\end{eqnarray*}
Let us define the set
\begin{eqnarray*}
S\coloneqq\Big\{k~\Big|~\Pr[k\gets\cA(|\$_k\rangle^{\otimes t})]\ge\frac{1}{2p}\Big\}.
\end{eqnarray*}
Then we have
\begin{eqnarray*}
\sum_{k\in S}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\ge\frac{1}{2p}.
\end{eqnarray*}
Let us also define the set 
\begin{eqnarray*}
T\coloneqq\Big\{k~\Big|~\Pr[\top\gets\mathsf{QM}.\Ver(k,\ket{\$_k})]\ge 1-\frac{1}{2(t+1)}\Big\}.
\end{eqnarray*}
Then, we have
\begin{eqnarray*}
\sum_{k\in T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]\ge1-\negl(\secp).
\end{eqnarray*}
From the union bound,
\begin{eqnarray*}
\sum_{k\in S\cap T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
&\ge& \frac{1}{2p}+1-\negl(\secp)-1\\
&\ge& \frac{1}{2p}-\negl(\secp).
\end{eqnarray*}

From the $\cA$, we construct a QPT adversary $\cB$ that breaks the security of
the private-key quantum money scheme as follows:
On input $|\$_k\rangle^{\otimes t}$, run $k'\gets\cA(\ket{\$_k}^{\otimes t})$, 
run $\ket{\$_{k'}}^{\otimes t+1}\gets\mathsf{QM}.\Mint(k')$, and output $\xi\coloneqq \ket{\$_{k'}}^{\otimes t+1}$.
The probability that the $\cB$ breaks the security of the private-key quantum money scheme is
\begin{eqnarray*}
&&\sum_{k,k'}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
\Pr[k'\gets\cA(\ket{\$_k}^{\otimes t})]\Pr[\mathsf{Count}(k,|\$_{k'}\rangle^{\otimes t+1})\ge t+1]\\
&\ge&\sum_k\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
\Pr[k\gets\cA(\ket{\$_k}^{\otimes t})]\Pr[\mathsf{Count}(k,|\$_k\rangle^{\otimes t+1})\ge t+1]\\
&=&
\sum_k\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
\Pr[k\gets\cA(\ket{\$_k}^{\otimes t})]
\Pr[\top\gets\mathsf{QM}.\Ver(k,\ket{\$_k})]^{t+1}\\
&\ge&
\sum_{k\in S\cap T}\Pr[k\gets\mathsf{QM}.\KeyGen(1^\secp)]
\Pr[k\gets\cA(\ket{\$_k}^{\otimes t})]
\Pr[\top\gets\mathsf{QM}.\Ver(k,\ket{\$_k})]^{t+1}\\
&\ge&
\frac{1}{2p}
\Big(1-\frac{1}{2(t+1)}\Big)^{t+1}
\Big(\frac{1}{2p}-\negl(\secp)\Big)\\
&\ge&
\frac{1}{2p}
\Big(1-\frac{1}{2}\Big)
\Big(\frac{1}{2p}-\negl(\secp)\Big),
\end{eqnarray*}
which is non-negligible.
Here, in the last inequality, we have used Bernoulli's inequality.
The $\cB$ therefore breaks the security of the private-key quantum money scheme.

\end{proof}



==> computationallyinconvertiblestates.tex <==
\section{Computationally inconvertible states generators}

\begin{definition}[Computationally inconvertible states generators (CISG)]
A QPT algorithm $\StateGen(1^\secp,b)\to|\psi_b\rangle_{AB}$ that, on input the security parameter $\secp$ and a bit $b\in\bit$,
outputs a quantum state $|\psi_b\rangle_{AB}$ on registers $A$ and $B$ is called a computationally inconvertible states generator
if 
%$|\langle\psi_0|\psi_1\rangle|\le\negl(\secp)$, and 
for any QPT unitary $U$ and any $\poly(\secp)$-qubit state $|\tau\rangle$,
%\begin{eqnarray*}
%&&\|(\langle \psi_1|_{AB}\otimes I_C) (I_A\otimes U_{BC})(|\psi_0\rangle_{AB}|\tau\rangle_C)\\
%&+&(\langle \psi_0|_{AB}\otimes I_C) (I_A\otimes U_{BC})(|\psi_1\rangle_{AB}|\tau\rangle_C)
%\|\le\negl(\secp).
%\end{eqnarray*}
\begin{eqnarray*}
&&|(\langle \psi_1|_{AB}\langle\tau|_C) (I_A\otimes U_{BC})(|\psi_0\rangle_{AB}|\tau\rangle_C)\\
&+&(\langle \psi_0|_{AB}\langle\tau|_C) (I_A\otimes U_{BC})(|\psi_1\rangle_{AB}|\tau\rangle_C)
|\le\negl(\secp).
\end{eqnarray*}
\end{definition}
\mor{Statistical convertibility is necessary as well, and if it is required, CISG is equivalent to EFI
due to AAS.}

\begin{theorem}
EFI pairs imply CISGs.
\end{theorem}

\begin{proof}
Let $\mathsf{EFI}.\StateGen(1^\secp,b)\to\rho_b$ be an EFI pair.
Without loss of generality, we can assume that it applies a QPT unitary $U_{1^\secp,b}$ on $|0...0\rangle_{AB}$ 
to generate $|\psi_b\rangle_{AB}\coloneqq U_{1^\secp,b}|0...0\rangle_{AB}$, and traces out the $A$ register to get
the state $\rho_b$ of the $B$ register.
Define $\mathsf{CISG}.\StateGen(1^\secp,b)$ be a QPT algorithm that outputs
\begin{eqnarray*}
|x\rangle\coloneqq\frac{|0\rangle|\psi_0\rangle+|1\rangle|\psi_1\rangle}{\sqrt{2}}
\end{eqnarray*}
if $b=0$ and
\begin{eqnarray*}
|y\rangle\coloneqq\frac{|0\rangle|\psi_0\rangle-|1\rangle|\psi_1\rangle}{\sqrt{2}}
\end{eqnarray*}
if $b=1$
in the obvious way by running the controlled $U_{1^\secp,b}$.
We claim that $\mathsf{CISG}.\StateGen$ is a CISG.

\if0
Due to the statistical distinguishability of EFI pairs,
\begin{eqnarray*}
\frac{1}{2}\||\psi_0\rangle\langle\psi_0|-|\psi_1\rangle\langle\psi_1|\|_1
\ge\frac{1}{2}\|\rho_0-\rho_1\|_1
\ge1-\negl(\secp),
\end{eqnarray*}
which means that $|\langle\psi_0|\psi_1\rangle|^2\le\negl(\secp)$.
\fi

Due to the computational indistinguishability of EFI pairs,
we have that for any (non-uniform) QPT adversary $\cA$,
\begin{eqnarray*}
|\Pr[1\gets\cA(\rho_0)]-\Pr[1\gets\cA(\rho_1)]|\le\negl(\secp).
\end{eqnarray*}
Equivalently,
for any (non-uniform) QPT adversary $\cA$ who can act on only the register $B$,
\begin{eqnarray*}
|\Pr[1\gets\cA(|\psi_0\rangle_{AB}|0\rangle_C)]-\Pr[1\gets\cA(|\psi_1\rangle_{AB}|1\rangle_C)]|\le\negl(\secp).
\end{eqnarray*}
Due to \cite{HMY22}, it means that for any QPT unitary $U$ and any $\poly(\secp)$-qubit state $|\tau\rangle$,
\begin{eqnarray*}
&&\|(\langle x|_{ABC}\otimes I_D) (I_{AC}\otimes U_{BD})(|y\rangle_{ABC}|\tau\rangle_{D})\\
&+&
(\langle y|_{ABC}\otimes I_D)(I_{AC}\otimes U_{BD})(|x\rangle_{ABC}|\tau\rangle_D)\|
\le\negl(\secp).
\end{eqnarray*}

\end{proof}

\begin{theorem}
OWSGs imply CISGs.
\end{theorem}

\begin{proof}
Let $\mathsf{OWSG}.\StateGen(1^\secp,k)\to|\phi_k\rangle$ be a OWSG.
Define
\begin{eqnarray*}
|\psi_0\rangle_{AB}&\coloneqq&\frac{1}{\sqrt{2^n}}\sum_{k\in\bit^n} |k\rangle_A\otimes|k0^{m-n}\rangle_B,\\
|\psi_1\rangle_{AB}&\coloneqq&\frac{1}{\sqrt{2^n}}\sum_{k\in\bit^n}|k\rangle_A\otimes|\phi_k\rangle_B.
\end{eqnarray*}
%\begin{eqnarray*}
%|\psi_b\rangle\coloneqq\frac{1}{\sqrt{2^n}}\sum_{k\in\bit^n} |k\rangle_A\otimes\Big(\frac{|0\rangle|k0^{m-n}\rangle+(-1)^b|1\rangle|\phi_k\rangle}{\sqrt{2}}\Big)_B.
%\end{eqnarray*}
\mor{They are not statistically convertible unless $|\phi_k\rangle$ are orthogonal with each other.}
Let $\mathsf{CISG}.\StateGen(1^\secp,b)$ be a QPT algorithm that outputs $|\psi_b\rangle$ in the obvious way.
We claim that $\mathsf{CISG}.\StateGen$ is a CISG.
In fact, assume that there exists a QPT unitary $U$ and a $\poly(\secp)$-qubit state $|\tau\rangle$ such that
\begin{eqnarray*}
&&\|(\langle \psi_0|_{AB}\otimes I_C) (I_A\otimes U_{BC})(|\psi_1\rangle_{AB}|\tau\rangle_{C})\\
&+&
(\langle \psi_1|_{AB}\otimes I_C)(I_A\otimes U_{BC})(|\psi_0\rangle_{AB}|\tau\rangle_C)\|
=\Gamma
\end{eqnarray*}
with a non-negligible $\Gamma$.
It means that
$\|(\langle \psi_0|_{AB}\otimes I_C) (I_A\otimes U_{BC})(|\psi_1\rangle_{AB}|\tau\rangle_{C})\|\ge\Gamma$
or
$\|(\langle \psi_1|_{AB}\otimes I_C)(I_A\otimes U_{BC})(|\psi_0\rangle_{AB}|\tau\rangle_C)\|\ge\Gamma$.
Without loss of generality, we assume the former.
Then, we have
\begin{eqnarray*}
\Delta^2
&\le&
\Big|\Big(\frac{1}{\sqrt{2^n}}\sum_k\langle k|_A\langle k0^{m-n}|_B\Big)\langle\tau|_C 
(I_A\otimes U_{BC})
\Big(\frac{1}{\sqrt{2^n}}\sum_k|k\rangle_A|\phi_k\rangle_B\Big)|\tau\rangle_{C}\Big|^2\\
&=&
\Big|\frac{1}{2^n}\sum_k\langle k0^{m-n}|_B\langle\tau|_C 
U_{BC}
|\phi_k\rangle_B|\tau\rangle_{C}\Big|^2\\
&\le&
\Big(\frac{1}{2^n}\sum_k
|\langle k0^{m-n}|_B\langle\tau|_C 
U_{BC}
|\phi_k\rangle_B|\tau\rangle_{C}|\Big)^2\\
&\le&
\frac{1}{2^n}\sum_k
|\langle k0^{m-n}|_B\langle\tau|_C 
U_{BC}
|\phi_k\rangle_B|\tau\rangle_{C}|^2\\
&\le&
\frac{1}{2^n}\sum_k
\|(|k\rangle\langle k|\otimes I)
U_{BC}
|\phi_k\rangle_B|\tau\rangle_{C}\|^2,
\end{eqnarray*}
which breaks the security of OWSG.
\end{proof}
